A Deterministic Algorithm for Balanced Cut with Applications to Dynamic Connectivity, Flows, and Beyond

We consider the classical Minimum Balanced Cut problem: given a graph $G$, compute a partition of its vertices into two subsets of roughly equal volume, while minimizing the number of edges connecting the subsets. We present the first {\em deterministic, almost-linear time} approximation algorithm for this problem. Specifically, our algorithm, given an $n$-vertex $m$-edge graph $G$ and any parameter $1\leq r\leq O(\log n)$, computes a $(\log m)^{r^2}$-approximation for Minimum Balanced Cut on $G$, in time $O\left ( m^{1+O(1/r)+o(1)}\cdot (\log m)^{O(r^2)}\right )$. In particular, we obtain a $(\log m)^{1/\epsilon}$-approximation in time $m^{1+O(1/\sqrt{\epsilon})}$ for any constant $\epsilon$, and a $(\log m)^{f(m)}$-approximation in time $m^{1+o(1)}$, for any slowly growing function $m$. We obtain deterministic algorithms with similar guarantees for the Sparsest Cut and the Lowest-Conductance Cut problems. Our algorithm for the Minimum Balanced Cut problem in fact provides a stronger guarantee: it either returns a balanced cut whose value is close to a given target value, or it certifies that such a cut does not exist by exhibiting a large subgraph of $G$ that has high conductance. We use this algorithm to obtain deterministic algorithms for dynamic connectivity and minimum spanning forest, whose worst-case update time on an $n$-vertex graph is $n^{o(1)}$, thus resolving a major open problem in the area of dynamic graph algorithms. Our work also implies deterministic algorithms for a host of additional problems, whose time complexities match, up to subpolynomial in $n$ factors, those of known randomized algorithms. The implications include almost-linear time deterministic algorithms for solving Laplacian systems and for approximating maximum flows in undirected graphs.

==> KKOV.tex <==
%!TEX root = main_det_cut.tex


\subsection{Key Tool 2: Modified KKOV's Cut-Matching Game}

\label{sec:KKOV}
\paragraph{The Cut-matching Game.}
The \emph{cut-matching
game} is introduced by Khandekar, Rao, and Vazirani \cite{KhandekarRV09} and can be viewed as a process for ``forcing'' an adversary to construct an expander for us. 
Suppose that we want to construct an expander and an adversary wants to slow us down. 
The cut-matching game between the adversary and us proceeds in rounds as follows. Initially,  we start with an empty graph $W$. In each round $t$, we first choose a cut $(S_{t},\ol{S}_{t})$ \yp{$V \setminus S_t$?} cleverly.
Then, an
adversary chooses an \emph{arbitrary} matching $M_t$ of size $\min\{|S_{t}|,|\ol{S}_{t}|\}$ \yp{$V \setminus S_t$?} crossing the cut $(S_{t},\ol{S}_{t})$ \yp{$V \setminus S_t$?} and set $W \gets W \cup M_t$. The key contribution in \cite{KhandekarRV09} is to show that even in this adversarial process, there is a simple and efficient algorithm for choosing a cut in each round so that, within a polylogarithmic number of rounds, $W$ is guaranteed to be an expander (to be more precise, the sparsity $\sigma_W$ is high). 


The crucial property of the cut-matching game is that, given a graph $G$, the process allows us to easily embed $W$ into $G$. This is because embedding a matching crossing a cut $(S_{t},\ol{S}_{t})$ exactly corresponds to finding a  flow where  $S_t$ contains source nodes and  $\ol{S}_t$ contains sink nodes (and decomposing the flow into paths). As $W$ is a union of such matchings, it suffices to solve polylogarithmic instances of the flow problem. Since the resulting $W$  must be an expander, we can arguing about the conductance of $G$.

The  algorithm for choosing cuts by   \cite{KhandekarRV09} is inherently randomized and we do not know how to use it.
Fortunately, Khandekar, Khot, Orecchia, and Vishnoi
(KKOV) \cite{KhandekarKOV2007cut} show another way for choosing a cut in the cut-matching game. They show that, by choosing a most-vertex-balanced sparsest cut in each round, the number of rounds is at most logarithmic. Although this can be found deterministically,  finding such cut is NP-hard. 

In this section, we slightly modify KKOV's framework and show that the number of rounds is still small even when we allow an approximate result -- in particular, when a cut is returned by $\vBCut$. This idea was also used in vertex connectivity algorithms~\cite{GaoLNPSY19}.


%In this section, we state a process for constructing expanders which
%is a variant of a general framework called the \emph{cut-matching
%game} introduced by Khandekar, Rao, and Vazirani \cite{KhandekarRV09} where the process involves
%alternation between finding cuts and adding matchings. Our process is a slight
%modification of the one by Khandekar, Khot, Orecchia, and Vishnoi
%(KKOV) \cite{KhandekarKOV2007cut} and is implicit in \cite{GaoLNPSY19}.

\begin{thm}
\label{thm:KKOV}Given a number $n$, a parameter $\phi\in[0,1/4]$,
\ref{alg:KKOV} calls a $\vBCut$ algorithm for $R\ge c_{\KKOV}\log n$ many times where
$c_{\KKOV}$ is some constant, and then returns an $n$-node graph
$W$ with maximum degree $R$ and $\sigma_{W}\ge\phi/9$. Hence, $\Phi_{W}\ge\phi/9R$.
\yp{$\Phi(W)$?}
\end{thm}

The proof of \ref{thm:KKOV} is almost the same as the one in \cite{KhandekarKOV2007cut}
but we slightly adjust small details so that it fits well with other parts of our algorithms. Therefore, we only include the proof in the appendix for completeness.

\begin{algorithm}[H]
\underline{Input}: A number $n$ and a parameter $\phi\in[0,1/4]$. Let
$R\ge c_{\KKOV}\log n$ where $c_{\KKOV}$ is some constant.

\underline{Output}: An $n$-node graph $W$ with maximum degree $R$
and $\sigma_{W}\ge\phi/9$ (so $\Phi_{W}\ge\phi/9R$ \yp{$\Phi(W)$?}).
\begin{enumerate}
\item Let $W_{0}$ be an $n$-node empty graph.\danupon{This should be $W_1$ or we should start from $t=0$.} 
\item For $t=1,\dots,R$:
\begin{enumerate}
\item $A_{t}\gets\vBCut(W_{t},R,1/4,\phi)$.
\item Let $B_{t}$ be an arbitrary subset of $V-A_{t}$ where $|B_{t}|=|A_{t}|$.
\item $W_{t}\gets W_{t-1}\cup M_{t}$ where $M_{t}$ is an \emph{arbitrary} matching
between $A_{t}$ and $B_{t}$ of size $|A_{t}|$.
\end{enumerate}
\item Return $W=W_{R}$. 
\end{enumerate}
\caption{\label{alg:KKOV}The modified cut-matching game framework of \cite{KhandekarKOV2007cut}.}
\end{algorithm}



==> abstract-para.tex <==
Specifically, we provide a deterministic algorithm, that, for any parameter $1\leq r\leq O(\log n)$, computes a$(\log m)^{r^2}$-approximate solution to the Balanced Cut problem on an $m$-edge graph $G$, in time $O\left ( m^{1+O(1/r)+o(1)}\cdot (\log m)^{O(r^2)}\right )$. In particular, we obtain  a $(\log m)^{1/\epsilon}$-approximation  in time $m^{1+O(1/\sqrt{\epsilon})}$ for any constant $\epsilon$, and a $(\log m)^{f(m)}$-approximation in time $m^{1+o(1)}$, for any slowly growing function $m$. We obtain deterministic algorithms with similar guarantees for the Sparsest Cut and the Lowest-Conductance Cut problems.

==> alg-names.tex <==
Thm 1.5: \cutorcert
Thm 2.4: \constructexpander
Lemma 2.9: \extractexpander

Cor 3.7: \routeorcut
Thm 3.8: \routeorcutp


Section 5.2: \reducedegree
Lemma 5.3: \makecanonical


Algorithm \reducedegree from \ref{subsec:constant degree}
 Algorithm \makecanonical from \ref{lem: degree reduction balanced cut case}

==> application-leftovers.tex <==







\subsection{R\"{a}cke tree and Multi-commodity flow}
\thatchaphol{TODO:Explain this more.}
The single-tree based oblivious routing scheme (a.k.a. R\"{a}cke tree)
by R\"{a}cke, Shah, and Taubig~\cite{RackeST14} can also be
derandomized by using our balanced cut routine as the
cut player in its cut-matching game.
However, this use introduces again an overhead of $n^{o(1)}$
in the approximation ratio.
%Therefore, matching the best randomized overhead of $\polylog(n)$ 
%for approximate maximum flow~\cite{Peng16} may be the most
%direct goal for improving the performances of these derandomized
%graph preconditioning routines.

Once R\"{a}cke tree can be derandomized, we can immediately obtain an $\Ohat(mk/\eps)$-time deterministic algorithm for $(1+\eps)$-approximate $k$-concurrent-commodity flow~\cite{Sherman17} by plugging a deterministic R\"{a}cke tree into the algorithm by \cite{Sherman17}.
On the other hand, the more recent  method by Sidford and Tian~\cite{SidfordT18} uses randomization in its intermediate steps: it remains an interesting question whether it can be derandomized as well.


\subsection{$\ell_{p}$ Norm Sparsifier}
The deterministic spectral sparsifier algorithm from \ref{cor:sparsifier} also implies derandomization of 
the mixed $\ell_{2}$ and $\ell_{p}$ norm sparsifier
in unit-capacitated graphs by Kyng, Peng, Sachdeva, and Wang~\cite{KyngPSW19}\label{item:L2pSparsify}. 	
This further implies a derandomization of the overall
$\ell_{p}$-norm flow algorithm in~\cite{KyngPSW19}.
This is due to the direct analog between that algorithm and
the Spielman-Teng solver~\cite{SpielmanT14-ThirdJournal},
namely that it builds ultra-sparsifiers by moving edges
around a low-stretch spanning tree, and then sparsifies
the graph on a smaller subset of vertices.
This gives an algorithm for computing the minimum energy 
$\ell_{p}$ flows to an additive error of $1 / \poly(n)$
in undirected unit weighted graphs that runs in time
$\Ohat(\exp(O(p^{3/2})) m^{1 + O(\frac{1}{\sqrt{p}})})$.
This subroutine can also be applied to the more general
weighted setting, leading to running times of the
form $\Ohat(\exp(O(p)) ( m + n^{\frac{|p-2|}{2p + |p-2|}}))$
for $1 / poly(n)$ relative error solutions~\cite{AdilKPS19}.
It can also be used in conjunction with subsequent improvements
on the $p$ dependences~\cite{AdilPS19:arxiv,AdilS20}.
\thatchaphol{TODO: ask richard. Does this imply $m^{11/8}$-time deterministic algorithm for max flow and so on?}




\subsection{Simplification of the [KT] Algorithm}
Given  \ref{cor:exp decomp nophi},
we can significantly simplify   Kawarabayashi and Thorup's  \cite{KawarabayashiT19} deterministic algorithm for computing edge
connectivity. 
The idea is as follows: Suppose we are given an $n$-node $m$-edge graph with minimum degree  $\delta$.
The key step in  \cite{KawarabayashiT19} is to compute the \emph{KT-decomposition} of a graph into \emph{clusters} such that, each cluster can overlap any min cut by at most two nodes. In \cite{KawarabayashiT19}, they give a quite involved algorithm for computing this decomposition. 

We argue that, by paying a $n^{o(1)}$ in the running time, this decomposition algorithm can be simplified into a three-step algorithm: 
First, compute a $\delta$-sparse certificate \cite{NagamochiI92} as in \cite{KawarabayashiT19}.
Second, compute expander decomposition on the sparse certificate using \ref{cor:exp decomp nophi} with $\epsilon = n^{o(1)}/\delta$. 
Third, \emph{trim} each expander from the previous step where the operation trim is defined in \cite{KawarabayashiT19}. It can be shown in each trimmed expander must be a cluster according to  KT-decomposition (see \cite{DagaHNS19}).
After contracting the \emph{core} of each cluster (as defined in \cite{KawarabayashiT19}), we will obtain a graph with $n^{1+o(1)}$ edges and $n^{1+o(1)}/\delta$ nodes where all non-trivial min cuts are preserved. So we can compute the edge connectivity on this contracted graph in $\Ohat(m)$ time using Gabow's algorithm as \cite{KawarabayashiT19} does.   

==> application-max-flow-back-up.tex <==
%!TEX root = main_det_cut.tex

\subsection{Congestion Approximators and Approximate Maximum Flow}

In this subsection we discuss applications of our results to approximate maximum $s$-$t$ flow in undirected edge-capacitated graphs. Given an edge-capacitiated graph $G=(V,E)$, and a target flow value $b$, together with an accuracy parameter $0<\eps<1$, the goal is to either compute an $s$-$t$ flow of value at least $(1-\epsilon)b$, or to certify that the maximum $s$-$t$ flow value is less than $b$, by exhibiting an $s$-$t$ cut of capacity less than $b$. We note that the problem can equivalently be defined using a demand function $\bb: V\rightarrow \reals$ with $\sum_{v\in V}\bb_v=0$, by setting $\bb_s=1$, $\bb_t=-1$, and, for all $v\in V\setminus\set{s,t}$, $\bb_v=0$. %Given a cut $(S,\overline S)$ in $G$, we denote 
In general, given an arbitrary demand function $\bb: V\rightarrow \reals$ with $\sum_{v\in V}\bb_v=0$, we say that a flow $f$ \emph{satisfies} the demand $\bb$ iff, for every vertex $v\in V$, the \emph{excess flow at $v$}, which is the total amount of flow entering $v$ minus the total amount of flow leaving $v$, is precisely $\bb_v$.

The maximum $s$-$t$ flow problem is among the most basic and extensively studied problems. There are several  near-linear time randomized algorithms for computing $(1+\epsilon)$-approximate maximum flows \cite{Sherman13,KelnerLOS14,Peng16}; the fastest current randomized algorithm, due to Sherman \cite{Sherman17}, has running time $\Otil(m/\epsilon)$. Our results imply a deterministic algorithm for approximate maximum flow in undirected edge-capacitated graphs, with almost-linear running time.

%A $(1+\epsilon)$-approximate max flow in undirected edge-capacitated graphs can be computed in near-linear time by randomized algorithms \cite{Sherman13,KelnerLOS14,Peng16}. The currently fastest randomized algorithm takes  $\Otil(m/\epsilon)$ time and is by Sherman \cite{Sherman17}. Below, we present a $\Ohat(m/\epsilon^2)$-time deterministic algorithm. 
%Combining the congestion approximators with the area convexity based accelerated methods by Sherman~\cite{Sherman17} gives a deterministic, almost linear time, approximate max-flow algorithm with $1 / \epsilon$ dependencies.
\begin{cor}
\label{cor:maxflow} There is a deterministic algorithm that, given an $m$-edge graph $G$ with capacities $\cc_e\geq 0$ on edges $e\in E$, such that $\frac{\max_{e}\cc_{e}}{\min_{e}\cc_{e}}\leq O(\poly(n))$, a demand function $\bb\in\mathbb{R}^{V}$  with  $\sum_{v\in V}\bb_{v}=0$, and an accuracy parameter $0<\epsilon\leq 1$, computes, in time $T_{\Maxflow}(m,\epsilon)=O\left(m\cdot 2^{O(\log m\log \log m)^{5/6}}\epsilon^{-2}\right)$,
one of the following: either
\begin{itemize}
\item \textbf{(Flow): }a flow satisfying the demand $\bb$ with $\abs{f(e)}\le (1+\epsilon)\cc_e$ for every edge $e$; or
\item \textbf{(Cut):} a cut $S$ such that $\sum_{e\in E(S,\overline{S})}\cc_{e}<\abs{\sum_{v\in S}\bb_{v}}$
\end{itemize}
\end{cor}

%We first use \ref{cor:sparsifier} to sparsify $G$ into $G'$ with $O(n\log ^2 n)$ edges. $G'$ is an $n^{o(1)}$-approximate spectral sparsifier construct deterministically a oblivious routing scheme 
%We explain the proof of this application in more detail because it will be used later for our balanced cut algorithm in the low conductance regime.

Our proof of Corollary \ref{cor:maxflow} closely follows the algorithm of ~\cite{Sherman13}, and proceeds by constructing a congestion approximator. Unlike the algorithm in~\cite{Sherman13}, our algorithm for computing the congestion approximator is deterministic, and is obtained by replacing a randomized procedure in~\cite{Sherman13} for constructing a cut sparsifier with the deterministic algorithm from \ref{cor:sparsifier}. We then use the reduction from $(1+\eps)$-approximate maximum flow to congestion approximators by~\cite{Sherman13}. 

Suppose we are given a graph $G=(V,E)$, where $E=\set{e_1,\ldots,e_m}$, with capacities $\cc_e$ on edges $e\in E$. Let $C$ be the diagonal $(m\times m)$ matrix, such that for all $1\leq i\leq m$, the entry $(i,i)$ in the matrix is $\cc_{e_i}$. Assume now that we are given a demand vector $\bb:V\rightarrow \reals$, with $\sum_{v\in V}\bb_v=0$. Let $f$ be any flow that satisfies the demand $b$. The \emph{congestion} $\eta$ of this flow is the maximum, over all edges $e\in E$, of $f(e)/\cc_e$. Equivalently, $\eta=\norm{C^{-1}f}_{\infty}$. By scaling flow $f$ by factor $\eta$, we obtain a valid flow routing demand $\bb/\eta$. Therefore, the maximum $s$-$t$ flow problem is equivalent to the following problem: given a graph $G=(V,E)$ with capacities $\cc_e$ on edges $e\in E$ and a demand vector $\bb:V\rightarrow \reals$, with $\sum_{v\in V}\bb_v=0$, compute a flow $f$ satisfying the demand $\bb$, while minimizing the congestion  $\eta=\norm{C^{-1}f}_{\infty}$ among all such flows.
For convenience, we define an \emph{incidence} matrix $B$ associated with graph $G$. We direct the edges of graph $G$ arbitrarily. Matrix $B$ is an $(m\times n)$ matrix, whose rows are indexed by edges and columns by vertices of $G$. Entry $(e_i,v_j)$ is $-1$ if $e_i$ is an edge that leaves $v_j$, it is $1$ if $e_i$ is an edge that enters $v_j$, and it is $0$ otherwise. Notice that, given any flow $f$, the $j$th entry of $B\cdot f$ is the \emph{excess flow} on vertex $v_j$: the total amount of flow entering $v_j$ minus the total amount of flow leaving $v_j$.



We start by recalling the definition of congestion approximators from \cite{Sherman13}.
\begin{defn}
Let $G$ be a graph with $n$ vertices and $m$ edges, let $C$ be the diagonal matrix containing of edge weights and let $B$ be the $n\times m$ incidence matrix. An $\alpha$-congestion approximator for $G$ is a matrix $R$ that contains $n$ columns and an arbitrary number of rows, such that for any demand vector $\bb$, 
\[
\norm{R\bb}_{\infty}\le \mathsf{opt}(\bb)\le \alpha\norm{R\bb}_{\infty},
\] where $\mathsf{opt}(\bb)$ is the value of the optimal solution for the minimum-congestion flow problem
\[
\min\ \norm{C^{-1}f}_{\infty} s.t.\ Bf=\bb.
\]
\end{defn}



The main goal of this section is to prove the following lemma, that provides a deterministic construction of congestion approximators, and is used to replace its randomized counterpart, Theorem 1.5 in \cite{Sherman13}. We note that we obtain somewhat weaker parameters in the approximation factor and the running time.


\begin{lem}[Deterministic version of Theorem 1.5,~\cite{Sherman13}]
\label{lem:det15sherman13}
%Let $f(x)$ be a family of functions that are bounded by
%$x\cdot 2^{O(\log (x)\log\log (x))^{2/3}}$. $O\left(f(m)+f(n)\right)$.
There is a routine $\mathtt{CongestionApproximator}(G, k)$ that
for any $1\le k\le O(\log n)$, constructs a $(2^{k \cdot O(\log n\log \log n)^{2/3}})$-congestion
approximator $R$, in deterministic time $O(m^{1 + 1/k} 2^{k \cdot O(\log n\log \log n)^{2/3}} )$.
Once constructed, for any vector $b\in \reals^n$,
we can compute $Rb$ and $R^\top b$ in time $\Otil(n^{1+1/k} \log^{O(k)} n)$.
\end{lem}


Given a cut $(S,\overline S)$ in an edge-capacitated graph $G$, we denote $\cc_S=\sum_{e\in E(S, \overline{S})}\cc_e$. Given a demand vector $\bb$ for $G$, we also denote $\bb_S=\abs{\sum_{v\in S}\bb_v}$.

Sherman \cite{Sherman13} provides the following method for turning an
efficient congestion approximator to an approximate maximum flow algorithm.

\begin{lem}[Theorem 1.2~\cite{Sherman13}]
	\label{lem:almost} There is a deterministic algorithm that, given a graph $G=(V,E)$ with edge weights $\cc_e$ for $e\in E$ and a  demand vector $\bb: V\rightarrow \reals$ with $\sum_{v\in V}\bb_v=0$, together with an access 
	access to an $\alpha$-congestion-approximator $R$ of $G$, makes $\tilde{O}(\alpha \eps^{-2})$ iterations, and returns a flow $f$ and cut $S$ in $G$, with $Bf = \bb$ and $\norm{C^{-1}f}_{\infty} \le (1 + \eps)\bb_S/\cc_S$. Each iteration requires $O(m)$ time, plus a multiplication of a vector in $\reals^n$ by $R$ and $R^\top$.

\end{lem}

Note that combing~\ref{lem:det15sherman13} with the parameter $k=(\log n)^{1/6}$ and~\ref{lem:almost} immediately yields a proof of~\ref{cor:maxflow}. Indeed, if the algorithm from~\ref{lem:almost} outputs a cut $S$ with $\bb_S>\cc_S$, then we return the cut $S$ as the outcome of our algorithm for~\ref{cor:maxflow}. Otherwise, $\bb_S/\cc_S\le 1$ must hold, and so the flow $f$ output by~\ref{lem:almost} satisfies $\norm{C^{-1}f}_{\infty}\le 1+\epsilon$. We then return $f$ as the outcome of~\ref{cor:maxflow}. 
The algorithm from \ref{lem:almost}  performs $\tilde O(\alpha/\eps^2)$ iterations, where $\alpha=\left(2^{O(k\log n\log \log n)^{2/3}}\right)=2^{O(\log m\log \log m)^{5/6}}$. Every iteration takes time $O(m+n^{1+1/k})$. Therefore, the total running time
of the algorithm from \ref{lem:almost} is at most $O\left (m\cdot 2^{O(\log m\log \log m)^{5/6}}/\eps^2\right )$. The additional time that is needed in order to construct the cut approximators is $O\left (m\cdot 2^{O(\log (m)\log\log (m))^{2/3}}\right )$, and so the total running time of the algorithm is bounded by $O\left (m\cdot 2^{O(\log m\log \log m)^{5/6}}/\eps^2\right )$.

Thus, for the max-flow routines claimed in \ref{cor:maxflow},
it remains to show the deterministic construction of congestion approximators
as stated in \ref{lem:det15sherman13}.

\yp{I started editting here}

This construction is in turn a direct modification of the J-tree based
construction of cut approximators by Madry~\cite{Madry10-jtree}.
It is based on the ability to alternatively reduce vertices an dedges
in graphs, the former via routing along adaptively generated low stretch
spanning trees, and the latter via cut sparsifiers, which are implied
by the spectral sparsifiers as specified in~\ref{cor:sparsifier}.
Our modifications of the constructions of Madry~\cite{Madry10-jtree}
and Sherman~\cite{Sherman13} consist of three main components:
\begin{enumerate}
	\item Observing that the routing along trees is entirely deterministic.
	\item Showing that the cut sparsifier can be directly substituted by the
	deterministic variants from~\ref{cor:sparsifier}.
	\item Showing that instead of sampling the distribution over partial routings,
	we can instead recurse on each of them, and analyzing the total cost of the
	recursion.
\end{enumerate}

To do this, we first need to formally introduce the notion of
partial routings along trees.
This is defined as a J-tree below Figure 2 of~\cite{Madry10-jtree}.

\begin{defn}
	A graph $H$ is a $j$-tree if it's a union of:
	\begin{enumerate}
		\item a subgraph $H'$ of $H$ induced by a subset of at most $j$ vertices, $V_{H'}$ plus
		\item a forest where each connected component has exactly one vertex in $V_{H'}$.
	\end{enumerate}
\end{defn}

Intuitively these objects are formed by moving edges along edges
of a spanning tree to a suitably identified subset of vertices.
This incurs congestion along the tree edges, and this congestion
is in turn distributed over the trees from the distribution via
a multiplcative update scheme simliar to the construction of nearly-optimal
oblivious routings by Racke~\cite{Racke08}.
Such guarantee can be encapsulated by the following rephrasing of
Theorem 3.6. from~\cite{Madry10-jtree}.

\begin{lem}[\cite{Madry10-jtree}] \label{thm:madrythm}
	There is a deterministic algorithm that, given an edge-weighted graph $G=(V, E, \ww)$ with $|E|=m$ and $U=\frac{\max_{e\in E}\ww_e}{\max_{e\in E}\ww_e}\leq O(\poly(n))$, together with a parameter $t \geq 1$, computes, in time $\tilde{O}(tm)$, a distribution $\set{\lambda_i}_{i=1}^{\ceil{t\log U}}$ over a collection of $\ceil{t\log U}$ edge-weighted graphs $G_1,\ldots,G_{\ceil{t\log U}}$, where for each $1\leq i\leq \ceil{t\log U}$, $G_i=(V, E_i, \ww_i)$, and the following hold:
	\begin{itemize}
		\item for all $1\leq i\leq \ceil{t\log U}$, graph $G_i$ is an $O(m/t)$-tree, whose core contains at most $m$ edges;
		\item for all $1\leq i\leq \ceil{t\log U}$, $G$ embeds into $G_i$ with congestion $1$; \yg{was $G_i$ embeds into $G$} and %, i.e. for each cut $C\subseteq V$, $\sum_{e\in E_i(C, \overline{C})}(\ww_i)_e\ge \sum_{e\in E(C, \overline{C})}\ww_e$.
		%\thatchaphol{Either define dominate, or just write the mathematical definition here.}
		\item the graph that's the average of these graphs over the distribution,
		$\tilde G= \sum_{i} \lambda_i G_i$ can be embedded into $G$ with congestion $O(\log n (\log\log n)^{O(1)})$.
	\end{itemize}
\end{lem}

This distribution of $O(m / t)$-trees essentially lets us reduce the cuts
to consider to:
\begin{enumerate}
	\item singleton edges among the trees, plus
	\item cuts separating the $O(m / t)$ core vertices,
	with all the tree/forest edges omitted.
\end{enumerate}

This is formally proven by first showing that the embedability conditions
gives that checking the capcaities of these trees across all cuts gives
an $O(\log{n})$-approximation to the optimum congestion of the max-flow.
This is shown in the proofs of Theorem 4.1 and Lemma 6.1.
of~\cite{Madry10-jtree}.
Specificlaly, these lemmas show that a tree sampled from the distribution
with probability proportional to $\lambda_{i}$ gives a good bound to the
optimum with constant probability.
That in turn implies checking through all the $O(m / t)$-trees in the
collection ensures that we examine that instance as well.

Next, we show that it suffices to check all core cuts,
plus all tree edge cuts in each of the $j$-trees.

\begin{lem}
	If $H = (V_H, E_H, \cc_{H})$ is a j-tree with core $V_{H'}$,
	and $\bb$ is a demand vector such that:
	\begin{enumerate}
		\item for tree in the peripheral forest, the demand routes
		with congestion $\rho$,
		\item the demand vector that's the sum over each of the trees
		routes on the core graph with congestion $\rho$,
	\end{enumerate}
	then $\bb$ routes in $H$ with congestion $O(\rho)$ as well.
\end{lem}
Note that these cuts are a subset of all possible cuts in $H$,
so checking these cuts (ones on trees, plus ones on core) provides
a lower bound on the congestion needed to route $\bb$ as well.

\todo{the proof below is a sketch, but I feel the pieces are there already}

\begin{proof}
	Consider routing $\bb$ in two stages:
	first, all the demand in each tree moves to its root.
	The congestion of this is exactly the max congestion of a
	tree edge, since the flow across a tree is uniquely determined
	by the vertex demands.
	
	Then we route all the demands at the root vertices
	across the core graph.
\end{proof}

%\thatchaphol{TODO: explain more the output of \Cref{lem:almost} gives gives approximate max flow in \Cref{cor:maxflow}.}
%\thatchaphol{TODO: compute the subpolynomial factor in the running time because it will be used later in other section.}
%\yu{This requires the running time of~\ref{cor:sparsifier} which requires that of~\ref{cor:expander decomp}}

Thus, we can recurse on all core graphs after sparsifying them.
This leads to the algorithm $\mathtt{CongestionApproximator}$
whose pseudocode is given~\ref{alg:CongestionApproximator}

\begin{algorithm}
	$\mathtt{CongestionApproximator}(G, k)$:
	\begin{itemize}
		\item If $n=1$, return.
		\item Using theorem \ref{thm:madrythm} with $t = m^{1/k}$,
		compute distribution $(\lambda_i, H_i)_{i=1}^{\ceil{ t\log U}}$ of $\max(1,m/t)$-trees.  
		\item For each $i$:
		\begin{itemize}
			\item For each edge $e$ in the forest of $G_i$:
			\begin{itemize}
			\item %Add all tree cuts in $G_i$ to the list of cuts in the congestion approximator.
			Let $c$ be the capacity of $e$. Let $S$ be the set of vertices that are disconnected with the core of $H_i$ when cutting $e$. We call $S$ a tree cut with capacity $c$. Append a row $\chi_S/c$ into the congestion approxi mator.)
			\end{itemize} 
			\item Let $H'_i$ be the core graph of $H_i$ (with edges in the forest of $H_i$ removed).
			\item Set $\tilde{H}'_i \leftarrow \mathtt{Sparsify}(H'_i, r), t)$, where
				$\mathtt{Sparsify}$ was introduced in~\ref{cor:sparsifier}.
			\item Recursively call $\mathtt{CongestionApproximator}(\tilde{H}'_i, k)$.
		\end{itemize}
	\end{itemize}
\caption{Pseudocode for Constructing Congestion Approximator}
\label{alg:CongestionApproximator}
\end{algorithm}

We analyze the correctness of the congestion approximator
produced, and the overall running time, below.

\begin{proofof}{\Cref{lem:det15sherman13}}
	We first bound the quality of the congestion approximator
	produced.
	
	The recursion will proceed for $k$ levels.
	Each layer, the converstion to $j$-trees incur a multiplicative error of $O(\log{n})$,
	while the sparsifier by~\ref{cor:sparsifier} and the setting of $r \leftarrow k$
	incurs a multiplicative error of $O(\log^{O(k^2)}n)$.
	So compounding across the $k$ layers gives that the resulting set of cuts
	is an $O(\log^{k^3}n)$ approximator.
	
	Then it remains to bound the total running time and size of approximators.
	At each level, each of the $\max\{1, m/t\}$-trees have at $m/ t$ vertices,
	which by the increases in sizes in the cut sparsifiers from~\ref{cor:sparsifier}
	gives at most $O(m^{1-1/k} \log^{2}n)$ edges.
	Summing across the $\tilde{O}(t \log{n})$ graphs in the distribution
	gives a total size of $O(m \log^{3}n)$, aka. an increase by a factor of
	$O(\log^{3}n)$ across each level of the recursion.
	Thus the total sizes of these graph after $k$ levels of recursion is
	$O(m \log^{3k} n$.
	
	This size serves as an upper bound on the total number of cuts examined in the trees.
	Multiplying in the cost of running the sparisifer then gives the overall runtime as well.
\end{proofof}

\yp{below is the previous version}

\paragraph{Proof of \Cref{lem:det15sherman13}.}

We modify the algorithm called $\mathtt{ComputeTrees}$ from \cite{Sherman13} that relies on two main components: 
 \emph{$j$-trees}, and cut sparsifiers. We now discuss each of these components in turn.

\begin{algorithm}
	$\mathtt{ComputeTrees}(G,t)$:
	\begin{itemize}
		\item If $n=1$, return.
		\item Using theorem \ref{thm:madrythm}, compute distribution $(\lambda_i, G_i)_{i=1}^{t'}$ of $\max(1,n/t)$-trees.  
		\item Pick the $t$ graphs of largest $\lambda_i$, throw away the rest, and scale the kept $\lambda_i$ to sum to $1$.
		\item For $i = 1,\ldots,t$:
		\begin{itemize}
			\item $H_i' \gets \mathtt{Sparsify}(H_i)$, where $H_i$ is the core of $G_i$
			\item $L_i \gets \mathtt{ComputeTrees}(H_i', t)$
		\end{itemize}
		\item Return the list $L = (\lambda_i, F_i, L_i)_{i=1}^t$ where $F_i$ is the forest of $G_i$.
	\end{itemize}
	
\end{algorithm}


Next, we generalize our definition of embeddings of graphs to weighted graphs.

\begin{defn} [Embeddings of weighted graphs]
	Let $G$, $H$ be two graphs with $V(G)= V(H)$. Assume also that we are given edge weights $\ww_e$ for all edges $e\in E(H)$ be $\ww_e$. An \emph{embedding} of $H$ into $G$ is a collection $\pset=\set{P(e)\mid e\in E(H)}$ of paths in $G$, such that for each edge $e\in E(H)$, path $P(e)$ connects the endpoints of $e$ in $G$. We say that the embedding causes \emph{congestion} $\cong$ iff for every edge $e'\in E(G)$: \[\sum_{\stackrel{e\in E(H):}{e'\in P(e)}}\ww_e\le \cong.\]
	\end{defn}


We also need the following definition for composition of graphs.

\begin{defn}
Let $G=(V, E, \ww)$ and $H=(V, E', \ww')$ be two edge-weighted graphs defined over the same vertex set. We define their composition $K=G+H$ be an edge-weighted graph $K=(V, F, \zz)$, where $F$ is the disjoint union of the edge sets $E$ and $E'$, and for every edge $e\in F$, its weight is defined to be $\zz_e=\ww_e$ if $e\in E$ and $\zz_e=\ww'_e$ if $e\in E'$.

Given an edge-weighted graph $G=(V, E, \ww)$ and a scalar $\alpha$, we let $\alpha G$ be the edge-weighted graph $(V, E, \alpha \ww)$.
\end{defn}

Notice that we can naturally extend graph decomposition to more than two graphs. This allows us to define, for a given distribution over graphs $G_1,\ldots,G_r$ that are defined over the same vertex set, an ``expectation'' graph $\expect[i]{G_i}$:

\begin{defn}
	Suppose we are given a family $\set{G_1,\ldots,G_r}$ of edge-weighted graphs, where for all $1\leq i\leq r$, $G_i=(V,E_i,\ww^i)$, so all graphs are defined over the same vertex set. Assume further that we are given a probability distribution $\set{\lambda_i}_{i=1}^r$ over these graphs. Then the \emph{expectation graph} is defined to be $\tilde G=\expect[i]{G_i}=\sum_{i=1}^r\lambda_iG_i$. In other words, $V(\tilde G)=V$; $E(\tilde G)=\bigcup_{i=1}^rE_i$, and, for every edge $e\in E(\tilde G)$, its weight in $\tilde G$ is defined to be $\lambda_i\ww^i_e$, where $1\leq i\leq r$ is the index with $e\in E_i$. 
\end{defn}
 

Lastly, we need the following definition.

\begin{defn}
	Suppose we are given two edge-weighted graphs $G=(V,E,\ww)$ and $H=(V,E',\ww')$ that are defined over the same vertex set. We say that \emph{$G$ cut-dominates $H$}, and denote $G\geq_c H$ iff for every partition $(S,\overline S)$ of $V$, $\sum_{e\in E_G{S,\overline S}}\ww_e\geq \sum_{e\in E_H{S,\overline S}}\ww_e'$.
\end{defn}

We are now ready to state the theorem of Madry \cite{Madry10-jtree} that provides a deterministic algorithm for computing $j$-trees.

\begin{thm}[\cite{Madry10-jtree}] \label{thm:madrythm}
	There is a deterministic algorithm that, given an edge-weighted graph $G=(V, E, \ww)$ with $|E|=m$ and $U=\frac{\max_{e\in E}\ww_e}{\max_{e\in E}\ww_e}\leq O(\poly(n))$, together with a parameter $t \geq 1$, computes, in time $\tilde{O}(tm)$, a distribution $\set{\lambda_i}_{i=1}^{\ceil{t\log U}}$ over a collection of $\ceil{t\log U}$ edge-weighted graphs $G_1,\ldots,G_{\ceil{t\log U}}$, where for each $1\leq i\leq \ceil{t\log U}$, $G_i=(V, E_i, \ww_i)$, and the following hold:
	\begin{itemize}
		\item for all $1\leq i\leq \ceil{t\log U}$, graph $G_i$ is an $O(m/t)$-tree, whose core contains at most $m$ edges;
		\item for all $1\leq i\leq \ceil{t\log U}$, $G_i\ge_c G$; and %, i.e. for each cut $C\subseteq V$, $\sum_{e\in E_i(C, \overline{C})}(\ww_i)_e\ge \sum_{e\in E(C, \overline{C})}\ww_e$.
		%\thatchaphol{Either define dominate, or just write the mathematical definition here.}
		\item graph $\tilde G=\expect[i]{G_i}$ can be embedded into $G$ with congestion $O(\log n (\log\log n)^{O(1)})$.
	\end{itemize}
\end{thm}


\paragraph{Cut Sparsifiers.}
For the second component, the algorithm by \cite{Sherman13} uses the randomized algorithm of Benczur and Karger \cite{BK} for computing cut sparsifiers: given any graph $G$ with $m$ edges, the algorithm computes a $2$-approximate cut sparsifier $G'$ for $G$ containing $O(n\log n)$ edges. We replace this algorithm by the deterministic algorithm given in \ref{cor:sparsifier} that for any graph $G$ with $n$ vertices and $m$ edges, computes an $2^{O(\log n\log \log n)^{2/3}}$-approximate spectral sparsifier $G'$ for $G$ with $O(n\log ^2n)$ edges. We call this algorithm $\mathtt{Sparsify}(G)$. 

Since the deterministic algorithm provides weaker guarantees than that of \cite{BK}  in terms of the approximation factor,
the congestion that our algorithm incurs in each recursive layer of Algorithm $\mathtt{ComputeTrees}$ from~\cite{Sherman13} increases by factor $n^{o(1)}$. This is our only modification to $\mathtt{ComputeTrees}$.

The following lemma is key to our algorithm. The lemma is similar to   Lemma 3.4~\cite{Sherman13}, except that it provides a deterministic algorithm, a the cost of obtaining worse running time and congestion guarantees. We emphasize that the randomized algorithm $\mathtt{SampleTree}$ in the statement of \ref{lem:34sherman13} is used for analysis of the proof only. 


\begin{lem}[modified version of Lemma 3.4,~\cite{Sherman13}]
\label{lem:34sherman13}
Let $f(x)$ be the family of functions bounded above by $x2^{O(\log (x)\log\log (x))^{2/3}}$. Let $G$ have $\Otil(n)$ edges, and set $L\leftarrow \mathtt{ComputeTrees}(G,t)$.  Then, every tree $T$ in the sample space of $\mathtt{SampleTree}(L)$ satisfies $T\ge G$, and $E[\mathtt{SampleTree}(L)]$ can be embedded in $G$ with congestion $\left(2^{O(\log n\log \log n)^{2/3}}\right)^{\log n/\log t}$. Further, the computation of $L$ takes $O(f(n))$ time.
\end{lem}
%It remains to prove \ref{lem:34sherman13}.

\begin{proof}
The following proof is almost identical with the proof of Lemma 3.4 in \cite{Sherman13}.
By induction on $n$. For $n=1$ the claim is vacuous, so suppose $n=t^{k+1}$.  The distribution output by~\ref{thm:madrythm} will have $t\log U$ entries.  We have $H'_i\ge H_i$ and $H_i+F_i\ge G$. Furthermore, the inductive hypothesis implies that every tree $T_i$ in $\mathtt{SampleTree}(L_i)$ satisfies $T_i\ge H'_i$. Then, \[T_i+F_i\ge H'_i+F_i\ge H_i+F_i=G_i\ge G.\] Sparsifying the distribution from $t\log U$ to $t$ scales $\lambda_i$ by at most $\log U$, so that $\sum^t_{i=1}\lambda_i G_i$ can be embedded in $G$ with congestion at most $\log U$ larger than the  original distribution. Since $H'_i\le 2^{O(\log n\log \log n)^{2/3}}H_i$, by the multicommodity max-flow/min-cut theorem~\cite{LeightonR99} $H'_i$ can be embedded in $H_i$ with congestion $2^{O(\log n\log \log n)^{2/3}}$.  By the inductive hypothesis, $E[\mathtt{SampleTree}(L_i)]$ is routable in $H'_i$ with congestion $\left(2^{O(\log n\log \log n)^{2/3}}\right)^k$. It follows then that $E[\mathtt{SampleTree}(L)]$ can be embedded in $G$ with congestion at most $\left(2^{O(\log n\log \log n)^{2/3}}\right)^{k+1}$. Finally, $\mathtt{ComputeTrees}$ requires $\Otil(tn)$ time to compute the distribution, another $O(f(n))$  time to sparsify the cores, and then make $t$ recursive calls on sparse graphs with $n/t$ vertices. It follows that the running time of $\mathtt{ComputeTrees}$ is $O(f(n))$.
\end{proof}


Several lemmas from~\cite{Sherman13} are required to prove \ref{lem:det15sherman13} but their proofs remain the same: 

\begin{lem}[Lemma 3.5,~\cite{Sherman13}] Let $R$ be the matrix that has a row for each forest edge in our data structure, and $(Rb)_e$ is the congestion on that edge when routing $b$.  If $\E[\SampleTree(L)]$ can be embedded in $G$ with congestion $\alpha$, then $R$ is a $\alpha$-congestion-approximator for $G$.  Further, $R$ has $\tilde{O}(tn)$ rows.
\end{lem}

Having constructed our representation of $R$,~\cite{Sherman13} shows how to multiply by $R$ and $R^\top$. The following lemmas which are simple applications of leaf-elimination on trees are used as subroutines.
\begin{lem}[Lemma 3.6,~\cite{Sherman13}]\label{treeflow} There is an algorithm $\mathtt{TreeFlow}$ that, given a tree $T$ and a demand vector $b$, takes $O(n)$ time and outputs for each tree edge, the flow along that edge when routing $b$ in $T$.
\end{lem}

\begin{lem}[Lemma 3.7,~\cite{Sherman13}]\label{treepot} There is an algorithm $\mathtt{TreePotential}$ that, given a tree $T$ annotated with a price $p_e$ for each edge, takes $O(n)$ time and outputs a vector of vertex potentials $v$ such that, for any $i,j$, the sum of the prices on the path from $j$ to $i$ in $T$ is $v_i - v_j$.
\end{lem}

To compute $R$, we take as input the demand vector $b$, and then annotate each forest edge $e$ with the congestion $r_e$ induced by routing $b$ through a tree containing $e$.

\begin{algorithm}
$\mathtt{Compute}R(b, L = (\lambda_i, F_i, T_i)_i^t)$:
\begin{itemize}
\item For $i = 1,\ldots,t$:
\begin{itemize}
\item Let $T$ be the tree formed by taking $F_i$, adding a new vertex $s$, and an edge from $s$ to each core-vertex of $F_i$.  Augment $b$ with demand zero to the new vertex.
\item $f \gets \mathtt{TreeFlow}(b, T)$.
\item Set $r_e \gets f_e/c_e$ for each forest edge in $F_i$.
\item Set $b'$ to a vector indexed by core-vertices, with $b'_j$ equal to the flow on the edge from $s$ to core-vertex $j$.
\item $\mathtt{ComputeR}(b', T_i)$.
\end{itemize}
\end{itemize}
\end{algorithm}

\begin{lem} [Lemma 3.8,~\cite{Sherman13}]\label{lem:38sherman13}The procedure $\mathtt{Compute}R(b, L)$ correctly annotates each edge $e$ with $r_e = (Rb)_e$, and takes $\tilde{O}(tn)$ time.
\end{lem} 

To compute $R^\top$, we assume each forest edge $e$ has been annotated with a price $p_e$ that must be paid by any flow per unit of congestion on that edge, and output potentials $v$ such that $v_i - v_j$ is the total price to be paid for routing a unit of flow from $j$ to $i$.

\begin{algorithm}
$\mathtt{Compute}R^\top(L = (\lambda_i, F_i, T_i)_i^t)$:
\begin{itemize}
\item $v \gets 0$
\item For $i = 1,\ldots,t$:
\begin{itemize}
\item $v' \gets \mathtt{Compute}R^\top(T_i)$.
\item Let $T$ be the tree formed by taking $F_i$, adding a vertex $s$, and an edge from $s$ to each core-vertex of $F_i$.  Set $q_e = p_e/c_e$ for each forest edge, and $q_e = v'_j$ for edge $e$ from $s$ to core-vertex $j$.
\item $v'' \gets \mathtt{TreePotential}(T, q)$
\item Add $v''$ to $v$ after removing the entry for $s$.
\end{itemize}
\item Return $v$
\end{itemize}
\end{algorithm}

\begin{lem} [Lemma 3.9,~\cite{Sherman13}]\label{lem:39sherman13}Given edges annotated with per-congestion prices, the procedure $\mathtt{Compute}R^\top(L)$ correctly returns potentials $v$ such that $v_k - v_j$ is the cost per unit of flow from vertex $j$ to $k$.
\end{lem} 
% \thatchaphol{State more precisely why \ref{lem:34sherman13} implies \ref{lem:det15sherman13}. For example, specify all the lemmas in Sherman'13 that are needed and say that we do not need to modify anything in those lemmas.}
Back to the proof of \Cref{lem:det15sherman13}, the construction time follows from first apply $\mathtt{sparsify}$ on the input graph and then setting $t=n^{1/k}$ in~\Cref{lem:34sherman13}. The time to apply $R$ or $R^\top$ are proved by~\Cref{lem:38sherman13} and~\Cref{lem:39sherman13}, respectively.


==> application-vertex-cut.tex <==

\subsection{Low-Expansion Vertex Cuts}

Next, we show that a fast algorithm for computing a cut with low \emph{vertex expansion}, a notion similar to conductance and sparsity.  
%
For any graph $G=(V,E)$, a vertex cut $(L,S,R)$ is a partition of
$V$ such that $L,R\neq\emptyset$ and $E_{G}(L,R)=\emptyset$. A
vertex expansion of a vertex cut $(L,S,R)$ is denoted by $h_{G}(L,S,R)=\frac{|S|}{\min\{|L|,|R|\}+|S|}$
and a vertex expansion of a graph is denoted by $h_{G}=\min_{(L,S,R)}h_{G}(L,S,R)$. We define \emph{balance} of $(L,S,R)$ as $\Bal_G(L,S,R) =\frac{\min\{|L|,|R|\}+|S|}{\max\{|L|,|R|\}+|S|}$.
 

\begin{cor}
\label{cor:vertex expansion}There is a deterministic algorithm that,
given $(G,\phi,\beta)$ where $G$ is an $m$-edge $n$-node undirected graph $G$, $\phi\in[0,1]$ is a vertex expansion parameter, and $\beta \in [0,1]$ is a balanced parameter,
in time
$O(m^{1+o(1)}/\phi)$ either 
\begin{enumerate}

\item declares there is no  vertex cut $(L,S,R)$ where  $h_{G}(L,S,R)<\phi$ and $\Bal_G(L,S,R) > \beta$, or
\item finds a vertex cut $(L,S,R)$ where $h_{G}(L,S,R)\le\phi2^{O(\log n\log\log n)^{2/3}}$ and $\Bal_G(L,S,R) \ge \beta/ 2^{O(\log n\log\log n)^{2/3}}$. 

\end{enumerate}
\end{cor}
This algorithm is a vertex expansion variant of the \textsc{MostBalance} algorithm that we will prove formally later in \ref{thm: sparse edge cut of large profit or witness}. The main difference is that our goal now is to embed an expander with small congestion on nodes instead of on edges. 
So, in each round of the cut-matching game, 
we need to solve a variant of the $\Match$ problem with small vertex congestion. This can be implemented in either $\Otil(m/\phi)$ time (based on the bounded-height push relabel or blocking flow similar the $\PushMatch$ algorithm, or in time  $\Otil(m\sqrt{n})$ (based on the deterministically vertex capacitated exact max flow algorithm by Theorem 1.4 of \cite{NanongkaiSY19}). Following the same proof of \ref{thm: sparse edge cut or expander}, we obtain the above claim.


\subsection{Vertex Versions of Max Flow, Min Cut, and Lowest-Expansion Vertex Cut }

We can also derandomize the decremental single-source shortest path ($\mathsf{SSSP}$)
algorithm by Chuzhoy and Khanna \cite{ChuzhoyK19}. \begin{cor}
There is a deterministic algorithm that, given a simple undirected
weighted $n$-node graph $G=(V,E)$ undergoing vertex deletions, a
special source vertex $s\in V$, and a parameter $\epsilon>0$, supports
queries $\mathsf{path\text{-}query}(v)$. For each query $\mathsf{path\text{-}query}(v)$,
the algorithm returns a path from $s$ to $v$, if such a path exists,
whose length is at most $(1+\epsilon)\dist(s,v)$. The total running
time of the algorithm is $O(n^{2+o(1)}\epsilon^{-2}\log^{3}(1/\epsilon)\log L)$
where $L$ is the ratio of largest to smallest edge weights, and each
query is answered in $O(n^{1+o(1)}\log L\log(1/\epsilon))$ time.
\end{cor}

\begin{proof}
By applying \ref{cor:vertex expansion} with
$\phi=1/n^{o(1)}$, we can derandomize the construction of the \emph{core
decomposition} in \cite{ChuzhoyK19} which is the only randomized
component in the whole paper.
\end{proof}
%

Chuzhoy and Khanna \cite{ChuzhoyK19} also show applications of their algorithm to computing approximate vertex max flow, min
cut, and cut with lowest vertex expansion. As the reductions are deterministic, we immediately obtain:
\begin{cor}\label{cor:vmaxflow}
There is a deterministic algorithm that, given an undirected $n$-node
graph $G=(V,E)$ with capacities $c(v)\ge0$ on vertices, a source
$s$, a sink $t$, and a parameter $\epsilon\in(0,1]$, computes a
$(1+\epsilon)$-approximate maximum $s$-$t$ flow and a $(1+\epsilon)$-approximate
minimum vertex $s$-$t$ cut in $O(n^{2+o(1)}/\poly(\epsilon))$ time.
\end{cor}

\begin{cor}\label{cor:vexpansion_ck}
There is a deterministic algorithm that, given an undirected $n$-node
graph $G=(V,E)$, computes a $O(\log^{4}n)$-approximate to the lowest
vertex expansion cut in $O(n^{2+o(1)})$ time.
\end{cor}

Note that this algorithm is incomparable to one from \ref{cor:vertex expansion}.

\begin{comment}
\subsection{Vertex Connectivity}
\begin{cor}
There is a deterministic algorithm that, given an undirected $n$-node
$m$-edge graph $G=(V,E)$ and a parameter $k<n^{1/8}$, computes
a vertex cut of size at most $k$ or determine if none exists in time
\[
\Ohat(m+\min\{n^{1.??}k^{??},n^{1.??}k^{??}\}).
\]
\end{cor}

\begin{proof}
In \cite{GaoLNPSY19}, they $n^{o(1)}$-approximate vertex expansion
in $O(m^{1.6})$ time. Here, we can do in $\Ohat(m/\phi)$ time using
\ref{cor:vertex expansion} where $\phi\gg1/\sqrt{n}$. {*}{*}Do math.
\end{proof}
%

\end{comment}

==> cut.tex <==
%!TEX root = main_det_cut.tex

\section{Cut Player's Problem Variants and Their Reductions}
\label{sec:cut}

In this section, we formally define the main problem in this paper called $\BCut$ and related problems. In \ref{sec:BCut_high_cond,sec:BCut_nophi}, we will show fast algorithms for $\BCut$ and many applications that follow from them in \ref{sec:app}. At a high level, the goal in  $\BCut$  is to either cut a balanced sparse cut, or prune (i.e. delete)  a small part
of the  input graph so that the rest forms an expander.\begin{defn}[$\Cut$ and $\BCut$]
\label{def:CP}In the $\Cut$ problem, an algorithm is given $(G,\phi_{U},\phi_{L},\beta)$
where $G=(V,E)$ is an $m$-edge graph, $\phi_{U},\phi_{L}\in[0,1]$
where $\phi_{L}\le\phi_{U}$ and $\beta\le1/3$, and returns either 
\begin{enumerate}
\item \textbf{(Cut):} \label{enu:CP cut}a cut $S\subset V$ such that $\beta\vol_{G}\le\vol_{G}(S)\le\vol_{G}/2$
and $\Phi_{G}(S)\le\phi_{U}$
\yp{$\phi_G(S)$}, or 
\item \textbf{(Prune):} \label{enu:CP prune}a cut $S\subset V$ such that
$\vol_{G}(S)\le\vol_{G}/2$, $\delta_{G}(S)\le\phi_{U}\vol_{G}$ and
$\Phi_{G-S}\ge\phi_{L}$. 
\yp{$\Phi(G - S)$}
\end{enumerate}
Let $T_{\Cut}(m,\phi_{U},\phi_{L},\beta)$ denote the worst-case time
required for deterministically solving $\Cut$ with the above parameters.
Let $\BCut$ be a problem defined in the same way as $\Cut$ 
where $\beta=1/3$ is fixed, and let $T_{\BCut}(m,\phi_{U},\phi_{L})$
be defined similarly.
\end{defn}

Below, we also state the related problems including
$\vBCut$ and $\CA$. These problems will help us highlighting
the key idea as follows. We show in this section the following rather straightforward
reductions. (Lemma numbers indicate the corresponding lemmas stated below.)
\begin{equation}
\vBCut\xrightarrow{\text{Lem~\labelcref{lem:vBCut from BCut}}}
\BCut\xrightarrow{\text{Lem~\labelcref{lem:BCut from Cut}}}
\Cut\xrightarrow{\text{Lem~\labelcref{lem:Cut from CA}}}
\CA.\label{eq:basic reduc}
\end{equation}
That is, an algorithm for $\CA$ implies the ones for $\Cut$,
$\BCut$, and $\vBCut$ respectively. Then, in \Cref{sub:CA via vBCut}
we will show the follwing main technical reduction that runs on \emph{graphs with fewer nodes}. (We use ``$\Rightarrow$'' to emphasize that the reduction produces graphs with fewer nodes.)
\[
\CA\xRightarrow{\text{Lem~\labelcref{lem:CA recursive}}}
%\Rightarrow
\vBCut
\]
%
This will imply recursive algorithms
for solving all these problems, including the main one $\BCut$. The
fact that we only need to show a reduction from $\CA$ to $\vBCut$
helps us presenting the key idea in a cleaner way.

Now, we define $\vBCut$ which is almost the same as $\BCut$ except that it concerns the sparsity and vertex-balance of a cut instead of its conductance (edge)-balance.

%This is, in fact the problem that the cut player in our cut-matching game need to solve:\danupon{I don't understand the last sentence.}

\begin{defn}[$\vBCut$]
\label{def:vCP}In the $\vBCut$ problem, an algorithm is given $(G,\phi_{U},\phi_{L})$\danupon{Should have $\delta$ too}
where $G=(V,E)$ is an $n$-node connected graph with maximum degree
$\Delta$, and $\phi_{U},\phi_{L}\in[0,1]$ where $\phi_{L}\le\phi_{U}$,
and returns either 
\begin{enumerate}
\item \textbf{(Cut):} \label{enu:vCP cut}a cut $S\subset V$ such that
$|V|/6\le|S|\le|V|/2$ and $\sigma_{G}(S)\le\phi_{U}$, or 
\item \textbf{(Prune):} \label{enu:vCP prune}a cut $S\subset V$ such that
$|S|\le|V|/2$, $\delta_{G}(S)\le\phi_{U}|V|$ and $\sigma_{G-S}\ge\phi_{L}$. 
\end{enumerate}
Let $T_{\vBCut}(n,\Delta,\phi_{U},\phi_{L})$ denote the worst-case
time required for deterministically solving $\vBCut$ with the above
parameters.
\end{defn}

Next, we define $\CA$. At a high level, the goal in  $\CA$  is to either cut a balanced sparse cut, or augment (i.e.~insert) a number of edges so that the input graph  becomes  an expander.
\begin{defn}[$\CA$]
\label{def:CA}In the $\CA$ problem, an algorithm is given $(G,\phi_{U},\phi_{L},\beta_{\cut},\beta_{\aug})$
where $G=(V,E)$ is an $m$-edge graph, $\phi_{U},\phi_{L}\in[0,1]$
where $\phi_{L}\le\phi_{U}$ and $\beta_{\cut},\beta_{\aug}\in[0,1]$, and returns either 
\begin{enumerate}
\item \textbf{(Cut):} \label{enu:CA cut}a set $S\subset V$ such that $\beta_{\cut}\vol_{G}\le\vol_{G}(S)\le\vol_{G}/2$
and $\Phi_{G}(S)\le\phi_{U}$\yp{$\phi_G(S)$}, or 
\item \textbf{(Augment):} \label{enu:CA aug}a set $F$ of edges where $|F|\le\beta_{\aug}\vol_{G}$
and $\Phi_{G\cup F}\ge\phi_{L}$.
\yp{$\Phi(G \cup F)$}
\end{enumerate}
Let $T_{\CA}(m,\phi_{U},\phi_{L},\beta_{\cut},\beta_{\aug})$ denote
the worst-case time required for deterministically solving $\CA$
with the above parameters.
\end{defn}


\subsection*{Reductions as in \labelcref{eq:basic reduc}}
%\label{subsec:basic reductions}
%\paragraph{Details of Reductions in \Cref{eq:basic reduc}.}
Below we provide details of the chain of simple reductions presented in \labelcref{eq:basic reduc}.
%We first state and prove the rightmost reduction from $\Cut$ to $\CA$. For the proof, 
To get the rightmost reduction from $\Cut$ to $\CA$, 
we use an algorithm developed in \cite{SaranurakW19,Wulff-Nilsen17,NanongkaiS17}  called $\Prune$.\danupon{New}
At a high level, suppose we are given an expander $G'=(V,E')$ and we need to delete a set of edges $D \subset E(G').  $   
So, $G\defeq G'-D$ might not be an expander anymore. $\Prune$ can ``repair'' this expander by pruning a small set $P$ of nodes from $G$ so that $G-P$ is an expander.  The  formal statement below follows from Theorem 1.3 in the paper by Saranurak and Wang \cite{SaranurakW19}.
\begin{thm}[$\Prune$ \cite{SaranurakW19}]
        \label{thm:prune}Let $c_{\Prune}$ be a large enough constant. There
        is an algorithm called $\Prune$ that take as an input a tuple $(G,D,\phi)$ where $G=(V,E)$
        is an $m$-edge graph, $D$ is a set of edges of size
        $|D|=d$, and $\phi\in[0,1]$ is such that $G'=(V,E\cup D)$ has conductance $\Phi_{G'}\ge\phi$. 
        %
        The algorithm then
        outputs a set $P\subset V$ in time 
        $$T_{\Prune}(m,d,\phi)=O(d\log m/\phi^{2})$$
        such that $\Phi_{G-P}\ge\phi/6$\yp{$\Phi(G - P)$}, $\vol_{G}(P)\le c_{\Prune}d/\phi$,
        and $\delta_{G}(P)\le c_{\Prune}d$.\footnote{In \cite{SaranurakW19} it is guaranteed that $\Phi_{G\{V-P\}}\ge\phi/6$ instead of $\Phi_{G-P}\ge\phi/6$.  Observe that the former implies the latter. We only need the latter here. (Recall that both are measures on induced subgraphs on $V-P$, but we add self-loops in $G\{V-P\}$ to preserve nodes' degrees.)}
\end{thm}


Given an algorithm for $\CA$, we combine it with $\Prune$ and immediately obtain an algorithm for $\Cut$: 


\begin{lem}[$\Cut\rightarrow\CA$]
\label{lem:Cut from CA}Let $c_{\Prune}$ be the constant from \ref{thm:prune}.
There is an algorithm for solving $\Cut$ with $6\phi_{L}\leq \phi_{U}$ such that
\begin{align*}
T_{\Cut}\left(m,\phi_{U},\phi_{L},\beta\right)&\le T_{\CA}\left(m,\phi_{U},6\phi_{L},\beta,\frac{\phi_{L}}{c_{\Prune}}\right)+T_{\Prune}\left(m,\left\lfloor\frac{2m\phi_{L}}{c_{\Prune}}\right\rfloor,6\phi_{L}\right)\\
&=T_{\CA}\left(m,\phi_{U},6\phi_{L},\beta,\frac{\phi_{L}}{c_{\Prune}}\right)
+O\left(\left(m\log m\right)/\phi_L\right).
\end{align*}
\end{lem}

\begin{proof}

        
Given an input tuple $(G,\phi_{U},\phi_{L},\beta)$ for $\Cut$,
we invoke $\CA(G,\phi_{U},6\phi_{L},\beta,\frac{\phi_{L}}{c_{\Prune}})$
in time $T_{\CA}(m,\phi_{U},6\phi_{L},\beta,\frac{\phi_{L}}{c_{\Prune}})$.
%\footnote{Since  $6\phi_{L}\leq \phi_{U}$, we satisfy the input conditions in \Cref{def:CA} for $\CA$.}
If $\CA$ returns a cut $S$, then it is clear that $S$ satisfies
the conditions of \ref{enu:CP cut} from \ref{def:CP} for $\Cut$. Otherwise,
a set $F$ is returned, where $|F|\le(\frac{\phi_{L}}{c_{\Prune}})\vol_{G}\le\frac{2m\phi_{L}}{c_{\Prune}}$
and $\Phi_{G\cup F}\ge6\phi_{L}$\yp{$\Phi(G \cup F)$}.
Then, we invoke $\Prune(G\cup F,F,6\phi_{L})$.
In time $T_{\Prune}(m,\lfloor\frac{2m\phi_{L}}{c_{\Prune}}\rfloor,6\phi_{L})$ the algorithm
returns a set $P$ where (i) $\Phi_{G-P}\ge (6\phi_L)/6$\yp{$\Phi(G - P)$?}, (ii) $\vol_{G}(P)\le\frac{c_{\Prune}|F|}{6\phi_{L}}\le\vol_{G}/6$
and (iii) $\delta_{G}(P)\le c_{\Prune}|F|\le\phi_{L}\vol_{G}\le\phi_{U}\vol_{G}$.
Hence, outputting $S=P$ gives $S$ that satisfies the conditions of \ref{enu:CP prune}
from \ref{def:CP}. (Note that since $6\phi_{L}\leq \phi_{U}\leq 1$, we satisfy the input conditions in \Cref{def:CA,thm:prune} for $\CA$ and $\Prune$, respectively.)
%
\end{proof}
%
Given an algorithm for solving $\Cut$, it is easy to obtain
the ones for $\BCut$ and $\vBCut$, respectively. The idea
is straightforward: We simply repeatedly cut the graph
until the union of all cuts is balanced (in terms of the volume or the number of nodes). The union is a sparse cut by \ref{prop:union}. To make this idea formal,
there are several cases in the analysis which are quite tedious. So,
we defer the proofs to Appendix.
\begin{lem}[$\BCut\rightarrow\Cut$]
\label{lem:BCut from Cut}There is an algorithm for $\BCut$ with $3\phi_L\leq \phi_U$ such
that
\[
T_{\BCut}(m,\phi_{U},\phi_{L})\le O(1/\beta)\cdot T_{\Cut}(m,\phi_{U}/3,\phi_{L},\beta).
\]
\end{lem}

\begin{lem}[$\vBCut\rightarrow\BCut$]
\label{lem:vBCut from BCut}There is an algorithm for $\vBCut$ with $60\Delta\phi_L\leq \phi_U$
such that
\[
T_{\vBCut}(n,\Delta,\phi_{U},\phi_{L})\le O(\Delta)\cdot T_{\BCut}(n\Delta,\phi_{U}/(60\Delta),\phi_{L}).
\]
\end{lem}




==> match.tex <==
%!TEX root = main_det_cut.tex

\section{Matching Player's Problem and Algorithms}
\label{sec:match}
In this section, we give the definition of the $\Match$ problem that the \emph{matching player} in our (variant of) \emph{cut-matching game} needs to solve. 
The matching player in previous works that are based on the cut-matching game \cite{KhandekarRV09,KhandekarKOV2007cut,OrecchiaSVV08,SaranurakW19} also implicitly solves this problem but only when $k=1$:
\begin{defn}[$\Match$]
\label{def:CM}In the $\Match$ problem, the input is $(G,\phi,\cong,\beta,\{A_{1},B_{1},\dots,A_{k},B_{k}\})$
where $G=(V,E)$ is an $n$-node graph with maximum degree at most
$20$, $\phi\in[0,1]$ is a conductance parameter, $\cong\ge1$ is
a congestion parameter, $\beta\in[0,1]$ is a balance parameter, and
$A_{1},B_{1},\dots,A_{k},B_{k}$ are disjoint subsets of $V$ where
$|A_{i}|=|B_{i}|$ %\ge n/2k$ Thatchaphol: this is not neeeded anywhere.
for each $i$, and $T=A_{1}\cup B_{1}\cup\dots\cup A_{k}\cup B_{k}$
is called the set of \emph{terminals}, and returns either 
\begin{enumerate}
\item \textbf{(Cut):} \label{enu:CM cut}a cut $S$ where $\beta\vol_{G}/160\le\vol_{G}(S)\le\vol_{G}/2$
and $\Phi_{G}(S)\le\phi_{}$
\yp{$\phi_G(S)$?}, or 
\item \textbf{(Match):} \label{enu:CM match}a collection $\P$ of paths
connecting $u\in A_{i}$ to $v\in B_{i}$ such that each terminal
is an endpoint of exactly one path, except at most $\beta n$ many
terminals which are not an endpoint of any path, and every edge is
contained in at most $\cong$ paths.
\end{enumerate}
For $1\le i\le k$, let $M_{i}=\{(u,v)\mid u\in A_{i}$ and $v\in B_{i}$
are the two endpoint of a path in $\P\}$. Note that $M_{i}$ is a matching
(which might not be a subgraph of $G$) and $|T-\cup_{i=1}^{k}V(M_{i})|\le\beta n$.
When a $\Match$ algorithm returns \ref{enu:CM match}, it is required to also
return $M_{1},\dots,M_{k}$. Let $T_{\Match}(n,k,\phi,\cong,\beta)$
denote the worst-case time required for deterministically solving $\Match$ with the
above parameters.
\end{defn}

It will be clear later that our algorithms for $\Match$ can be extended
to work with general graphs, instead of only constant degree graphs.
However, this does not fit quite well with the rest of our framework.
Therefore, \ref{def:CM} is stated only for constant degree graphs. 
%
Also note that $\cong$ can be thought of as a congestion guarantee that is different for each $\Match$ algorithm. We treat it as an input here, since this makes results more convenient to state and use.  

The main goal of this section is to show two algorithms for solving the $\Match$ problem. The first one works for any parameter $k \ge1$ which is crucial in our main recursive algorithm in \ref{sub:CA via vBCut}.

\begin{thm}[$\ESMatch$ Algorithm]
\label{thm:ES match}Let $c_{\match}$ be a large enough constant.
There is an algorithm called $\ESMatch$ for solving the $\Match$ problem
that, for any $(n,k,\phi,\cong,\beta)$ where 
\[
\cong\ge c_{\match}\phi^{-2}\log^{2}n,
\]
has running time $T_{\Match}(n,k,\phi,\cong,\beta)=O(nk(\log^{3}n)/\phi^{3})$.
\end{thm}

When $k=1$, we also show an algorithm which is faster and has less
restricted lower bound on $\cong$. To obtain our  main result in \ref{thm:BCut general}, using  the following $\PushMatch$ algorithm instead of $\ESMatch$  improves both the approximation and  running time.  

\begin{thm}[$\PushMatch$ Algorithm]
\label{thm:push match}
%Let $c'_{\match}$ be a large enough constant.\danupon{New}
There is an algorithm called $\PushMatch$ for solving the $\Match$ problem
that, for any $(n,k,\phi,\cong,\beta)$ where $k=1$ and
\[
\cong\ge 4\phi^{-1}
\]
has running time $T_{\Match}(n,1,\phi,\cong,\beta)=O(n\phi^{-1}\log n)$.
\end{thm}

\subsection{An Algorithm for $k\ge1$ (Proof of \Cref{thm:ES match})}
\label{sec:match k large}
In section, we prove \ref{thm:ES match}. The idea of the proof is
based on using Even-Shiloach trees (ES-trees) \cite{EvenS} for either
finding a sparse cut or listing many disjoint paths connecting the sets $A_i$
and $B_i$ of terminals. This idea was used first by Chuzhoy and
Khanna \cite{ChuzhoyK19}. We slightly extend it to work with $k$
pairs of terminal sets $\{(A_{1},B_{1}),\dots(A_{k},B_{k})\}$ by
working with $k$ many ES-trees.

Before describing  the $\ESMatch$ algorithm itself, we start with the following
simple algorithm for finding sparse cuts that separates two sets $A$
and $B$ that are far away. For any two sets $A,B \subset V$ in $G=(V,E)$, we denote by $\dist_G(A,B)$ the minimum distance between any two nodes $u \in A$ and $v\in B$.
\begin{lem}[$\SingleAB$ Algorithm]
\label{lem:SingleABCut}There is an algorithm called $\SingleAB$ that, given
$(G,(A,B))$ where $G=(V,E)$ is an $m$-edge graph and $A,B\subset V$
are two disjoint subsets, returns in $O(m)$ time a cut $S$ where
$\Phi_{G}(S)\le\frac{10\log m}{\dist_{G}(A,B)}$
\yp{$\phi_G(S)$?}, $\vol_{G}(S)\le\vol_{G}/2$,
and $S$ separates $A$ from $B$ (i.e. either ($A\subseteq S$ and
$B\cap S=\emptyset$) or ($B\subseteq S$ and $A\cap S=\emptyset$)).
\end{lem}

\begin{proof}
For any set $X\subset V$ and a number $r$, let $\ball(X,r)$ denote
the set of all nodes within distance at most $r$ from $X$. Let $L=\dist_{G}(A,B)$.
We can assume that $L\geq 10\log m$; otherwise the lemma holds trivially.
Observe that $\ball(A,L/3)$ and $\ball(B,L/3)$ are disjoint. The
algorithm is to simply perform breadth-first search from $A$ and
$B$ and compute $\ball(A,r)$ and $\ball(B,r)$ for all $r\le L/3$.
This can be done in $O(m)$ time. 

We assume w.l.o.g.\ that $\vol_{G}(\ball(A,L/3))\le\vol_{G}/2$. It
suffices to prove that there is some $i\le L/3$ such that $\Phi_{G}(\textsc{Ball}(A,i))\leq\frac{10\log m}{L}$
\yp{$\phi_G(...)$}.
Suppose otherwise for a contradiction. Then, for every $i\le L/3$, 
%$$\vol_{G}(\ball(A,i+1))\ge(1+\frac{10\log n}{L})\vol_{G}(\ball(A,i)).$$
$$\vol_{G}(\ball(A,i+1))\ge(1+\frac{10\log m}{L})\vol_{G}(\ball(A,i)).$$
This is because the conductance of $\ball(A,i)$ is $\frac{\vol_{G}(\ball(A,i+1))-\vol_{G}(\ball(A,i))}{\vol_{G}(\ball(A,i))}$, which is assumed to be at least $\frac{10\log m}{L}$.
%
So 
$$\vol_{G}(\ball(A,L/3))\ge(1+\frac{10\log m}{L})^{L/3}>\vol_{G}$$
which is a contradiction (since $L\geq 10\log m$; note that the logarithmic is to base two).
\end{proof}
Next, we slightly extend $\SingleAB$ to work with $k$
pairs of $(A_{1},B_{1}),\ldots,(A_{k},B_{k})$. This algorithm returns
a sparse cut if the distance between $A_{i}$ and $B_{i}$ is large
for every $i$.
\begin{lem}[$\ManyAB$ Algorithm]
\label{lem:ManyABCut}There is an algorithm called $\ManyAB$ that, given an
$m$-edge graph $G=(V,E)$ and disjoint sets $A_{1},B_{1},\ldots,A_{k},B_{k}\subset V$
where $L=\min_{i}\{\dist_{G}(A_{i},B_{i})\}$ and $\nu=\sum_{i=1}^{k}\min\{\vol_{G}(A_{i}),\vol_{G}(B_{i})\}$,
returns in $O(km)$ time a cut $S$ where $\Phi_{G}(S)\le\frac{30\log m}{L}$\yp{$\phi_G(S)$}
and $\nu/2\le\vol_{G}(S)\le\vol_{G}/2$. 
\end{lem}

\begin{proof}
See \ref{alg:ManyABCut} for the description of the algorithm. We assume that $L\geq 30\log m$; otherwise the lemma trivially holds.
%Let $L=\min_{i}\{\dist_{G}(A_{i},B_{i})\}$ and $\nu=\sum_{i=1}^{k}\min\{\vol_{G}(A_{i}),\vol_{G}(B_{i})\}$.
Obviously, $$\vol_{G}(S)\le\vol_{G}/2$$ 
since we always return the set of smaller volume among $\Shat$ and $V-\Shat$. 
%regardless of whether $S$ is returned as in \Cref{item:returnCase2} or \Cref{item:returnCase1}. 
Observe that, before the cut $S$ is returned, we have that $\Shat=\cup_{i=1}^{k'}S_{i}$
where $k'\le k$. By \ref{lem:SingleABCut}, $\frac{\delta_{\Ghat_{i}}(S_{i})}{\vol_{\Ghat_{i}}(S_{i})}\le\frac{10\log m}{L}$
where $\Ghat_{i}$ is the graph $\Ghat$ before removing $S_{i}$.
By \ref{prop:union}, we have that \
% OLD: $$\frac{\delta_{G}(S)}{\vol_{G}(S)}\le\frac{10\log m}{L}.$$
$$\frac{\delta_{G}(\Shat)}{\vol_{G}(\Shat)}\le\frac{10\log m}{L}.$$
%Now, there are two cases.

{\bf Case 1.} If we return $S=\Shat$ as in \Cref{item:returnCase1} of \Cref{alg:ManyABCut}, then we have $\vol_{G}(\Shat)\le\vol_{G}/2$.
%
%If $k'=k$, then $S=\Shat$\danupon{Why?}, and we have $\vol_{G}(S)\le\vol_{G}/2$.
%So $\Phi_{G}(S)=\frac{\delta_{G}(S)}{\vol_{G}(S)}\le\frac{10\log m}{L}.$
So $\Phi_{G}(S)=\frac{\delta_{G}(\Shat)}{\vol_{G}(\Shat)}\le\frac{10\log m}{L}.$
Observe we have separated $A_{i}$ and $B_{i}$ by removing the set
$S_{i}$ returned by \ref{lem:SingleABCut} for all $i$. So, in the
final graph $\Ghat$,  either $V(\Ghat)\cap A_{i}=\emptyset$
or $V(\Ghat)\cap B_{i}=\emptyset$ for every $i$. In other words, either $S\supseteq A_{i}$ or
$S\supseteq B_{i}$, for every $i$. So $\vol_{G}(S)\ge\nu\ge\nu/2$. 

{\bf Case 2.} If we return $S=V-\Shat$ as in \Cref{item:returnCase2}  of \Cref{alg:ManyABCut}, 
%If $k'<k$, then $S=V-\Shat$ and 
%then we have $\vol_{G}(S)\le\vol_{G}/2$.
%Let 
then let $S'=\cup_{i=1}^{k'-1}S_{i}$. \jl{\textbackslash bigcup or \textbackslash cup for inline equations?} We have $\vol_{G}(S')\le\vol_{G}/2$
and $\vol_{\Ghat}(S_{k'})\le\vol_{\Ghat}/2=\vol_{G}(V-S')/2$. So
$$\vol_{G}(\Shat)=\vol_{G}(S')+\vol_{\Ghat}(S_{k'})\le3\vol_{G}/4.$$
(The above use the fact that modifying $G$ to $G\{V-\Shat\}$ does not change nodes' degrees.)
It follows that $\vol_{G}(S)\ge\vol_{G}/4\ge\nu/2$, and
%Since $\vol_{G}(V-S)\le3\vol_G(S)$,
$\vol_{G}(\Shat)\le3\vol_G(S)$. 
The latter implies that 
\[%\pushQED{\qed} 
\Phi_{G}(S)\le3\cdot\frac{\delta_{G}(S)}{\vol_{G}(S)}\le\frac{30\log m}{L}.\qedhere
%\popQED
\] 
\end{proof}
\begin{algorithm}
\underline{Input}: An $m$-edge graph $G=(V,E)$ and disjoint sets
$A_{1},B_{1},\ldots,A_{k},B_{k}\subset V$. 

\underline{Output}: A cut $S$ such that $\nu/2\le\vol_{G}(S)\le\vol_{G}/2$
and $\Phi_{G}(S)\le\frac{30\log m}{L}$ \yp{$\phi_G(S)$}where $L=\min_{i}\{\dist_{G}(A_{i},B_{i})\}$
and $\nu=\sum_{i=1}^{k}\min\{\vol_{G}(A_{i}),\vol_{G}(B_{i})\}$.

\underline{Algorithm}: 
\begin{enumerate}[noitemsep]
\item Initialize $\Shat\leftarrow\emptyset$, $i\gets1$ and $\Ghat\gets G$.
\item For $i=1,\dots,k$: 
\begin{enumerate}[noitemsep]
\item $S_{i}\leftarrow\SingleAB(\Ghat,(V(\Ghat)\cap A_{i},V(\Ghat)\cap B_{i})$
(by \ref{lem:SingleABCut}).
\item $\Ghat\gets\Ghat\{V-S_{i}\}$. 
\item $\Shat\leftarrow\Shat\cup S_{i}$.
%\item $\Shat\leftarrow\Shat\cup S_{i}$.  
%\item $\Ghat\gets\Ghat\{V-\Shat\}$.\danupon{I changed the algorithm description a bit. The old one is incorrect.}
\item \label{item:returnCase2} If $\vol_{G}(S)\ge\vol_{G}/2$, return $S=V-\Shat$. 
\end{enumerate}
\item \label{item:returnCase1}Return $S=\Shat$. 
\end{enumerate}
\caption{\label{alg:ManyABCut}$\protect\ManyAB(G,\{(A_{1},B_{1}),\ldots,(A_{k},B_{k})\})$ // For \Cref{lem:ManyABCut}}

\end{algorithm}

Finally, we describe the $\ESMatch$ algorithm for $\Match$
in \ref{alg:ESMatch}. We show the correctness and
analyze the running time below.

\begin{algorithm}
The input and output are as defined in \Cref{def:CM}, namely:

\underline{Input}: %As in \Cref{def:CM}, 
An $n$-node graph $G$ with maximum degree $20$,
a conductance parameter $\phi\in[0,1]$, a congestion parameter $\cong\ge1$,
a balance parameter $\beta\in[0,1]$, and  disjoint subsets $A_{1},B_{1},\dots,A_{k},B_{k}$ of $V$.
% where $|A_{i}|=|B_{i}|$ forevery $i$.

\underline{Input Conditions}: (i) $\cong\ge c_{\match}\phi^{-2}\log^{2}n$
for large enough constant $c_{\match}$. (ii) $\forall i: |A_{i}|=|B_{i}|$. 
%for every $i$.

\underline{Output}:  %As in \Cref{def:CM}, 
Let $T=A_{1}\cup B_{1}\cup\dots\cup A_{k}\cup B_{k}$
be the set of \emph{terminals}. The algorithm returns either 
\begin{enumerate}[noitemsep,nolistsep]
\item a cut $S$ where $\beta\vol_{G}/160\le\vol_{G}(S)\le\vol_{G}/2$ and
$\Phi_{G}(S)\le\phi$, or 
\item a collection $\P$ of paths connecting $u\in A_{i}$ to $v\in B_{i}$
such that each terminal is an endpoint of exactly one path, except
at most $\beta n$ many terminals which are not an endpoint of any
path, and every edge is contained in at most $\cong$ paths.
\end{enumerate}
\underline{Algorithm}: 
\begin{enumerate}[noitemsep]
\item Set the length parameter $L\leftarrow120\phi^{-1}\log m$.
\item Initialize $\Ahat_{i}\leftarrow A_{i}$, $\Bhat_{i}\leftarrow B_{i}$
for all $i$. Below, we maintain $\That=\cup_{i=1}^{k}(\Ahat_{i}\cup\Bhat_{i})$
as the ``current'' terminal set.
\item \label{enu:Match loop}Repeat until $|\That|<\beta n$: 
\begin{enumerate}[noitemsep]
\item Set $\Ghat\leftarrow G$. 
\item \label{enu:ES-tree}While there is a path $P$ of length at most $L$ connecting
nodes between $\Ahat_{i}$ and $\Bhat_{i}$ for some $i$:
\begin{enumerate}
\item Add $P$ to $\P$. 
\item Remove the two endpoints of $P$ from $\Ahat_{i}$ and $\Bhat_{i}$. 
\item Delete edges in $P$ from $\Ghat$. 
\end{enumerate}
\item If fewer than $\phi|\That|/24L$ paths are added to $\P$ in this
iteration: \label{line:ProgressLowerBound} 
\begin{enumerate}
\item $\Shat\gets\ManyAB(\Ghat,\{(\Ahat_{1},\Bhat_{1}),(\Ahat_{2},\Bhat_{2}),\ldots(\Ahat_{k},\Bhat_{k})\}\}$
(by \ref{lem:ManyABCut}). 
\item \label{item:ESMatch:return_cut} Return $S=\Shat$ if $\vol_{G}(\Shat)\le\vol_{G}/2$, otherwise return
$S=V-\Shat$.
\end{enumerate}
\end{enumerate}
\item  \label{item:ESMatch:return_paths} Return $\P$.
\end{enumerate}
\caption{\label{alg:ESMatch}$\protect\ESMatch(G,\phi,\cong,\beta,\{A_{1},B_{1},\dots,A_{k},B_{k}\})$ //For
\ref{def:CM,thm:ES match}}

\end{algorithm}


\paragraph{Correctness of $\ESMatch$.}
First, observe that there are at most 
$$
r
=O\left(\frac{L\log n}{\phi}\right)
=O\left(\frac{\log^{2}n}{\phi^{2}}\right)
$$
iterations in the repeat loop of \ref{alg:ESMatch}. This is because
as long as the condition on \ref{line:ProgressLowerBound} in  \ref{alg:ESMatch} is not
true, we remove at least $\Omega(\phi/L)$ fraction of nodes from
$\That$ in each iteration. Now, we prove the output satisfies the
conditions of the problem.

\underline{Case 1} Suppose that a collection $\P$ of paths is returned (from \Cref{item:ESMatch:return_paths}). It is clear
that each terminal is an endpoint of at most one path $P$, because
when $P$ is added into $\P$ we immediately remove the endpoints of
$P$ from $\That$. As we have $|\That|<\beta n$, this just means
there are at most $\beta n$ many terminals which are not an endpoint
of any path. Also every edge is contained in at most $r=O(\frac{\log^{2}n}{\phi^{2}})\le\cong$
paths, because all paths added to $\P$ in the same iterations are
disjoint and $\cong$ is required to be at least $c_{\match}\frac{\log^{2}n}{\phi^{2}}$ for a large enough constant $c_{\match}$. 
Thus, $\P$ satisfies the output conditions. 

\underline{Case 2} Suppose that a cut $S$ is returned (from \Cref{item:ESMatch:return_cut}). Let $\Ghat$ be the graph before
$\textsc{\ensuremath{\ManyAB}}$ is called and $\Shat$ be the cut
returned. We will be done after showing that 
\begin{align}
 \beta\vol_{G}/160\le\vol_{G}(S)\le\vol_{G}/2  \quad \mbox{   and   } \quad \Phi_{G}(S)\le\phi.\label{eq:ESMatch:Goal2}
%\Phi_{G}(S)&\le\phi\label{eq:ESMatch:Goal3}
\end{align}
\yp{$\phi_G(S)$}

\underline{First inequality of \labelcref{eq:ESMatch:Goal2}} 
%It suffices to show that 
%\begin{align}
%\vol_{\Ghat}(\Shat)&\ge xxx
%\end{align} 
%
%To prove the first inequality, 
By \ref{lem:ManyABCut} we have 
\begin{align}
\vol_{\Ghat}/2\ge\vol_{\Ghat}(\Shat)\ge\nu/2,\label{eq:ESMatch:ShatVolBounds}
\end{align}
where $\nu=\sum_{i=1}^{k}\min\{\vol_{\Ghat}(\Ahat_{i}),\vol_{\Ghat}(\Bhat_{i})\}$.
%
It follows from the first inequality in \Cref{eq:ESMatch:ShatVolBounds} that 
\begin{align}
\vol_{\Ghat}(\Shat)\leq \vol_{\Ghat}/2\le \vol_{\Ghat}(V-\Shat).\label{eq:ESMatch:volGhatBound}
\end{align}

Additionally, we can bound $\nu$ as follows.
\begin{align}
\nu & \ge\sum_{i=1}^{k}\min\{|\Ahat_{i}|,|\Bhat_{i}|\}=\sum_{i=1}^{k}|\Ahat_{i}| & (|\Ahat_{i}|=|\Bhat_{i}|\text{ is maintained})\nonumber\\
& =|\That|/2
%\mbox{($|\That|\geq \beta n$ when we start the iteration and we remove at most $\phi|\That|/(24L)$ paths during the iteration)}\\
\ge\beta n/4 &\mbox{($|\That|\geq \beta n-\phi|\That|/(24L)$ so $|\That|\geq \beta n/2$)}\label{eq:ESMatch:BoundThat}\\
&\ge\beta\vol_{G}/80 & (G\text{ has maximum degree }20).\label{eq:ESMatch:nuBound}
\end{align}
%where \Cref{eq:ESMatch:BoundThat} 
%%
%Combining the above with \Cref{eq:ESMatch:ShatVolBounds}, we have 
%\begin{align}
%\vol_{\Ghat}(\Shat)\ge \beta\vol_{G}/160.\label{eq:ESMatch:ShatBound}
%\end{align}
If the algorithm returns $S=\Shat$ in \Cref{item:ESMatch:return_cut}, we have 
$$\vol_G(S)=\vol_G(\Shat)\geq \vol_{\Ghat}(\Shat)\stackrel{\labelcref{eq:ESMatch:ShatVolBounds}}{\ge} \nu/2 \stackrel{\labelcref{eq:ESMatch:nuBound}}{\ge}\beta\vol_{G}/160.$$
%\stackrel{\labelcref{eq:ESMatch:ShatBound}}{\ge} \beta\vol_{G}/160.$$ 
Thus, the first inequality of \Cref{eq:ESMatch:Goal2} holds. 
%
Similarly, if the algorithm returns  $S=V-\Shat$, we have 
$$\vol_G(S)=\vol_G(V-\Shat)\geq \vol_{\Ghat}(V-\Shat)\stackrel{\labelcref{eq:ESMatch:volGhatBound}}{\ge}\vol_{\Ghat}(\Shat)\stackrel{\labelcref{eq:ESMatch:ShatVolBounds}}{\ge} \nu/2 \stackrel{\labelcref{eq:ESMatch:nuBound}}{\ge}\beta\vol_{G}/160.$$
%\stackrel{\labelcref{eq:ESMatch:ShatBound}}{\ge} \beta\vol_{G}/160;$$ 
%where %``$\stackrel{\footnotesize(*)}{\ge}$'' 
%$(*)$ above is because, by \Cref{eq:ESMatch:ShatVolBounds}, 
%%, by \ref{lem:ManyABCut},
%\begin{align}
%\vol_{\Ghat}(\Shat)\leq \vol_{\Ghat}/2\le \vol_{\Ghat}(V-\Shat).\label{eq:ESMatch:volGhatBound}
%\end{align}

\underline{Second inequality of \labelcref{eq:ESMatch:Goal2}} As we set $S=\Shat$ if $\vol_{G}(\Shat)\le\vol_{G}/2$ and otherwise set $S=V-\Shat$, we have $\vol_{G}(S)\le\vol_{G}/2$. 

\underline{Third inequality of \labelcref{eq:ESMatch:Goal2}} Let $\P'$ be the set of paths added into $\P$ in this iteration. Let $E'=\cup_{P\in\P'}P$
be a set of edges in such paths. As the condition in \ref{line:ProgressLowerBound} in  \ref{alg:ESMatch} holds, we have $|\P'|\le \phi|\That|/(24L)$; thus
\begin{align}
|E'|\le L\cdot|\P'|<\phi|\That|/24\stackrel{\labelcref{eq:ESMatch:BoundThat}}{\le} \phi \nu/12
\stackrel{\labelcref{eq:ESMatch:ShatVolBounds}}{\le}\phi\vol_{\Ghat}(\Shat)/6.\label{eq:ESMatch:EpBound}
\end{align}
% **** INEQUALITY BELOW IS TRUE BUT WE DON'T NEED IT
%So, 
%\begin{align}
%\vol_{G}(\Shat) & \le\vol_{\Ghat}(\Shat)+2|E'| \stackrel{\labelcref{eq:ESMatch:EpBound}}{\le}4\vol_{\Ghat}(\Shat)/3 \stackrel{\labelcref{eq:ESMatch:ShatVolBounds}}{\le}2\vol_{\Ghat}/3\le2\vol_{G}/3; \mbox{in particular, }\label{eq:ESMatch:volShatBound}
%\end{align}
Note that
\begin{align}
\Phi_{\Ghat}(\Shat)&\le\frac{30\log m}{L} & \mbox{(since $\min_{i}\{\dist_{\Ghat}(\Ahat_{i},\Bhat_{i})\}>L$ and by \ref{lem:ManyABCut})}\nonumber\\
&=\phi_{}/4.\label{eq:ESMatch:PhiBound}
% &\mbox{()}.
\end{align}
%$\Phi_{\Ghat}(\Shat)\le\frac{30\log m}{L}\le\phi_{}/4$ by
%\ref{lem:ManyABCut}.
Thus
%\begin{align*}
%\delta_{G}(\Shat) & \le|E'|+\delta_{\Ghat}(\Shat) \stackrel{\labelcref{eq:ESMatch:EpBound},\labelcref{eq:ESMatch:PhiBound}}{\le}\phi\vol_{\Ghat}(\Shat)/6+\phi\vol_{\Ghat}(\Shat)/4 
% \le\phi\vol_{G}(\Shat)/2.
%\end{align*}
\begin{align}
\delta_{G}(\Shat) & \le|E'|+\delta_{\Ghat}(\Shat)\nonumber\\
& \le\phi\vol_{\Ghat}(\Shat)/6+\phi\vol_{\Ghat}(\Shat)/4 &\mbox{(by \Cref{eq:ESMatch:EpBound,eq:ESMatch:PhiBound})}\nonumber\\
& \le\phi\vol_{\Ghat}(\Shat) \label{eq:ESMatch:boundDelta1}\\
&\leq \phi\vol_{\Ghat}(V-\Shat) &\mbox{(by \Cref{eq:ESMatch:volGhatBound})}\label{eq:ESMatch:boundDelta2}
%&\stackrel{\labelcref{eq:ESMatch:volGhatBound}}{\leq} \phi\vol_{\Ghat}(V-\Shat)/2 
\end{align}
The last two inequality implies that 
$$\delta_{G}(\Shat)\stackrel{\labelcref{eq:ESMatch:boundDelta1},\labelcref{eq:ESMatch:boundDelta2}}{\leq} \phi\cdot {\min\{\vol_{\Ghat}(\Shat),\vol_{\Ghat}(V-\Shat)\}}\leq \phi\cdot {\min\{\vol_{G}(\Shat),\vol_{G}(V-\Shat)\}}.$$ 
So, 
$\Phi_{G}(S)=\frac{\delta_{G}(\Shat)}{\min\{\vol_{G}(\Shat),\vol_{G}(V-\Shat)\}}\le\phi.$
%
This completes the correctness.\danupon{To do: A super clean version can use smaller $L$ (e.g. $60XXX$ instead of $120XXX$). This only affects \Cref{eq:ESMatch:PhiBound}.}

\paragraph{Running time of $\ESMatch$.}

We start with the following key lemma for the running time.
\begin{lem}
\ref{enu:ES-tree} of \ref{alg:ESMatch} can be implemented in $O(kmL)$
time.
\end{lem}

\begin{proof}
For each $1 \le i \le k$, we create an auxiliary graph $\Ghat_i$ from $\Ghat$ as follows. We add a source node $s_{i}$ and edges $(s_{i},a)$ for all $a\in \Ahat_i$ and we add a sink node $t_{i}$ into $\Ghat$ and edges $(b,t_{i})$ for all $b\in\Bhat_{i}$. Whenever $\Ghat,\Ahat_i,\Bhat_i$ are updated, we will update $\Ghat_i$ accordingly. 
Observe that $\Ghat_i$ will undergo only edge deletions. Now, we initialize the following \emph{Even-Shiloach Tree (ES-tree) data structure}. 

\begin{lem}[\cite{EvenS}]
        There is a deterministic data structure called ES-tree that, given an unweighted undirected graph $G$ undergoing edge deletions, a root node $s$, and a depth parameter $D$, maintains, for every node $v$ a value $\delta(s,v)$ such that $\delta(s,v) = \dist_G (s,v)$ if $\dist_G (s,v) \le D$ and $\delta(s,v) = \infty$ otherwise. It has a total update time of $O(mD+n)$. During the updates, it can also report a shortest $sv$-path $P$ in $O(|P|)$ time. 
\end{lem}       

%\danupon{The above might be a bit redundant with below (but not much).}

Note that there are many algorithms that have faster total update time then that of the ES-tree (e.g. \cite{HenzingerKN18-DecrementalSSSP,BernsteinC16,ChuzhoyK19,HenzingerKN16-SICOMP,HenzingerKN14_stoc,BernsteinR11,HenzingerKN14,Bernstein17}), but we cannot use any of them because they are either randomized or can return only distance (not the path).
Moreover, since we are only interested in short length paths (small $D$), a total update time improvement would not benefit us much anyway.
% Thatchaphol: I remove this list of papers because we cannot use any of these randomized algorithms.
%

We use the ES-tree to maintain a BSF tree $\cT_{i}$ rooted at $s_{i}$ of depth $L+2$
in $\Ghat_i$ undergoing edge deletions. It takes $O(mL)$ total update time.
Therefore, the total time for maintaining all $\cT_{i}$ is $O(kmL)$.
%
The ES-tree data structure can also report whenever the depth of $t_{i}$
in $\cT_{i}$ is more than $L+2$. Note that $\dist_{\Ghat}(\Ahat_{i},\Bhat_{i})\le L$
iff the depth of $t_{i}$ in $\cT_{i}$ is at most $L+2$. So as long
as $\dist_{\Ghat}(\Ahat_{i},\Bhat_{i})\le L$, we can obtain a path
$P$ of length at most $L$ from $\Ahat_{i}$ to $\Bhat_{i}$ in time
$O(|P|)$ by cutting the path from $s_{i}$ to $t_{i}$ in $\cT_{i}$.
Therefore, the total time for returning all such paths is $O(m)$.
\end{proof}
As there are $O(\frac{\log^{2}n}{\phi^{2}})$ iterations, the total
running time on \ref{enu:ES-tree} is $O(kmL)\cdot O(\frac{\log^{2}n}{\phi^{2}})=O(km\cdot\frac{\log^{3}n}{\phi^{3}})$.
The running time spent on $\ManyAB$ is  $O(km)$ by
\ref{lem:ManyABCut}. So the total running time of \ref{alg:ESMatch}
is $O(km\cdot\frac{\log^{3}n}{\phi^{3}})=\tilde{O}(kn/\phi^{3})$. (Recall that the maximum degree of $G$ is 20.)

\subsection{An Improved Algorithm for $k=1$ (Proof of \Cref{thm:push match})}
\label{sec:match k one}


\ref{thm:push match} is an easy application of either the \emph{bounded
height} variant of the push-relabel-based max flow algorithm by Henzinger
Rao and Wang \cite{HenzingerRW17} or the \emph{bounded height} variant of
the blocking-flow-based algorithms by Orrecchia and Zhu \cite{OrecchiaZ14}.\footnote{Both algorithms are designed to have \emph{local} running time, i.e.
they do not need to read the whole graph. However, we do not need
this important property to prove \ref{thm:push match}.} Note that this algorithm helps in improving the approximation ratio of our main result. Most of our applications (e.g. dynamic connectivity) still hold without using this algorithm.



\paragraph{High-Level Ideas.}
Both push-relabel and blocking flow algorithms try
to route flow from sources to sinks as much as possible while maintaining a \emph{level}
$\ell(u)\ge0$ on each node $u$. In the standard variants \cite{GoldbergT88,dinic1970algorithm},
levels can be as large as $O(n)$, the running time is $O(mn)$,
and the algorithm either returns a flow satisfying the demand or return
a cut which certifies that there is no feasible flow (this corresponds
to returning the exact max flow and min cut).

In the bounded height variant, the levels are bounded to be at most
$h$ where $h$ is a parameter. This immediately speeds up the running time to $O(mh)$. However,
even if there exists a flow satisfying the demand, the algorithm might
not return it because it stops early. Fortunately, even when the algorithm
does not return a feasible flow, using a ball growing argument, one
can show that there must exist a level cut $S_{i}=\{u\mid\ell(u)\ge i\}$
for some $i$ such that the conductance $\Phi_{G}(S_{i})\le O(\log m/h)$\yp{$\phi_G(S_{i})$}.
To summarize, we can speed up the algorithm significantly if the goal is to either return a flow satisfying the demand
or return a sparse cut. 

To take care of balancedness of a cut, we
can extend the argument above and show that, given a parameter $x$, the
algorithm either flow satisfying the demand except for $x$ many units
or return a sparse cut volume at least $\sim x$. To prove \ref{thm:push match},
we just set each node in $A$ as a source of $1$ unit and each node
in $B$ as a sink of $1$ unit, and set $h=O(\log m/\phi)$ and $x=\Theta(\beta n)$
and invoke either the algorithms by \cite{HenzingerRW17} or \cite{OrecchiaZ14}. 

\danupon{Can we shorten the above? I feel that it's vague and a bit too long for something vague}

\paragraph{Preliminaries.}
Now, we introduce definitions so that we can formally invoke the known
algorithms above which is formally stated in \ref{lem:unitflow}.
We follow the notations from \cite{SaranurakW19}. Given an unweighted
undirected graph $G=(V,E)$, let $\Delta:V\rightarrow\mathbb{Z}_{\ge0}$
denote a \emph{source function} and $T:V\rightarrow\mathbb{Z}_{\ge0}$
denote a \emph{sink function}. We use \emph{mass} to refer to the
substance being routed. For a node $v$, $\Delta(v)$ specifies the
amount of mass initially placed on $v$, and $T(v)$ specifies the
capacity of $v$ as a sink. We require that $\sum_{u}\Delta(u)\le\sum_{u}T(u)$,
i.e. the total amount of mass to be routed is at most the total capacity
of sinks. 

A \emph{routing} $f:V\times V\rightarrow\mathbb{R}$ satisfies $f(u,v)=-f(v,u)$ 
and $f(u,v)=0$ for $(u,v)\notin E$. $f(u,v)>0$ means that mass
is routed in the direction from $u$ to $v$. A \emph{congestion}
of $f$ is $\max_{e\in E}|f(e)|$. We say that $f$ is a \emph{preflow
}if $|f(e)|\le1$ for each $e\in E$ and $\sum_{u}f(v,u)\le\Delta(v)$
for each $v$ (i.e. the net amount of mass routed away from a node
can be at most the amount of its initial mass). We also treat $f$
as a function on vertices, where $f(v)=\Delta(v)+\sum_{u}f(u,v)$
is the amount of mass ending at $v$ after the routing $f$. We define
the \emph{absorbed mass} on a node $v$ as $\ab_{f}(v)=\min(f(v),T(v))$
and the excess on $v$ is $\ex_{f}(v)=f(v)-\ab_f(v)$
which measure the
amount of flow on $v$ which cannot be absorbed.
Note that if $\ex_{f}(v)=0$
for all $v$, then all the mass are successfully routed to sinks.
Let $|\ex_{f}(\cdot)|=\sum_{v}\ex_{f}(v)$ denote the total amount
of mass which is not successfully routed.

Below, we formulate a lemma that is easy to use for us, which can
be derived from Theorem 3.3 in \cite{NanongkaiSW17} (or Theorem 3.1
in \cite{HenzingerRW17}) by  substituting some parameters.
\begin{lem}
\label{lem:unitflow}There is a deterministic algorithm called $\BoundPush$ that
takes as an input a tuple $(G,\Delta,T,\phi)$ where $G=(V,E)$ is an $m$-edge graph,
$\Delta$ is a source function such that $\Delta(u)\le \deg_{G}u$
$\forall u\in V$, 
$T$ is a sink function where $T(u)\le\deg_{G}u$
$\forall u\in V$ and $\sum_{u}\Delta(u)\le\sum_{u}T(u)$, and $\phi\ge0$
is a conductance parameter. 
%
In time $O(m\phi^{-1}\log m)$ the algorithm returns
an integral preflow $f$ with congestion at most $4/\phi$ and the excess $\ex_{f}(\cdot)$
of $f$. Moreover, if $|\ex_{f}(\cdot)|>0$, then the algorithm also
returns a cut $(S,\overline{S})$\yp{$V \setminus S$ instead of $\overline{S}$} where $\Phi_{G}(S)<\phi$ and \yp{$\phi_G(S)$} $\min\{\vol_{G}(S),\vol_{G}(\overline{S})\}\ge|\ex_{f}(\cdot)|$.
\yp{$V \setminus S$ instead of $\overline{S}$}
\end{lem}


\paragraph{Proof of \ref{thm:push match}.}

Now, we describe the $\PushMatch$ algorithm and prove \ref{thm:push match}.
Given $(G,\phi,\cong,\beta,\{A,B\})$, we define a source function
$\Delta(u)=1$ for $u\in A$ otherwise $\Delta(u)=0$, and a sink
function $T(u)=1$ for $u\in A$ otherwise $T(u)=0$. Then, we invoke $\BoundPush(G,\Delta,T,\phi)$. Let $f$ be the returned preflow
with congestion at most $4/\phi\le\cong$, where the inequality is by the condition on $\cong$ in \Cref{thm:push match}.

Consider when $|\ex_{f}(\cdot)|\ge\beta n/4\ge\beta\vol_{G}/160$ (the last inequality is because the maximum degree is at most 20). 
In this case we return
the smaller side of the cut \textit{$(S,\overline{S})$ }\textit{\emph{which
satisfies the condition of }}\ref{enu:CM cut} of \ref{def:CM}. Otherwise,
we have that $|\ex_{f}(\cdot)|<\beta n/4$. By definition, all the
mass from $A$ is successfully routed by the preflow $f$ to $B$
except $|\ex_{f}(\cdot)|$ units. As the congestion of $F$ is at
most $4/\phi$, we can decompose the preflow $f$ into a collection
$\P$ of paths in time $O(m/\phi)$ using, for example, the link-cut tree \cite{SleatorT83} or depth-first search.\footnote{Algorithm sketch: First, we remove the excess by finding a path from the node $v$ with $\ex_f(v)>0$ in a depth-first search manner. It can can be argue that we will eventually reach a source node. Reduce the flow on every traversed edge by one. Repeat this until there is no excess left. 
Secondly, we decompose the resulting flow into paths in a similar way, as follows. Start from a source $s$ s.t. $f(s)>0$. Follow edges $(u,v)$ with $f(u,v)>0$ in a depth-first search manner. It can be argued that we will eventually reach a sink $t$ with $f(t)<0$. Report the traversed path and reduce the flow on every edge in this path by one. Repeat the process until no such source $s$ can be found.}
By
the definitions of $\Delta$ and $T$, each path starts from $A$ and ends
at $B$. Moreover, each terminal node in $A\cup B$ is an endpoint of
exactly one path, except at most $2|\ex_{f}(\cdot)|<\beta n$ many
terminals which are not an endpoint of any path. \textit{\emph{This
satisfies the condition of }}\ref{enu:CM match} of \ref{def:CM}.
The total running time is $O(m\phi^{-1}\log m)=O(n\phi^{-1}\log n)$.





==> matchingalternate.tex <==
%!TEX root = main_det_cut.tex


\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
\renewcommand\ll{\boldsymbol{\mathit{l}}}
\newcommand\opt{\textsc{OPT}}

\section{Alternate Matching Player}
\label{sec:MatchingAlternate}

In this section, we show an alternate approach for
solving the $\Match$ problem that runs in
almost-linear time.
It is more involved than the approach given in
Theorem~\ref{thm:ES match}, but has the advantage of having
better performances in the low conductance / high
number of commodities regime.

The algorithm is based on directly calling $k$-commodity
flow algorithms that rely on congestion
approximators~\cite{KelnerLOS14,Sherman17}.
Our goal is to directly work with the dual of the linear
program.
We formalize this as an LP. Let:
\begin{enumerate}
	\item $\ff^{(i)}$ denote the amount of satisfied demand of commodity i;
	\item $P^{(i)}$ be the set of simple path from some vertex in $A_i$ to some vertex in $B_i$.
	\item $P^{(i)}_j$ be the $j$-th path in $P^{(i)}$.
	\item Let $\ff^{(i)}_j$ be the amount of flow routed on path $P^{(i)}_j$.
\end{enumerate}
Then the problem of routing the maximum amount of flow
from some $A_i$ to $B_i$, subject to capacities, is then:
\begin{align}
	\max \qquad \sum_{i} \ff^{\left( i \right)}&\\
	\forall e\in E, \sum_{P^{(i)}_j\ni e}\ff^{(i)}_j&\le \cc_e\\
	\forall i\in [k], \ff^{\left( i \right)}
	- \sum_{j}\ff^{(i)}_j&\le 0\\
	\ff^{\left( i \right)}&\ge 0\\
	\ff^{\left(i\right)}_j&\ge 0
\end{align}
Its dual is then the following optimization problem
over edge lengths $\ll \in \Re^{E}_{+}$:
\begin{align}
	\min \qquad \sum \cc_e \ll_e&\\
	\forall i\in [k], j, \sum_{e\in P^{(i)}_j}\ll_e&\ge \ll^{\left( i\right)}\\
	\forall i\in [k], \ll^{\left( i\right)}&\ge 1\\
	\ll_e&\ge 0\\
	\ll^{\left( i\right)}&\ge 0
\end{align}
This can be simplified by removing
the $\ll^{(i)}$ variables, giving: 
\begin{align}
	\min \qquad \sum \cc_e \ll_e&\\
	\forall i\in [k], j, \sum_{e\in P^{(i)}_j}\ll_e&\ge 1\\
	\ll_e&\ge 0.\\
\end{align}
The dual variables $\ll_e$ can be interpreted as the lengths of edges in $G$ such that the shortest path between $A_i$ and $B_i$ is at least $1$ for each $i\in [k]$. 

The multiplicative weight update based approximate
$k$-commodity flow algorithms provide either a large
primal solution, or a small dual solution~\cite{Sherman17}.
\begin{lem}
	\label{lem:UsingCongestionApproximator}
	Given a congestion approximator for $G$,
	we can find in time $\Ohat(m k \epsilon^{-1})$
	either a primal solution with objective at least
	$(1 - \epsilon / 2)m$, or a dual solution with
	objective at most $(1 - \epsilon)m$.
\end{lem}

This cut approximator can in turn be constructed using
(deterministic) ultra-sparsifiers in the same manner
as the recursive approximate max-flow algorithm
in~\cite{Peng16}.
Thus, it suffices to produce a cut in the case of
a dual solution.
That is, an algorithm for the $\Match$ problem
boils down to proving the following:
\begin{lem}
\label{lem:420}
	Suppose we have a graph with $k$ demand
	pairs, along with lengths $\ll$s meeting the
	dual constraints in the linear program above,
	with objective $\opt$
	then we can produce in $\Ohat(m)$ time
	a cut $C$ such that 
	\begin{enumerate}
		\item $vol(C), vol(\overline{C}) \ge \beta/10 m$
		\item $|E(C,\bar{C})|\leq O(\log^2 n) \cdot \opt$
	\end{enumerate}
\end{lem}
Congestion is involved when invoking this lemma because
if the original capacities are $\overline{\cc}_e$, allowing a congestion
of $\rho$ turns the edge capacities into $\cc_e  = \rho \overline{\cc}_e$.
This in turn implies that capacities in $\cc_e$ would be bigger by a
factor of $\rho$ than capacities in the original graph.
Or that we obtain a cut whose size is $m / \rho$,
which is about $\Phi m$ when $\rho$ is set to $\Phi^{-1}$.

The proof strategy is by converting $\ll$ to a tree,
and then perform divide-and-conquer on the tree.
It can be viewed as speeding up the Klein et al.
rounding procedure for multicommodity flow with
general demands~\cite{KleinARR90}.
\begin{lem}
	\label{lem:tree_metric}
	Given any distances on the edges $\ll_e$,
	and any capacities $\cc_e$,
	we can find a (weighted) tree $T$
	such that the tree distance
	$\textsc{Dist}_{T}$ satisfies
	\[
	\ll_{uv}
	\leq
	\textsc{Dist}_{T}\left( u , v \right)
	\qquad \forall e = uv
	\]
	and
	\[
	\sum_{e} \textsc{Dist}_{T}\left( u , v \right)\cc_e
	\leq
	O\left( \log^2{n} \right)
	\sum_{e} \ll_{e} \cc_e
	\]
\end{lem}
This is done by invoking low stretch spanning trees~\cite{AbrahamN12}:
\begin{lem}
	\label{lem:LSST}
	Given any undirected weighted graph $G = (V, E, \ww)$,
	we can find a spanning tree $T$ (with the same
	weights) such that
	\[
	\sum_{e = uv}
	\frac{\textsc{Dist}_{T} \left( u, v\right)}{\ww_{uv}}
	\leq
	O\left( m \log{n} \log\log{n} \right).
	\]
\end{lem}

However, we need to slightly tweak both the congestion
and dilation here.

\begin{proof}(of~\cref{lem:tree_metric})
	
	By standard perburbation arguments based on the
	max-weight spanning trees~\cite{AbrahamN12},
	we may assume both $\ll$ and $\cc$ are integers
	between $1$ and $n^{O(1)}$.
	
	We can get out the general version via two operations:
	\begin{enumerate}
		\item Putting in $\cc_e$ parallel edges.
		\item Turning a $\ll_{e}$ lengthed edge into a
		path of $\ll_{e}$ length $1$ edges.
	\end{enumerate}
	
	Specifically:
	\begin{enumerate}
		\item The case of $\ll_{e} = \cc_{e} = 1$
		follows from a verbatim invocation, since
		$\sum_{e} \ll_{e} \cc_e = m$ a well.
		
		\item The case of $\ll_{e} = 1$ follows
		from turning each edge into $\cc_{e}$
		parallel edges: only one of them can be in the tree,
		and in the case where none of them are in the tree,
		the distance between $uv$ gets multiplied by a
		factor of $\cc_{e}$ in the sum.
		
		\item The case of $\cc_{e} = 1$ can be handled
		by turning an edge of length $\ll_{e}$ into
		a path of $\ll_{e}$ length $1$ edges.
		Because there are $\ll_{e} - 1$ intermediate
		vertices on this path, at most one of these
		edges can be left out of the tree.
		If it is left out, its stretch charge is
		\[
		\ll_{e} - 1 + \textsc{Dist}_{T}\left(u, v \right),
		\] which dominates $\textsc{Dist}_{T}\left(u, v \right)$. 
		
		If no edge is left out, their total stretch charge is 
		\[
		\ll_{e}
		\] which is equal to $\textsc{Dist}_{T}\left(u, v \right)=\ll_{e}$. 
		
		Also, instead of $m$, we now get $\sum_{e} \ll_{e}$.
		
		(To convert the tree to the original graph, we keep the edge $e$ if none of its $\ll_{e}$ edges are left out.) 
		
		\item The general $\ll_{e}$ \& $\cc_e$ case is handled
		by combining the two above: $e$ becomes a $\ll_e$-lengthed
		path of $c_e$-multi edges.
		This turns $m$ into $\sum_{e} \ll_{e} \cc_e$, which
		is the right number we want on the RHS.
		
		To convert the tree to the original graph, we keep the edge $e$ if there is one path (among the $\cc_e$ paths) such that no edge on this path is left out. 
		
		If $e$ is kept, its stretch is just $\ll_e$. It contributes $\ll_e\cc_e$ to LHS, which is less than the contribution of the $\cc_e$ $\ll_e$-length paths. 
		If $e$ is not kept, its strech is $\textsc{Dist}_T\left(u,v\right)$ which contributes $\cc_e\textsc{Dist}_T\left(u,v\right)$ to LHS. It is less than the contribution of the paths since each path has a missing edge which contributes  $\textsc{Dist}_T\left(u,v\right)$.
		
	\end{enumerate}
	
	The algorithmic observation for the overall running
	time is that the AN`12 algorithm~\cite{AbrahamN12}
	can still be efficiently simulated:
	this is because:
	\begin{enumerate}
		\item it's ball growing based,
		\item a bundle of edges still behaves like a single
		edge under shortest paths, with a slightly different
		book-keeping mechanism for how many are now on the
		boundary.
	\end{enumerate}
	
\end{proof}


It remains to prove that a good cut can be found
on a tree metric
\begin{theorem}
	\label{thm:tree_ball}
	Given any weighted tree $T$ with $k$ source sink
	pairs $(s_i, t_i)$ such that
	\[
	\textsc{Dist}_{T}\left( s_i, t_i \right)
	\geq 1
	\qquad
	\forall i
	\]
	we can find a distance-shrinking embedding of $T$
	on the line such that there exists a point $x$ with
	at least $0.1k$ $s_i/t_i$s less than $x - 0.1$,
	and at least $0.01k$ $s_i/t_i$s more than $x + 0.1$.
\end{theorem}

One way to obtain this embedding is to find a
`ball separator' vertex:
\begin{lem}
	\label{lem:BallSeparator}
	Given any weighted tree along with $k$ source sink
	pairs $(s_i, t_i)$, each at least $1$ apart in the tree,
	we can find a vertex $r$ such that $T \setminus r$
	has subtrees that can be grouped into at least two
	subsets containing at least $0.01k$ terminals more than
	distance $0.1$ from $r$.
\end{lem}

This Lemma leads to~\cref{thm:tree_ball}
because we can put everything in
one subtree to the left of $r$,
and everything in the other subtree to the right of $r$.

We find this separator by modifying the tree
separator algorithm.

\begin{proof}(of~\cref{lem:BallSeparator})
\begin{enumerate}
	\item Start with a separator $x$ that splits
	$T$ into two subtrees, $T_1$ and $T_2$, each with
	more than $0.3k$ terminals.
	\item For $x$ to not work, $B(x, 0.1)$ must consume
	at least $0.29k$ of either $T_1$ or $T_2$, WOLOG $T_1$.
	\item Then a big chunk of $T_1 \cap B(x, 0.1)$ must
	have matches that go outside of $T_1$ (through $r$).
	(note that nothing in $B(x, 0.1)$ can match to each other:
	the distances are simply too small)
	\item Let this set of matching terminals be $\hat{V}$.
	By the point above, $|\hat{V}| > 0.28k$.
	Also, note that for any $v \in \hat{V}$, we have:
	\[
	0.9 \leq \textsc{Dist}_T\left( r, v\right)
	=\textsc{Dist}_{\hat{T}}\left( r, v\right).
	\]
	\item Let the tree induced by these matched points be
	$\hat{T}$.
	\item Now just walk $r$ down $\hat{T}$, always towards
	the subtree with the maximum number of vertices:
	\begin{enumerate}
		\item If we ever walked a distance more than $0.1$,
		and still have more than $0.1k$ mass left, we're done,
		because we're now sufficiently far away from $T_1$.
		\item If at any point, the subtree size becomes less than $0.1k$, we terminate there: we can arrange
		all the hanging trees in a way that's balanced.
		Note here by triangle inequality, we still have
		\[
		B\left(r, 0.1\right) \cap \hat{V} = \emptyset.
		\] 
	\end{enumerate}
\end{enumerate}
\end{proof}

Putting this tree separation result with the low stretch
embedding then gives the dual algorithm.
\begin{proof} (of~\ref{lem:420})
	%For each vertex $v$ in $A_i$, we add another vertex $\widehat{v}$ and edge $\{\widehat{v}, v\}$ with capacity $vol_G(v)$. Let $H$ be the set of edges $\{\widehat{v}, v\}$ for all $v\in A_i, i\in [k]$. supply on vertex $v$ is moved to $\widehat{v}$. We further contract all $\hat{v}$ for $v\in A_i$ into a single vertex $s_i$. This modification to the multi-commodity flow problem (not to the original graph $G$) does not change the LP value. Similarly, for each $B_i$, we add a sink vertex $t_i$.\\
	
	By \cref{lem:tree_metric} and \cref{lem:tree_metric},
	we have distance labels $dis(v)$ for each $v\in V(H)$ and a spanning tree $T$ of $H$ such that 
	for $\cc(X)$ being the sum of capacities of edges in $X$,
	we have  
	\begin{align}
		&\int_{0}^{\infty} \cc\left(\{v|dis(v)< x\}, \{v|dis(v)>x\}\right) dx\\
		=&\sum_{\{a,b\}=e\in E, dis(a)>dis(b)} \cc_e(dis(a)-dis(b))\\
		\le&\sum_{\{a,b\}=e\in E} \cc_e dist_T(a,b)\\
		\le &O(\log ^2 n) \sum_{e\in E} \cc_e\ll_e
	\end{align} 
	where $dist_T(a,b)$ is the tree distance between vertices $a,b$ on $T$. Moreover, there exists a value $x$ such that $|\{v|v\in V(H)\backslash V(G), dis(v)<x-0.1\}|\ge 0.2 \beta m$ and $|\{v|v\in V(H)\backslash V(G), dis(v)>x+0.1\}|\ge 0.2 \beta m$.
	
	We have
	\begin{align}
		avg\defeq &\int_{-\infty}^{\infty} \cc\left(\{v|dis(v)< x\}, \{v|dis(v)>x\}\right) dx\\
		\le &O(\log ^2 n)\sum_{e\in E} \cc_e\ll_e \quad \text{(by property of distance labels)}\\
		=&O(\log ^2 n) \cdot F^*.
	\end{align}
	Consider the interval $I=[x-0.1, x+0.1]$. There exists $y\in I$ such that  
	$$\cc\left(\{v|dis(v)< y\}, \{v|dis(v)>y\}\right)\le 5 \cdot avg$$.
	Call this edge set $F$.
	Let $C$ be $\{v|dis(v)<y,v\in V(G)\}$,
	and $\overline{C} = V \backslash C$.
	
	Since $y\in I$, $C$ is $0.1$-balanced.
	We then ahve
	\[
	\cc(C,\bar{C})\le \cc(F)\le 5 \cdot avg =O(\log^2 n) \cdot OPT
	\]
	since the edges between $C$ and $\bar{C}$ is a subset of $F$. ($F$ may contain, for example, $\{\widehat{v},v\}$.) Thus we obtain $|E(C,\bar{C})|= \cc(C,\bar{C})\le O(\log ^2 n) \cdot OPT$.
\end{proof}



==> old-abstract.tex <==
We consider the classical Minimum Balanced Cut problem: given a graph $G$, compute a partition of its vertices into two subsets of roughly equal volume, while minimizing the number of edges connecting the subsets. We present the first {\em deterministic, almost-linear time} approximation algorithm for this problem. Our algorithm in fact provides a stronger guarantee: it either returns a balanced cut whose value is close to a given target value, or it certifies that such a cut does not exist by exhibiting a large subgraph of $G$ that has high conductance.
We use this algorithm to obtain deterministic algorithms for dynamic connectivity and minimum spanning forest, whose worse-case update time on an $n$-vertex graph is $n^{o(1)}$, thus resolving a major open problem in the area of dynamic graph algorithms. Our work also implies deterministic algorithms for a host of additional problems, whose time complexities match,  up to subpolynomial in $n$ factors,  those of known randomized algorithms. The implications include almost-linear time deterministic algorithms for solving Laplacian systems and for approximating maximum flows in undirected graphs. 

%Laplacian systems, maximum flows on undirected graphs, minimum-cost bipartite perfect matching, spectral sparsifiers



\endinput

We give the first deterministic algorithm for computing an expander decomposition with almost-linear running time. 
This implies a deterministic dynamic connectivity algorithm with $n^{o(1)}$ worst-case update time on an $n$-node graph, resolving a major open problem in dynamic graph algorithms whether the deterministic algorithm by Frederickson and Eppstein et.~al.~with $O(\sqrt{n})$ worst-case update time can be polynomially improved. Among many other applications, we show almost-linear-time determinsitc algorithms for solving Laplacian systems
and for computing approximate max flows in undirected graphs. 



%Our algorithm is the first recursive implementation of the cut-matching game framework, with the key insight being to make the ``matching'' player solve a harder problem similar to the multi-commodity flow problem. 


==> omit.tex <==
\section{Deferred Proofs}
\label{Sec:OmittedProofs}

\subsection{Proof of \ref{prop:conductance preserve}}
\label{subsec:BoundedDegreeReduction}


\begin{proof}
        Consider any cut $(S,\ol{S})$ in $G$ where $\vol_{G}(S)\le\vol_{G}(\ol{S})$.
        We will prove that either 
        \begin{enumerate}[label=(\roman*)]
                \item \label{item:one_cond_small} $\Phi_{G}(S)=\Omega(\Phi_{G}^{in})$, or
                \item \label{item:two_cond_small} we can obtain in
                $O(m)$ time a cut $T$ respecting the partition
                $\Vcal$ where (a) $\Phi_{G}(T)=O(\Phi_{G}(S)/\Phi_{G}^{in})$, (b) $\vol_{G}(T)=\Omega(\vol_{G}(S))$, and (c) $\vol_{G}(\overline{T})=\Omega(\vol_{G}(\overline{S}))$.
                %we can obtain, in $O(\vol_{G}(V))$ time, a cut $T$ as in \Cref{eq:two_cond}, i.e. a $\Omega(\beta)$-balanced
                %cut $(T,V-T)$ respecting $\P$ such that $\Phi_{G}(T)=O(\Phi_{G}(S)/\Phi_{G}^{in})$.
        \end{enumerate}
        
        Roughly, the above means that either $S$ is {\em not} so sparse, or we can quickly convert it into a cut $T$ respecting $\Vcal$ whose conductance is not much more than $S$ and that is almost as balanced as $S$. Observe that this implies both \ref{item:one_cond,item:two_cond} of \ref{prop:conductance preserve}. To see this for \ref{item:one_cond}, consider any cut $S$. Either  $\Phi_{G}(S)=\Omega(\Phi_{G}^{in})$ by \ref{item:one_cond_small} or, by \ref{item:two_cond_small}, there is a cut $T$ such that $\Phi_G(S)=\Omega(\Phi_G(T)\cdot\Phi_G^{in})=\Omega(\Phi_G^{out}\cdot\Phi_G^{in})$, where the first equality is because of (a) and the second is because $T$ respects $\Vcal$.  
        %
        To prove \ref{item:two_cond}, we start from $S$ as in \ref{item:two_cond} and use \ref{item:two_cond_small} to get a cut $T$ which, by (b) and (c), is $\Omega(\beta)$-balanced (since $S$ is $\beta$-balanced).\footnote{In more details, by (b) and (c), $T$ is such that $\vol_{G}(T)=\Omega(\vol_{G}(S))=\Omega(\beta \vol(V))$ (the last equality is because $S$ is $\beta$-balanced) and $\vol_{G}(\overline{T})=\Omega(\vol_{G}(\overline{S}))=\Omega(\beta \vol(V))$. These imply that $T$ is $\Omega(\beta)$-balanced. Moreover, $\Phi_{G}(T)  =\frac{\delta_{G}(T)}{\min\{\vol_{G}(T),\vol_{G}(\overline{T})} = O(\frac{\delta_{G}(S)/\Phi_{G}^{in}}{\min\{\vol_{G}(S),\vol_{G}(\overline{S})\}}) =O(\Phi_{G}(S)/\Phi_{G}^{in})$, where the second equality is because of (a), (b), and (c).} 
        %
        %In more details,  we have 
        %\begin{align*}
        %\Phi_{G}(T) & =\frac{\delta_{G}(T)}{\min\{\vol_{G}(T),\vol_{G}(\overline{T})}\\
        %& \lesssim\frac{\delta_{G}(S)/\Phi_{G}^{in}}{\min\{\vol_{G}(S),\vol_{G}(\overline{S})\}}\\
        %& =\Phi_{G}(S)/\Phi_{G}^{in}.
        %\end{align*}
        %
        %Observe that this implies both the first part of the lemma, i.e. $\Phi_{G}=\Omega(\Phi_{G}^{out}\cdot\Phi_{G}^{in})$, and also the second part.\danupon{DISCUSS: I don't see why this is true, e..g why does the first claim imply anything about the lemma? BTW, avoid "either ... otherwise".}
        It remains to prove that for any cut $S$, either \ref{item:one_cond_small} or \ref{item:two_cond_small} holds.  
        %
        Let 
        %$\P'=\{V_{i}\mid0<\vol_{G}(S\cap V_{i})<2\vol_{G}(V_{i}-S)\}$ and $\P''=\{V_{i}\mid\vol_{G}(S\cap V_{i})>2\vol_{G}(V_{i}-S)\}$. 
        $$\Vcal'=\{V_{i}\mid\vol_{G}(S\cap V_{i})<2\vol_{G}(V_{i}-S)\} \mbox{,  } \Vcal''=\{V_{i}\mid\vol_{G}(S\cap V_{i})\geq 2\vol_{G}(V_{i}-S)\} \mbox{ and } T=\bigcup_{V_{i}\in\Vcal''}V_{i}.$$ 
        %$$T=\bigcup_{V_{i}\in\P''}V_{i},\ \overline{T}=V-T\mbox{ and } \overline{S}=V-S.$$
        %\begin{align*}
        %\P'=\{V_{i}\mid\vol_{G}(S\cap V_{i})<2\vol_{G}(V_{i}-S)\} &\mbox{ and } \P''=\{V_{i}\mid\vol_{G}(S\cap V_{i})\geq 2\vol_{G}(V_{i}-S)\}.\\
        %T=\bigcup_{V_{i}\in\P''}V_{i}
        %%,\ \overline{T}=V-T &\mbox{ and } \overline{S}=V-S.
        %\end{align*}
        %
        In other words, $\Vcal'$ contains clumps that do not overlap much with $S$ and $\Vcal''$ contains those with big overlaps. The latter set defines a new cut $T$. Note that $T$ can be computed in $O(m)$ time. (Some readers may find \Cref{fig:SvsT} useful for following the arguments below.)
        
        \begin{figure}
                \centering
            
            	\begin{tikzpicture}[xscale = 1, yscale=1]
            	\draw (0,0) --(4,0) -- (4,1) -- (0,1) -- (0,0);
            	\draw (-3,-1) --(2,-1) -- (2,0) -- (-3,0) -- (-3,-1);
            	\draw (-4,-2) --(1,-2) -- (1,-1) -- (-4,-1) -- (-4,-2);
            	\draw (-6,-3) --(-2,-3) -- (-2,-2) -- (-6,-2) -- (-6,-3);
            	\node at (1, 0.5) {$V_1$};
            	\node at (0, -0.5) {$V_2$};
            	\node at (-2, -1.5) {$V_3$};
            	\node at (-3, -2.5) {$V_4$};
            	\draw [decorate,decoration={brace,amplitude=10pt}]
            	(4.4,1) -- (4.4,-0.98) node [black,midway, xshift=0.6cm] 
            	{$P'$};
            	\draw [decorate,decoration={brace,amplitude=10pt}]
            	(4.4,-1.02) -- (4.4,-3) node [black,midway, xshift=0.6cm] 
            	{$P''$};
            	\node at (-2, 1) [blue] {$S$};
            	\node at (-4, 0) [red] {$T$};
            	\filldraw[draw=black, color=pink](-2.96, -0.01) rectangle (-1.04, -0.98);
            	\node at (-2, -0.5)  {S-T};
            	\filldraw[draw=black, color=green](-0.96, -1.02) rectangle (0.96, -1.98);
            	\node at (0, -1.5)  {T-S};
       			\filldraw[draw=black,color=lightgray] (-1,1) rectangle (-1.2,-3);
            	\filldraw[draw=black,color=lightgray] (-3,0.5) rectangle (-3.2,-1);
            	\filldraw[draw=black,color=lightgray] (1,-1) rectangle (0.8,-2.5);
				\draw [line width=3pt, blue](-1, 1) -- (-1, -3);
            	\draw [line width=3pt, red](-3, 0.5) -- (-3, -1) -- (1, -1) -- (1, -2.5);
            	\end{tikzpicture}
            
                \caption{Relationships between $S$, $T$ and the clumps. The area of a part of each $V_i$ represents its volume (e.g. $\vol_G(S\cap V_3)$ is very high, thus $V_3\in \Vcal''$).}\label{fig:SvsT}
        \end{figure}
        %
        %
        %\begin{comment}
        Note that as $V_{i}$ is a clump, $\vol_{G[V_{i}]}(S\cap V_{i})=\Theta(\vol_{G}(S\cap V_{i}))$
        and $\vol_{G[V_{i}]}(V_{i}-S)=\Theta(\vol_{G}(V_{i}-S))$. So, 
        %$\delta_{G[V_{i}]}(V_{i}\cap S)\ge\Omega(\Phi_{G}^{in}\cdot\vol_{G[V_{i}]}(V_{i}\cap S))$
        %for each $V_{i}\in\P'$ and $\delta_{G[V_{i}]}(V_{i}-S)\ge\Omega(\Phi_{G}^{in}\cdot\vol_{G[V_{i}]}(V_{i}-S))$
        %for each $V_{i}\in\P''$. 
        %
        \begin{align}
        \forall V_i\in \Vcal': \delta_{G[V_{i}]}(V_{i}\cap S)&\ge\Omega(\Phi_{G}^{in}\cdot\vol_{G[V_{i}]}(V_{i}\cap S))\label{eq:cond:clump1} \mbox{  and}\\
        \forall V_i\in \Vcal'': \delta_{G[V_{i}]}(V_{i}-S)&\ge\Omega(\Phi_{G}^{in}\cdot\vol_{G[V_{i}]}(V_{i}-S)). \label{eq:cond:clump2} 
        \end{align}
        %
        %\end{comment}
        %
        %Let $T=\bigcup_{V_{i}\in\P''}V_{i}$, $\overline{T}=V-T$
        %and $\overline{S}=V-S$. 
        %
        Note a very important fact that {\em both} $\vol_{G}(T-S)$ and $\vol_{G}(S-T)$ are $O(\delta_{G}(S)/\Phi_{G}^{in})$. This exploits the definition of $T$ and the fact that each $V_i$ is a clump, as in the inequalities below.\footnote{Here we attempt to provide an intuition behind \Cref{eq:cond:S-T,eq:cond:T-S}. By the way we define $T$, we can write $\vol_{G}(S-T)$ and $\vol_{G}(T-S)$ as a sum of $\vol_G(X)$ over subsets $X\subseteq V_i$ (see the first lines).
                %that is contained in one side of the cut $(S, V-S)$ and in some $V_i$ (i.e. $X\subseteq V_i\cap S$ or $X\subset V_i\cap (V-S)=V_i-S$ as in the first lines of \Cref{eq:cond:S-T,eq:cond:T-S}). 
                %       
                We can bound this by $\vol_{G[V_i]}(X)$, exploiting that each $V_i$ is a clump (see the second lines). This allows us to related $\vol_{G[V_i]}(X)$ to $\delta_{G[V_i]}(X)$ with a blow up of $\Phi_G^{in}$, as in the third and fourth lines. We can then relate $\delta_{G[V_i]}(X)$ back to $\delta_G(S)$ using the fact that either $X=S\cap V_i$ or $X=V_i-S$; in both case we can conclude that $E_{G[V_i]}(X, V_i-X)\subseteq E(S, V-S)$.}
        
        
        
        %\noindent\begin{minipage}{.3\linewidth}
        %       \begin{align}
        %       \vol_{G}(S-T) & =\sum_{V_{i}\in\P'}\vol_{G}(S\cap V_{i}) \nonumber
        %       \end{align}
        %\end{minipage}%
        %\begin{minipage}{.7\linewidth}
        %       \begin{align}
        %       \vol_{G}(T-S) & =\sum_{V_{i}\in\P''}\vol_{G}(V_{i}-S) &\mbox{(by the definition of $T$)}\nonumber\\
        %       \end{align}
        %\end{minipage}
        
        \begin{align}
        \vol_{G}\left(S-T\right) & =\sum_{V_{i}\in\Vcal'}\vol_{G}(S\cap V_{i}) & \mbox{\small(by the definition of $T$)}\nonumber\\
        & \leq O\left(1 \right)\cdot \sum_{V_{i}\in\Vcal'}\vol_{G[V_{i}]}(S\cap V_{i}) &\mbox{\small($V_i$ is a clump)}\nonumber\\
        & \leq O\left(1 \right)\cdot \sum_{V_{i}\in\Vcal'}\delta_{G[V_{i}]}(S\cap V_{i})/\Phi_{G[V_i]} 
        &\mbox{\small (\Cref{eq:cond:clump1})}\nonumber\\
        %%&\mbox{\small (since $\forall X\subseteq V_i: \delta_{G[V_{i}]}(X)\geq \vol_{G[V_{i}]}(X)\cdot\Phi_{G[V_i]}$; here $X=S\cap V_i$)}\nonumber\\
        %&\mbox{\small($V_{i} \in \P'$)}\nonumber\\ %\label{eq:cond:S-T:three}\\
        %\footnotemark
        & \leq O\left(1 \right)\cdot \sum_{V_{i}\in\Vcal'}\delta_{G[V_{i}]}(S\cap V_{i})/\Phi_{G}^{in} &\mbox{\small($\Phi_{G[V_i]}\geq \Phi_{G}^{in}$)}\nonumber\\ % and $\delta_{G[V_{i}]}(S\cap V_{i})=\delta_{G[V_{i}]}(S)$)}\nonumber\\
        & \leq O\left( \delta_{G}(S)/\Phi_{G}^{in}. \right) &\mbox{\small($E(S\cap V_i,V_i-S)\subseteq E(S, V-S)$)} \label{eq:cond:S-T}
        \end{align}
        and similarly for the other side of the symmetric difference:
        \begin{align}
        %
        \vol_{G}\left(T-S\right) & =\sum_{V_{i}\in\Vcal''}\vol_{G}(V_{i}-S) &\mbox{\small(by the definition of $T$)}\nonumber\\
        & \leq O\left(1 \right)\cdot \sum_{V_{i}\in\Vcal''}\vol_{G[V_{i}]}(V_{i}-S) &\mbox{\small($V_i$ is a clump)}\nonumber\\
        & \leq O\left(1 \right)\cdot \sum_{V_{i}\in\Vcal''}\delta_{G[V_{i}]}(V_{i}-S)/\Phi_{G[V_i]} &\mbox{\small (\Cref{eq:cond:clump2})}\nonumber\\
        %\mbox{\small($V_{i} \in \Vcal''$)}\nonumber\\%\label{eq:cond:T-S:three}\\
        %\addtocounter{footnote}{-1}\footnotemark
        & \leq O\left( \delta_{G}(S)/\Phi_{G}^{in} \right) &\mbox{\small ($\Phi_{G[V_i]}\geq \Phi_{G}^{in}$ and $E(S\cap V_i,V_i-S)\subseteq E(S, V-S)$)}\footnotemark
        \label{eq:cond:T-S}
        %& =\delta_{G}(S)/\Phi_{G}^{in}.
        \end{align}
        \footnotetext{Note that the third lines of both \Cref{eq:cond:S-T,eq:cond:T-S}
                %\Cref{eq:cond:S-T:three,eq:cond:T-S:three} 
                follow from a more general fact that for all $ X\subseteq V_i$, $\delta_{G[V_{i}]}(X)\geq \vol_{G[V_{i}]}(X)\cdot\Phi_{G[V_i]}$ (here  $X=S\cap V_i$ and $X=V_i-S$). Also, the last lines follow from a more general fact that if $X=S\cap V_i$ or $X=V_i-S$, then  $E(X,V_i-X)\subseteq E(S, V-S)$. 
        }
        
        %Both of the two bounds above exploit the fact that $V_{i}$ is a clump.
        %From this, we obtain the first part of the claim:
        %Note that in \Cref{eq:cond:S-T} we did not overcount edges since we count only edges in each $G[V_i]$. 
        %\danupon{Need to define notations for  $E_{G[V_i]}[V_i,V_i-S]\subseteq E_G[S, V-S]$?}
        %In the first case, 
        
        Now consider two cases. 
        
        \paragraph{Case 1: $\vol_{G}(S-T)\ge\vol_{G}(S)/2$.} Inequalities below show that \ref{item:one_cond_small} holds, i.e.  $\Phi_{G}(S)=\Omega(\Phi_{G}^{in})$. %An intuition behind these inequalities is that $\delta_G(S)$ can be lower bounded from below by $\vol_G(S- T)$. 
        \begin{align}
        \delta_{G}(S) & =\Omega\left(\Phi_{G}^{in}\cdot\vol_{G}(S-T)\right) & \mbox{(by \Cref{eq:cond:S-T})}\nonumber\\%\label{eq:cond:case_1.4}\\
        & \ge\Omega\left(\Phi_{G}^{in}\cdot\vol_{G}(S)/2\right) & \mbox{(the assumption of this case).} \nonumber%\label{eq:cond:case_1.5}
        \end{align}
        %
        %\begin{align}
        %\delta_{G}(S) & \ge\sum_{V_{i}\in\P'}\delta_{G[V_{i}]}(S\cap V_{i})\label{eq:cond:case_1.1}\\% & \mbox{(no overcounting since we count only edges in $G[V_i]$'s)}\\
        % & =\Omega\left(\Phi_{G}^{in}\cdot\sum_{V_{i}\in\P'}\vol_{G[V_{i}]}(S\cap V_{i})\right) & \mbox{(since $\delta_{G[V_{i}]}(S\cap V_{i})\geq \vol_{G[V_{i}]}(S\cap V_{i})\cdot\Phi_{G[V_i]}$)}\nonumber\\%\label{eq:cond:case_1.2}\\
        % & =\Omega\left(\Phi_{G}^{in}\cdot\sum_{V_{i}\in\P'}\vol_{G}(S\cap V_{i})\right)&\mbox{(since $V_i$ is a clump)}\nonumber\\ %, $\vol_{G[V_{i}]}(S\cap V_{i})=\Omega(\vol_{G}(S\cap V_{i}))$)}\label{eq:cond:case_1.3}\\
        % & =\Omega\left(\Phi_{G}^{in}\cdot\vol_{G}(S-T)\right) & \mbox{(by the definition of $T$)}\nonumber\\%\label{eq:cond:case_1.4}\\
        % & \ge\Omega\left(\Phi_{G}^{in}\cdot\vol_{G}(S)/2\right) & \mbox{(assumption of this case).} \nonumber%\label{eq:cond:case_1.5}
        %\end{align}
        %Note that in \Cref{eq:cond:case_1.1} we did not overcount edges since we count only edges in each $G[V_i]$. 
        %, \Cref{eq:cond:case_1.2} is because of \Cref{eq:cond:degree_lower_bound}, \Cref{eq:cond:case_1.3} is because each $V_i$ is a clump, ...
        %So $\Phi_{G}(S)=\Omega(\Phi_{G}^{in})$.
        
        \paragraph{Case 2:  $\vol_{G}(S-T)< \vol_{G}(S)/2$.}
        We show that $T$ satisfies (a), (b), and (c), thus \Cref{item:two_cond_small} holds. By \Cref{eq:cond:S-T,eq:cond:T-S}, we have\footnote{To see the first inequality, observe that $\delta_{G}(T) 
                = |E(T\cap S, V-T-S)|+|E(T\cap S, S-T)| + |E(T-S,V-T-S)| + |E(T-S,S-T)|$. Moreover, $ |E(T\cap S, V-T-S)|\leq \delta_{G}(S)$, $|E(T\cap S, S-T)|\leq \vol_G(S-T)$, and $ |E(T-S,V-T-S)| + |E(T-S,S-T)|\leq \vol_G(T-S)$.}
        %
        % (1) $\delta_{G}(T)=O(\delta_{G}(S)/\Phi_{G}^{in})$,
        %(2) $\vol_{G}(T)=\Omega(\vol_{G}(S))$, and (3) $\vol_{G}(\overline{T})=\Omega(\vol_{G}(\overline{S}))$.
        %\danupon{I removed below and made them (a)-(c)
        %This would imply 
        %\begin{align*}
        %\Phi_{G}(T) & =\frac{\delta_{G}(T)}{\min\{\vol_{G}(T),\vol_{G}(\overline{T})}\\
        % & \lesssim\frac{\delta_{G}(S)/\Phi_{G}^{in}}{\min\{\vol_{G}(S),\vol_{G}(\overline{S})\}}\\
        % & =\Phi_{G}(S)/\Phi_{G}^{in}.
        %\end{align*}
        %and that $T$ is a $\Omega(\beta$)-balanced cut. 
        %}
        %Now, it remains
        %to prove the three claims.
        %
        %
        %\begin{claim}
        %We have the following:
        %\end{claim}
        %
        %\begin{itemize}
        %\item $\delta_{G}(T)=O(\delta_{G}(S)/\Phi_{G}^{in})$, 
        %\item $\vol_{G}(S)=O(\vol_{G}(T))$, and
        %\item $\vol_{G}(\overline{S})=O(\vol_{G}(\overline{T}))$. 
        %\end{itemize}
        %\begin{proof}
        %To do this, let us first show that $\vol_{G}(T-S)$ and $\vol_{G}(S-T)$ are both $O(\delta_{G}(S)/\Phi_{G}^{in})$.
        %it is convenient to bound $\vol_{G}(T-S)$ and $\vol_{G}(S-T)$ first:
        %We have 
        %\begin{align}
        %\vol_{G}(T-S) & =\sum_{V_{i}\in\P''}\vol_{G}(V_{i}-S)\nonumber\\
        % & \lesssim\sum_{V_{i}\in\P''}\vol_{G[V_{i}]}(V_{i}-S)\nonumber\\
        % & \lesssim\sum_{V_{i}\in\P''}\delta_{G[V_{i}]}(V_{i}-S)/\Phi_{G}^{in}\nonumber\\
        % & \le\delta_{G}(V-S)/\Phi_{G}^{in}=\delta_{G}(S)/\Phi_{G}^{in}.\label{eq:cond:case2.1}\\
        %%\end{align}
        %%%Next, 
        %%\begin{align}
        %\vol_{G}(S-T) & =\sum_{V_{i}\in\P'}\vol_{G}(S\cap V_{i})\nonumber\\
        % & \lesssim\sum_{V_{i}\in\P'}\vol_{G[V_{i}]}(S\cap V_{i})\nonumber\\
        % & \lesssim\sum_{V_{i}\in\P'}\delta_{G[V_{i}]}(S)/\Phi_{G}^{in}\nonumber\\
        % & \le\delta_{G}(S)/\Phi_{G}^{in}.\label{eq:cond:case2.2}
        %\end{align}
        %Both of the two bounds above exploit the fact that $V_{i}$ is a clump.
        %From this, we obtain the first part of the claim:
        %
        %
        %\begin{align*}
        %\delta_{G}(T) 
        %& = |E[T\cap S, V-T-S]|+|E[T\cap S, S-T]| + |E[T-S,V-T-S]| + |E[T-S,S-T]|\\
        % & \le\delta_{G}(S)+\vol_{G}(T-S)+\vol_{G}(S-T)\\
        % & =O(\delta_{G}(S)/\Phi_{G}^{in}).
        %\end{align*}
        %For the second part, we have 
        %
        $$ \delta_{G}(T) \le
        \delta_{G}(S)+\vol_{G}(T-S)+\vol_{G}(S-T)
        = O(\delta_{G}(S)/\Phi_{G}^{in}).$$
        %%
        This implies (a) in \Cref{item:two_cond_small}. For (b), we have 
        %
        %
        %\begin{align*}
        %\vol_{G}(S) & =\vol(S\cap T)+\vol(S-T)\\
        %& \le\vol_{G}(T)+\vol_{G}(S-T) \\
        % & \le\vol_{G}(T)+\vol_{G}(S)/2 
        %\end{align*}
        %
        $$\vol_{G}(S) =\vol_G(S\cap T)+\vol_G(S-T) \le\vol_{G}(T)+\vol_{G}(S-T)
        \le\vol_{G}(T)+\vol_{G}(S)/2$$
        %
        where the last inequality is because the assumption of Case 2. It follows that $\vol_{G}(S)=O(\vol_{G}(T))$, completing (b). For (c), first observe
        that
        \begin{align}
        \vol_{G}(T-S) & =\sum_{V_{i}\in\Vcal''}\vol_{G}(V_{i}-S)\nonumber\\
        & <\sum_{V_{i}\in\Vcal''}\vol_{G}(V_{i}\cap S)/2 & \mbox{(by the definition of $\Vcal''$)}\nonumber\\
        & =\vol_{G}(T\cap S)/2 &\mbox{(since $T\cap S=\bigcup_{V_i\in \Vcal''} V_i\cap S$; see \Cref{fig:SvsT}).}\nonumber\\
        &\le \vol_{G}(S)/2 &\mbox{($T\cap S\subseteq S$)}\nonumber\\
        &\le \vol_{G}(\overline{S})/2 &\mbox{($S$ is defined to be the smaller side in the cut)}
        \label{eq:cond:volT-S}
        \end{align}
        So we have
        \begin{align*}
        \vol_{G}(\overline{S}) & =\vol_{G}(\overline{T})+\vol_{G}(T-S) &\mbox{($\overline{S}=\overline{T}\cup (T-S)$; see \Cref{fig:SvsT})}\\
        % & <\vol_{G}(\overline{T})+\vol_{G}(T\cap S)/2 &\mbox{(by \Cref{eq:cond:volT-S})}\\
        % & \le\vol_{G}(\overline{T})+\vol_{G}(S)/2 &\mbox{($T\cap S\subseteq S$)}\\
        & \le\vol_{G}(\overline{T})+\vol_{G}(\overline{S})/2 &\mbox{(by \Cref{eq:cond:volT-S})},
        \end{align*}
        and so $\vol_{G}(\overline{S})=O(\vol_{G}(\overline{T}))$.
        %\end{proof}
\end{proof}




\iffalse

\subsection{Proof of \ref{lem:BCut from Cut}}

\begin{algorithm}
\begin{enumerate}
\item Let $i\gets1$, $G_{1}\gets G$, $S\gets\emptyset$.
\item While $\vol_{G}(S)\le\vol_{G}/3$
\begin{enumerate}
\item Let $S_{i}$ be the cut returned by $\Cut(G_{i},\phi_{L},\phi_{U},\beta)$.
\item $S\gets S\cup S_{i}$.
\item If $S_{i}$ is from \ref{enu:CP prune} of $\Cut$, then break.
\item $G_{i+1}\gets G_{i}\{V(G_{i})-S_{i}\}$.
\item $i\gets i+1$.
\end{enumerate}
\item If $\vol_{G}(S)\le\vol_{G}/2$, then return $\tilde{S}=S$. Else,
return $\tilde{S}=V-S$.
\end{enumerate}
\caption{\label{alg:BalCut}A reduction from $\protect\BCut$ to $\protect\Cut$}
\end{algorithm}

We will show an equivalent statement of $T_{\BCut}(m,3\phi_{U},\phi_{L})\le O(T_{\Cut}(m,\phi_{U},\phi_{L},\beta)\cdot\frac{1}{\beta})$. 
\begin{proof}
Given $(G,\phi_{U},\phi_{L})$, we run \ref{alg:BalCut}. Observe
that there are at most $O(1/\beta)$ iterations in the while loop.
Otherwise, $\vol_{G}(S)>\vol_{G}/3$. Therefore, the running time
is obvious. It remains to show the correctness.

Let $S_{t}$ be the last cut returned by calling $\Cut(G_{t},\phi_{U},\phi_{L},\beta)$.
Let $S'=\cup_{i\le t-1}S_{i}$. Note that $S=\cup_{i\le t}S_{i}=S'\cup S_{t}$.
Observe that $\vol_{G}(S')\le\vol_{G}/3$ and $\Phi_{G}(S')\le\phi_{U}$
by \ref{prop:union}. We need two small observations.
\begin{claim}
$\delta_{G}(S)\le\phi_{U}\vol_{G}$.
\end{claim}

\begin{proof}
We know $\delta_{G}(S')\le\phi_{U}\vol_{G}(S')$. Also, note that
$\delta_{G_{t}}(S_{t})\le\phi_{U}\vol_{G_{t}}=\phi_{U}\vol_{G}(V-S')$
where this is true either $S_{t}$ is from \ref{enu:CP cut} or \ref{enu:CP prune}
of $\Cut$. So we have 
\begin{align*}
\delta_{G}(S) & \le\delta_{G}(S')+\delta_{G_{t}}(S_{t})\\
 & \le\phi_{U}\vol_{G}(S')+\phi_{U}\vol_{G}(V-S')\\
 & =\phi_{U}\vol_{G}.
\end{align*}
\end{proof}
\begin{claim}
If $\vol_{G}(S)>\vol_{G}/2$, then $\vol_{G}/3\le\vol_{G}(V-S)\le\vol_{G}/2$.
\end{claim}

\begin{proof}
$\vol_{G}(V-S)\le\vol_{G}/2$ follows directly from the assumption.
To see another direction, we have $\vol_{G_{t}}(S_{t})\le\vol_{G_{t}}/2=\vol_{G}(V-S')/2$.
Therefore, 
\begin{align*}
\vol_{G}(S) & \le\vol_{G}(S')+\vol_{G}(V-S')/2\\
 & =\vol_{G}/2+\vol_{G}(S')/2\le(2/3)\vol_{G}.
\end{align*}
\end{proof}
There are four cases: whether $S_{t}$ is from \ref{enu:CP cut} or
\ref{enu:CP prune} of $\Cut$ and whether $\vol_{G}(S)\le\vol_{G}/2$. 

First, suppose $\vol_{G}(S)\le\vol_{G}/2$ and $S_{t}$ is from \ref{enu:CP cut}.
We have $\Phi_{G}(S)\le\phi_{U}$ by \ref{prop:union} and $\vol_{G}/3\le\vol_{G}(S)\le\vol_{G}/2$.
So $\tilde{S}=S$ satisfies the output conditions for \ref{enu:CP cut}
of $\BCut$.

Second, suppose $\vol_{G}(S)\le\vol_{G}/2$ and $S_{t}$ is from \ref{enu:CP prune}.
We claim that $\tilde{S}=S$ satisfies the output conditions for \ref{enu:CP prune}
of $\BCut$. This is because $\Phi_{G-S}=\Phi_{G_{t}-S_{t}}\ge\phi_{L}$
and $\delta{}_{G}(S)\le\phi_{U}\vol_{G}$.

Third, suppose that $\vol_{G}(S)>\vol_{G}/2$ and $S_{t}$ is from
\ref{enu:CP cut}. As $\vol_{G}(S)\le2\vol_{G}(V-S)$, and so
\[
\Phi_{G}(V-S)=\frac{\delta_{G}(S)}{\min\{\vol_{G}(S),\vol_{G}(V-S)\}}\le2\frac{\delta_{G}(S)}{\vol_{G}(S)}\le2\phi_{U}
\]
where the last inequality is by \ref{prop:union}. So $\tilde{S}=V-S$
satisfies the output conditions for \ref{enu:CP cut} of $\BCut$
with parameter $2\phi_{U}$.

Forth, suppose that $\vol_{G}(S)>\vol_{G}/2$ and $S_{t}$ is from
\ref{enu:CP prune}. We have
\[
\delta_{G}(S)\le\phi_{U}\vol_{G}\le3\phi_{U}\vol_{G}(V-S)
\]
by the two claims above. So $\tilde{S}=V-S$ satisfies the output
conditions for \ref{enu:CP cut} of $\BCut$ with parameter $3\phi_{U}$.
\end{proof}

\subsection{Proof of \ref{lem:vBCut from BCut}}

\begin{algorithm}
\begin{enumerate}
\item Let $i\gets1$ and $G_{1}\gets G$. Let $S\gets\emptyset$.
\item While $|S|\le|V|/3$
\begin{enumerate}
\item Let $S'_{i}$ be the cut returned by $\BCut(G_{i},\phi_{L},\phi_{U})$.
\item If $|S'_{i}|\le|V(G_{i})|/4$, then 
\begin{enumerate}
\item \label{enu:return vBCut expander }If $S'_{i}$ is from \ref{enu:CP prune}
of $\BCut$, then return $\tilde{S}=S\cup S'_{i}$.
\item $S_{i}\gets S'_{i}$.
\end{enumerate}
\item Else $|S'_{i}|>|V(G_{i})|/4$, then $S_{i}\gets V(G_{i})-S'_{i}$.
\item $S\gets S\cup S_{i}$
\item $G_{i+1}\gets G_{i}\{V(G_{i})-S_{i}\}$.
\item $i\gets i+1$.
\end{enumerate}
\item \label{enu:return vBCut normal}If $|S|\le|V|/2$, then return $\tilde{S}=S$.
Else, return $\tilde{S}=V-S$.
\end{enumerate}
\caption{\label{alg:vBalCut}A reduction from $\protect\vBCut$ to $\protect\BCut$}
\end{algorithm}

We will show an equivalent statement of $T_{\vBCut}(n,\Delta,60\Delta\phi_{U},\phi_{L})\le O(T_{\BCut}(n\Delta,\phi_{U},\phi_{L})\Delta)$.

\begin{proof}
Given $(G,\Delta,\phi_{U},\phi_{L})$, we run \ref{alg:BalCut}. Observe
that there are at most $t=O(\Delta)$ iterations in the while loop.
This is because at each iteration $i$, we either remove $S'_{i}$
or $V(G_{i})-S'_{i}$ from $G_{i}$. It suffices to show the following:
\begin{align*}
\min\{|S'_{i}|,|V(G_{i})-S'_{i}|\} & \ge\min\{\vol_{G_{i}}(S'_{i}),\vol_{G_{i}}(V(G_{i})-S'_{i})\}/\Delta & (\text{max degree is \ensuremath{\Delta}})\\
 & \ge\vol_{G_{i}}/3\Delta & (S'_{i}\text{ is from }\BCut)\\
 & \ge|V(G_{i})|/3\Delta\\
 & \ge|V|/6\Delta. & (|V(G_{i})|\ge2|V|/3)
\end{align*}
Therefore, the running time is obvious. It remains to show the correctness. 

Suppose that the returned cut $\tilde{S}$ is from Step \ref{enu:return vBCut expander }
of \ref{alg:vBalCut}. In this case, $|S|\le|V|/3$ and so 
\begin{align*}
|\tilde{S}| & =|S|+|S'_{i}|\le|S|+|V-S|/4=3|S|/4+|V|/4\le|V|/2.
\end{align*}
\yp{This is missing left and rights (many other places too)}
Also, $\sigma_{G-\tilde{S}}\ge\Phi_{G_{i}-S'_{i}}\ge\phi_{L}$. So
$\tilde{S}$ satisfies the output conditions for \ref{enu:vCP prune}
of $\vBCut$. 

Now, we assume that $\tilde{S}$ is returned from Step \ref{enu:return vBCut normal}.
In this case, we have $S=\cup_{i\le t}S_{i}$.
\begin{claim}
$\frac{\delta_{G}(S)}{|S|}\le12\Delta\phi_{U}$.
\end{claim}

\begin{proof}
We first analyze $\sigma_{G_{i}}(S_{i})=\sigma_{G_{i}}(S'_{i})$ for
each $i$. There are several cases. Suppose $S'_{i}$ is returned
from \ref{enu:CP cut} of $\BCut$, then by \ref{prop:sparsity vs conductance}
$\sigma_{G_{i}}(S')\le\Delta\Phi_{G_{i}}(S'_{i})\le\Delta\phi_{U}$
and we are done.

Now, we assume that $S'_{i}$ is returned from \ref{enu:CP prune}
of $\BCut$. In this case, we have 
\[
\delta{}_{G_{i}}(S_{i}')\le\phi_{U}\vol_{G_{i}}.
\]
We also have $\vol_{G_{i}}(V(G_{i})-S'_{i})\ge\vol_{G_{i}}/2$, so
\[
|V(G_{i})-S'_{i}|\ge\vol_{G_{i}}(V(G_{i})-S'_{i})/\Delta\ge\vol_{G_{i}}/2\Delta.
\]
As we assume that $\tilde{S}$ is returned from Step \ref{enu:return vBCut normal},
it must be the case that $|S'_{i}|>|V(G_{i})|/4$. So 
\[
|S'_{i}|>|V(G_{i})|/4\ge\vol_{G_{i}}/4\Delta.
\]
Put these together, we have 

\begin{align*}
\sigma_{G_{i}}(S_{i}) & =\frac{\delta{}_{G_{i}}(S_{i}')}{\min\{|S'_{i}|,|V(G_{i})-S'_{i}|\}}\\
 & \le\frac{\phi_{U}\vol_{G_{i}}}{\min\{\vol_{G_{i}}/4\Delta,\vol_{G_{i}}/2\Delta\}}\\
 & \le4\Delta\phi_{U}.
\end{align*}
That is, $\sigma_{G_{i}}(S_{i})\le4\Delta\phi_{U}$ for each $i$.
Given this, we have 

\begin{align*}
\frac{\delta_{G_{i}}(S_{i})}{|S_{i}|} & \le3\cdot\frac{\delta_{G_{i}}(S_{i})}{\min\{|S_{i}|,|V(G_{i})-S_{i}|\}} & (|S_{i}|,|V(G_{i})-S_{i}|\le3|V(G_{i})|/4)\\
 & =3\sigma_{G_{i}}(S_{i})\\
 & \le12\Delta\phi_{U}.
\end{align*}
By applying \ref{prop:union}, this conclude the claim.
\end{proof}
We now use the above claim to prove the lemma. Let $S'=\cup_{i\le t-1}S_{i}$.
Observe that $|S'|\le|V|/3$ and $S_{t}\le\frac{3}{4}|V(G_{t})|=\frac{3}{4}|V-S'|$.
Therefore, 
\[
|S|=|S'|+|S_{t}|\le\frac{|S'|}{4}+\frac{3|V|}{4}\le(\frac{1}{12}+\frac{3}{4})|V|=\frac{5}{6}|V|.
\]
So $|V-S|\ge|S|/5$. Therefore the returned cut $\tilde{S}$ satisfies
$|V|/6\le|\tilde{S}|\le|V|/2$, which in turn implies
\[
\sigma_{G}\left(\tilde{S}\right)
=
\frac{\delta_{G}(S)}{\min\left\{\left|S\right|,\left|V-S\right|\right\}}
\leq
5 \cdot \frac{\delta_{G}\left(S\right)}{\left|S\right|}
\leq
60 \Delta\phi_{U}.
\]
That is, $\tilde{S}$ satisfies the output conditions for
\ref{enu:vCP cut} of $\vBCut$ with parameter $60\Delta\phi_{U}$.
\end{proof}
%

\subsection{Proof of \ref{thm:KKOV}}

We call each iteration $t$ in the for loop of \ref{alg:KKOV} a \emph{round},
and call $M_{t}$ a matching of round $t$. Consider the following
random-walk process along the matchings. Imagine a particle located
at vertex $u$ before inserting $M_{t}$ (i.e. before round $t$).
Suppose there is an edge $(u,v)$ incident to $u$ in the matching
$M_{t}$. Then, the particle stays at $u$ with probability $1/2$
and jumps across $(u,v)$ with probability $1/2$. Let $p_{u,v}(t)$
denote the probability that the particle starting at $u$ reaches
node $v$ after inserting $M_{t}$ (i.e. after $t$ rounds).

Below, we let $V=V(W)$ and $p_{A,B}(t)=\sum_{u\in A,v\in B}p_{u,v}(t)$. 
\begin{prop}[\cite{KhandekarKOV2007cut}]
 We have the following:
\begin{itemize}
\item $p_{u,u}(0)=1$ for all $u$ and $p_{u,v}(0)=0$ for $u\neq v$. 
\item For all $t\ge0$ and $u\in V$, $p_{u,V}(t)=p_{V,u}(t)=1$.
\item For all $t\ge1$, $p_{u,v}(t)=p_{u,w}(t)=\frac{p_{u,v}(t-1)+p_{u,w}(t-1)}{2}$
if $(v,w)\in M_{t}$.
\end{itemize}
\end{prop}

Let $\Psi_{u}(t)=-\sum_{v\in V}p_{u,v}(t)\ln p_{u,v}(t)$ be the \emph{entropy}
of the distribution of the random walks starting from $u$ after $t$
rounds. We call $\Psi(t)=\sum_{u\in V}\Psi_{u}(t)$ the \emph{potential}.
We use the usual convention that $-0\ln0=\lim_{x\rightarrow0^{+}}-x\ln x=0$.
We have:
\begin{prop}[\cite{KhandekarKOV2007cut}]
We have the following: $\Psi(0)=0$ and $\Psi(t)\le n\ln n$ for
any $t$.
\end{prop}

The key observation is that each matching, except the last one, must
significantly increase the potential, which allows us to bound the
number of rounds.
\begin{lem}
\label{lem:potential increase}For each round $t$, if the cut $A_{t}$
is from \ref{enu:vCP cut} of $\BCut$, then $\Psi(t)-\Psi(t-1)=\Omega(n)$.
\end{lem}

\begin{proof}
Note that $|V|/6\le|A_{t}|\le|V|/2$. Let $\overline{A}_{t}=V-A_{t}$.
Observe that $p_{A_{t},\overline{A}_{t}}(t-1)\le|E_{W_{t-1}}(A_{t},\overline{A}_{t})|/2$.
To see this, when an edge $(v,w)\in E_{W_{t-1}}(A_{t},\overline{A}_{t})$
is inserted, there is exactly $1/2$ units of probability mass (summing
up over all starting points) transfers from $v$ to $w$. Moreover,
the edge $(v,w)\in E_{W_{t-1}}(A_{t},\overline{A}_{t})$ is used exactly
once for transferring the probability mass.

As $\sigma_{W_{t-1}}(A_{t})\le1/4$, we have $p_{A_{t},\overline{A}_{t}}(t-1)\le|A_{t}|/8$.
By an averaging argument, there are at least $|A_{t}|/2$ nodes $u\in A_{t}$
where $p_{u,\overline{A}_{t}}(t-1)\le1/4$. Fix such node $u$. It
suffices to prove that $\Psi_{u}(t)-\Psi_{u}(t-1)=\Omega(1)$.
This is because $|A_{t}|=\Omega(n)$,
and the monotonic increase of entropy under averaging implying that
$\Psi_{v}(t)-\Psi_{v}(t-1) \geq 0 $ for any $v \in V$.

Recall that, for each $v\in A_{t}$, there is a unique matching edge
$(v,\pi(v))\in M_{t}$.
Consider the sets
\begin{align*}
\textsc{Good}
& =
\left\{v\in S_{t}\mid p_{u,v}\left(t-1\right)\ge2p_{u,\pi(v)}\left(t-1\right)
\right\}\\
\textsc{Bad}
& =
\left\{v\in S_{t}\mid p_{u,v}\left(t-1\right)<2p_{u,\pi\left(v\right)}\left(t-1\right)
\right\}.
\end{align*}
From the definition, we have
\[
p_{u,\textsc{Bad}}\left(t-1\right)
\leq
2 p_{u,\overline{S}_{t}}\left(t-1\right)\le1/2.
\]
Therefore,
\[
p_{u, \textsc{Good}}\left(t-1\right)
=
p_{u,S_{t}}\left(t-1\right)-p_{u,\textsc{Bad}}\left(t-1\right)
\geq
3/4 -1/2 = 1/4. 
\]

For each $v\in \textsc{Good}$, let $q=p_{u,v}(t-1)$ and $r=p_{u,\pi(v)}(t-1)$,
and $q'=p_{u,v}(t)$ and $r'=p_{u,\pi(v)}(t)$. Note that $q'=r'=(q+r)/2$
and $q\ge2r$. So
\begin{align*}
\left(-q'\ln q'-r'\ln r'\right)
-
\left(-q\ln q-r\ln r\right)
& =
\left(-2\left(\frac{q+r}{2}\right)
\ln\left(\frac{q+r}{2}\right)\right)
-
\left(-q\ln q-r\ln r\right)\\
 & =\Omega\left(q\right).
\end{align*}
Therefore, $\Psi_{u}(t)-\Psi_{u}(t-1)=\Omega(p_{u,\textsc{Good}}(t-1))=\Omega(1)$
as desired. Finally, we prove that $-2\left(\frac{q+r}{2}\right)\ln\left(\frac{q+r}{2}\right)-\left(-q\ln q-r\ln r\right)=\Omega(q)$
when $r\in[0,q/2]$. Observe that this expression is minimized when
$r=q/2$. So we only show that the claim holds when $r=q/2$:
\begin{align*}
-2\left(\frac{q+r}{2}\right)\ln\left(\frac{q+r}{2}\right)-\left(-q\ln q-r\ln r\right) & =-2\left(\frac{3q}{4}\right)\ln\left(\frac{3q}{4}\right)-\left(-q\ln q-\frac{q}{2}\ln\frac{q}{2}\right)\\
& =\frac{q}{2}\ln\left(\frac{3q}{4}\right)^{-3}+\frac{q}{2}\ln q^{2}+\frac{q}{2}\ln\frac{q}{2}\\
& =\frac{q}{2}\ln\frac{4^{3}}{3^{3}2}=\frac{q}{2}\ln\frac{32}{27}=\Omega(q).
\end{align*}
\end{proof}

\begin{lem}
\label{lem:KKOV last round}$\sigma_{W}\ge\phi/9$. So $\Phi_{W}\ge\phi/9R$.
\end{lem}
\begin{proof}
Let $t$ be the first round where the cut $A_{t}$ is from \ref{enu:vCP prune}
of $\BCut$. We know that $t=O(\log n)$ because $\Psi(t)\le n\ln n$
and by \ref{lem:potential increase}. We assume $c_{\KKOV}$ is such
that $R=c_{\KKOV}\log n>t$. We will prove below that $\sigma_{W_{t}}\ge\phi/9$.
This will implies $\sigma_{W}\ge\phi/9$ because $\sigma_{W}$ does
not decrease under edge insertions. By \ref{prop:sparsity vs conductance},
we have $\Phi_{W}\ge\phi/9R$.

Let $(A_{t},\overline{A}_{t})$ be the cut returned by $\vBCut$ from \ref{enu:vCP prune} of \ref{def:vCP}. We have $\sigma_{W_{t-1}\{\overline{A}_{t}\}}\ge\phi$.
Note that, for each node $u\in A_{t}$, there is a matching edge $(u,v)$
in $M_{t}$ where $v\in\overline{A}_{t}$. Consider any cut $(T,\overline{T})$
where $|T|\le|\overline{T}|$. We will show that $\sigma_{W_{t}}(T)\ge\phi/9$.
There are several cases. 

First, suppose that $|T\cap\overline{A}_{t}|\ge3|\overline{T}\cap\overline{A}_{t}|$.
Then,
\[
|\overline{A}_{t}|
=
|T\cap\overline{A}_{t}|
+
|\overline{T}\cap\overline{A}_{t}|
\leq
\frac{4}{3}|T\cap\overline{A}_{t}|
\leq\frac{4}{3}|T|\le\frac{2}{3}|V|.
\]
So $|A_{t}|\ge\frac{1}{3}|V|$ and $|\overline{T}\cap\overline{A}_{t}|\le\frac{1}{3}|T\cap\overline{A}_{t}|\le\frac{1}{6}|V|$.
Therefore, the number of edges of $M_{t}$ connecting $A_{t}$ and
$T\cap\overline{A}_{t}$ is at least 
\[
|A_{t}|-|\overline{T}\cap\overline{A}_{t}|\ge\frac{1}{6}|V|,
\]
which in turn implies that $\sigma_{W}(T)$ is at least $1/3$.

Next, suppose that $|T\cap A_{t}|\ge2|T|/3$. That is, $|T\cap\overline{A}_{t}|\le|T\cap A_{t}|/2$.
Then, the number of edges of $M_{t}$ connecting $T\cap A_{t}$ and
$\overline{T}\cap\overline{A}_{t}$ is at least
\[
|T\cap A_{t}|-|T\cap\overline{A}_{t}|\ge|T\cap\overline{A}_{t}|/2\ge|T|/3,
\]
so
\[
\sigma_{W}(T)\ge\frac{|T|/3}{|T|}\ge1/3. 
\]

The remaining case is when $|T\cap\overline{A}_{t}|\ge|T|/3$ and
$|T\cap\overline{A}_{t}|\le3|\overline{T}\cap\overline{A}_{t}|$.
We claim that $\sigma_{W_{t}}(T)\ge\phi/9$. This is because $\sigma_{W_{t-1}\{\overline{A}_{t}\}}\ge\phi$
and so 
\[
\delta_{W_{t-1}\left\{\overline{A}_{t}\right\}}
        \left(T\cap\overline{A}_{t}\right)
\geq
\phi\min\left\{\left|T\cap\overline{A}_{t}\right|,
        \left|\overline{T}\cap\overline{A}_{t}\right|\right\}
\geq
\phi\left|T\cap\overline{A}_{t}\right|/3
\geq
\phi\left|T\right|/9.
\]
This completes the claim that $\sigma_{W_{t}}\ge\phi/9$.
\end{proof}
%

\subsection{Proof of \ref{lem:slow CA}}
\begin{proof}
It is known that there is a deterministic $\SlowLowCond$ algorithm
(e.g. \cite{LeightonR99}) which, given any graph $H$ with total
weight $W$ and $\phi$, in $O(n^{4})$ either find a cut $S$ where
$\vol_{H}(S)\le\vol_{H}/2$ and $\Phi_{H}(S)\le\phi$, or declare
that $\Phi_{H}\ge\phi/\log W$. 

The algorithm is to iteratively find a sparse cut from $G$ until
we cannot. More formally, we first preprocess $G$ in $O(m)$ so that
$G$ has at most $n^{2}$ weighted edges with total weight $W=m$.
Let $H\gets G$ and $\Shat\gets\emptyset$. As long as $\SlowLowCond(H,\phi/2)$
return a cut $S'$, then we set $H\gets H\{V-S'\}$ and $\Shat\gets S\cup S'$.
Whenever $\vol_{G}(\Shat)\ge\beta\vol_{G}$, we set $S=\Shat$ if
$\vol_{G}(S)\le\vol_{G}/2$, otherwise $S=V-\Shat$. In this case,
clearly $\beta\vol_{G}\le\vol_{G}(S)\le\vol_{G}/2$. We also that
\[
\Phi_{G}(S)=\frac{\delta_{G}(\Shat)}{\min\{\vol_{G}(\Shat),\vol_{G}(V-\Shat)\}}\le2\cdot\frac{\delta_{G}(\Shat)}{\vol_{G}(\Shat)}\le\phi
\]
The first inequality is because $\vol_{G}(V-\Shat)\le2\vol_{G}(S)$
(as $\vol_{H}(S')\le\vol_{H}/2$ in every iteration), and the second
inequality is by \ref{prop:union}. 

Suppose that, before $\vol_{G}(\Shat)\ge\beta\vol_{G}$, there is
an iteration where $\SlowLowCond(H,\phi/2)$ declares that $\Phi_{H}\ge\phi/2$.
Let $A=\Shat$ and $\overline{A}=V-\Shat$. Let $F$ be a set of edges
connecting $A$ and $\overline{A}$ such that $\deg_{F}(v)=\deg_{G}(v)$
for each $v\in A$ and $\deg_{F}(v)\le\deg_{G}(v)$ for $v\in\overline{A}$.
It is obvious how to construct this set. We claim that $\Phi_{G\cup F}\ge\phi/12\log m$.
First, note that for any $S$, $\vol_{G\cup F}(S)\le2\vol_{G}(2)$. 

Consider any cut $(T,\overline{T})$ where $\vol_{G}(T)\le\vol_{G}(\overline{T})$.
There are two cases. The proof is analogous to the one in \ref{lem:KKOV last round}.

Suppose that $\vol_{G}(T\cap A)\ge2\vol_{G}(T)/3$. That is, $\vol_{G}(T\cap\overline{A})\le\vol_{G}(T\cap A)/2$.
Then, the number of edges of $F$ connecting $T\cap A_{t}$ and $\overline{T}\cap\overline{A}$
is at least
\[
\vol_{G}(T\cap A)-\vol_{G}(T\cap\overline{A})\ge\vol_{G}(T\cap\overline{A})/2\ge\vol_{G}(T)/3,
\]
so $\Phi_{G\cup F}(T)\ge\frac{\vol_{G}(T)/3}{\vol_{G\cup F}(T)}\ge1/6$. 

Next, suppose that $\vol_{G}(T\cap\overline{A})\ge\vol_{G}(T)/3$.
Note that $\vol_{G}(T\cap\overline{A})\le\vol_{G}/2$ and $\vol_{G}(\overline{A})\ge2\vol_{G}/3$,
so $\vol_{G}(T\cap\overline{A})\le3\vol_{G}(\overline{T}\cap\overline{A})$.
As $\Phi_{G\{\overline{A}\}}\ge\phi/2\log m$ and so 
\begin{align*}
\delta_{G\{\overline{A}\}}(T\cap\overline{A}) & \ge\frac{\phi}{2\log m}\min\{\vol_{G\{\overline{A}\}}(T\cap\overline{A}_{t}),\vol_{G\{\overline{A}\}}(\overline{T}\cap\overline{A}_{t})\}\\
 & \ge\frac{\phi}{6\log m}\vol_{G}(T\cap\overline{A}_{t})\ge\frac{\phi}{18\log m}\vol_{G}(T).
\end{align*}
So $\Phi_{G\cup F}(T)\ge\frac{\phi\vol_{G}(T)/(18\log m)}{\vol_{G\cup F}(T)}\ge\phi/40\log m$. 

The running time is $O(m+n^{5})$. Indeed, we preprocess $G$ in $O(m)$.
We call $\SlowLowCond$ at most $n$ times. Each time takes at most
$n^{4}$ time.
\end{proof}

\fi

==> recursion.tex <==

\section{A Recursive Algorithm for $\protect\CA$}
\label{sub:CA via vBCut}

\danupon{I have changed 80 to 160 everywhere in this section due to the change in Definition 3.1. Subtle consequences should be checked.}


The  main technical lemma is presented in this section. At a high level, we show that solving $\CA$ can be reduced to solving $\Otil(k)$ instances of $\vBCut$ in graphs whose numbers of edges are smaller by a factor of roughly $k$ and also solving $\Otil(1)$ instances of $\Match$. As $\Match$ admits fast algorithms from \ref{sec:match} and $\vBCut$ can in turn be reduced to $\CA$ as shown in \ref{sec:cut}, this completes the cycle of reductions and gives us a recursive algorithm for $\CA$. From this, we will derive a fast algorithm for $\BCut$ in \ref{sec:BCut_high_cond} as our main result. The formal statement is as follows. (Below we use a constant $c_{\KKOV}$ from \ref{thm:KKOV} which will be stated and proved later in this section.)   
\begin{lem}[$\CA \Rightarrow \vBCut$]
\label{lem:CA recursive}Let $c_{\KKOV}$ and $c_{\match}$ be constants from \ref{thm:KKOV} and \ref{thm:ES match} respectively. There is a small
enough constant $c_{0}$ such that the following holds. 
\begin{enumerate}
\item \label{enu:CA k large}For any $k\ge1$, there is an algorithm for
the $\CA$ problem  that, for any input tuple $(m,\phi_{U},\phi_{L},\beta_{\cut},\beta_{\aug})$ and $R$\danupon{New}
such that 
\[
R\ge c_{\KKOV}\log(2m/k),\cong\ge\frac{c_{\match}\log^{2}2m}{\phi_{U}^{2}},\alpha\le\frac{1}{4},\phi_{L}\le\frac{c_{0}\alpha\phi_{U}}{R^{6}\cong\log m}\text{ and }\beta_{\cut}\le\text{\ensuremath{\beta}}_{\aug}/(330R),
\]
the algorithm has running time
\begin{align*}
T_{\CA}\left(m,\phi_{U},\phi_{L},\beta_{\cut},\beta_{\aug}\right)
& \le kR\cdot T_{\vBCut}\left(2m/k,R,1/4,\alpha\right)\\
 & \ \ \ \ + R\cdot T_{\Match}\left(2m,k,\phi_{U},\cong,160\beta_{\cut}\right)
 +O\left(m+k^{5}\right).
\end{align*}
\item \label{enu:CA k one}There is an an algorithm for the $\CA$ problem
 that, for any input tuple $(m,\phi_{U},\phi_{L},\beta_{\cut},\beta_{\aug})$ and $R$\danupon{New}
such that 
\[
R\ge c_{\KKOV}\log\left(2m\right),
\cong\ge\frac{c_{\match}\log2m}{\phi_{U}},\alpha\le\frac{1}{4},\phi_{L}
\le\frac{c_{0}\alpha}{R^{5}\cong}
\text{ and }
\beta_{\cut}\le\text{\ensuremath{\beta}}_{\aug}/(330R),
\]
the algorithm has running time 
\begin{align*}
T_{\CA}\left(m,\phi_{U},\phi_{L},\beta_{\cut},\beta_{\aug}\right)
 & \le R\cdot T_{\vBCut}\left(2m,R,1/4,\alpha\right)\\
 & \ \ \ \ + R\cdot T_{\Match}\left(2m,1,\phi_{U},\cong,160\beta_{\cut}\right)
 +O\left(m\right).
\end{align*}
\end{enumerate}
\end{lem}

Roughly the first result in \Cref{lem:CA recursive} gives a reduction from $\CA$ on an $m$-edge graph to $\vBCut$ on $kR$ graphs of $2m/k$ edges by solving $\Match$ with parameter $k$ for $R$ times. The second result requires milder conditions. It gives a reduction from $\CA$ to $\vBCut$ on $R$ graphs of $2m$ edges (i.e. the graphs are not smaller) by solving $\Match$ with $k=1$ for $R$ times.\danupon{NEW}
%
Behind these results is an algorithm that tries to \emph{embed} many small expanders
simultaneously into the input graph. 
%
%
The notion of \emph{embedding} is discussed in \ref{subsec:embedding}. The framework which allows us to embed expanders is based on the variant of the \emph{cut-matching game}  by Khandekar, Khot, Orecchia, and Vishnoi
 \cite{KhandekarKOV2007cut} which is discussed in \ref{sec:KKOV}. Finally, we describe our algorithm and its analysis in \ref{sec:main_algo}. 

\subsection{Key Tool 1: Simultaneous Small Expanders Embedding}
\label{subsec:embedding}

\danupon{There is some consistency here and readers might not understand why we use ``path embedding'' instead of just ``embedding''.  The risk of using confusing machine learning people seem lower than confusing a general audience. I propose that we just use ``embedding''.}

In this section, we define a notion of \emph{path embedding}  (or simply {\em embedding}) and  show a key observation in \ref{prop:embed partition} on how to certify that a given graph is expander by only embedding small expanders into it. 

\begin{defn}
        [Embedding]\label{def:embedding}An \emph{embedding $(H,\P)$ into}
        a graph $G=(V,E)$ consists of a graph $H=(V,E')$ and a collection
        of paths $\P$ in $G$ where each edge $e'=(u,v)\in E'$ represents
        a path in $\P$ connecting $u$ and $v$. $(G',\P)$ is called an
        \emph{$c$-congestion} embedding if every edge in $G$ is used by
        at most $c$ paths in $\P$. We also say that $H$ can be embedded
        into $G$ with congestion $c$.\footnote{More generally, to embed $W$ into $G$ usually means to find a multi-commodity
                flow where each commodity corresponds to the endpoints of an edge
                in $W$. In this paper, we can be more specific by finding a collection
                of (integral) paths $\P$.} 
\end{defn}

Observe that if we can embed an expander $H$ into a graph $G$ with small congestion, then $G$ must also be an expander:
\begin{prop}
        \label{prop:embed sparsity}If $H$ can be embedded into $G$ with
        congestion $c$, then $\sigma_{G}\ge\sigma_{H}/c$. 
\end{prop}

\begin{proof}
        Let $(H,\P)$ be an embedding into $G$ with congestion $c$. Consider
        any set $T$ where $|T|\le|V|/2$. It suffices to prove that $\delta_{H}(T)\le c\cdot\delta_{G}(G)$.
        To see this, for each edge $e'\in E_{H}(T,V-T)$, the corresponding
        path $P_{e'}\in\P$ must contains an edge from $E_{G}(T,V-T)$. However,
        each edge in $G$ can be used by at most $c$ many paths. So $\delta_{H}(T)\le c\cdot\delta_{G}(G)$. 
\end{proof}
\ref{prop:embed sparsity} has been the key observation in all previous flow-based algorithms (e.g. \cite{LeightonR99,AroraRV09,KhandekarRV09,KhandekarKOV2007cut,AroraHK10,Sherman09}) for certifying that a given graph is an expander. However, given a graph $G$, we do not know how to embed an expander $H$ of the same size into $G$ deterministically in almost-linear time. 

The following   is the key observation of our algorithm. Suppose we partition nodes of $G$ into $k$ parts $V_1,\dots,V_k$ of equal size, and let $G'$ be the graph after contracting each $V_i$. Let   $H_i$ be an expander whose node set is $V(H_i)=V_i$. So, the size of $H_i$ is smaller than $G$ by roughly a factor of $k$. If we can embed all $H_i$ into $G$ \emph{simultaneously} with low congestion and the contracted graph $G'$ is an expander, then $G$ must also be an expander. Roughly speaking, to certify an expander, the task reduces to embedding small disjoint expanders simultaneously instead of embedding one big expander. 
%
The statement below makes this observation precise:

\danupon{Why it's more convenient to use $\Phi$ instead of $\sigma$?}

\begin{lem}\label{prop:embed partition}
        Let $G=(V,E)$ be a graph with maximum degree $\Delta$. Let $\Vcal=\{V_{1},\dots,V_{k}\}$
        be a partition of $V$. For each $i$, let $H_{i}=(V_i, E_i)$ be a graph on
        vertex set $V_{i}$ with maximum degree $\Delta$. Let $G'$ be obtained
        from $G$ by contracting each $V_{i}$. If $\cup_{i=1}^{k}H_{i}$
        can be embedded into $G$ with congestion $c$, then $\Phi_{G}\ge\Omega(\frac{\Phi_{G'}\cdot(\min_{i}\Phi_{H_{i}})}{\Delta^{3}c})$.
        \yp{$\Phi(G)$?}
\end{lem}

\begin{proof}
        Consider $\Ghat=G\cup(\cup_{i=1}^{k}H_{i})$ (in other words, $\Ghat=(V, E\cup (\cup_{i=1}^{k}E_{i}))$).\danupon{new}
        Observe that $\Ghat$
        can be embedded into $G$ with congestion $c+1$: we can embed edges $\cup_{i=1}^{k}E_{i}$ with congestion $c$ and the rest edges $(u,v)$ in $\Ghat$ can be embedded to edge $(u, v)$ in $G$. 
        Thus, by \ref{prop:embed sparsity},
        \begin{align}
        \sigma_{G} \ge\sigma_{\Ghat}/(c+1)\label{eq:prop:embed sparsity}
        \end{align}
        
        \danupon{New}
        %
        Next, consider
        the inner conductance $\Phi_{\Ghat,\Vcal}^{in}$ and the outer conductance
        $\Phi_{\Ghat,\Vcal}^{out}$ of $\Ghat$ w.r.t.~$\Vcal$ (see the definitions in \Cref{subsec:constant degree}). As $G$ and each $H_i$ have maximum degree $\Delta$,\danupon{I don't see the reason immediately. We should add an explanation.} 
        %$\Phi_{\Ghat,\Vcal}^{in}\ge\min_{i}\Phi_{H_{i}}/\Delta$ and  $\Phi_{\Ghat,\Vcal}^{out}\ge\Phi_{G'}/\Delta$.
        \[
        \Phi_{\Ghat,\Vcal}^{in}\ge\min_{i}\Phi_{H_{i}}/\Delta \mbox{   and   } \Phi_{\Ghat,\Vcal}^{out}\ge\Phi_{G'}/\Delta.
        \]
        \yp{$\Phi(G')$ and $\Phi(H_i)$?}
        By \ref{prop:conductance preserve}, we have that $\Phi_{\Ghat}=\Omega(\Phi_{\Ghat,\Vcal}^{out}\cdot\Phi_{\Ghat,\Vcal}^{in})=\Omega(\Phi_{G'}\cdot(\min_{i}\Phi_{H_{i}})/\Delta^{2})$.
        \yp{$\Phi(\Ghat)$?}
        We can now conclude that
        \begin{align*}
        \Phi_{G} & \ge\sigma_{G}/\Delta & \mbox{(\ref{prop:sparsity vs conductance})}\\
        & \ge\sigma_{\Ghat}/(\Delta(c+1)) & \mbox{(\ref{eq:prop:embed sparsity})}\\
        & =\Phi_{\Ghat}/(\Delta(c+1)) & \mbox{(\ref{prop:sparsity vs conductance})}\\
        & =\Omega\left(\frac{\Phi_{G'}\cdot(\min_{i}\Phi_{H_{i}})}{\Delta^{3}c}\right)
        & \mbox{(\ref{prop:conductance preserve}).} &\qedhere
        \end{align*}
        \yp{$\Phi(G)$ and $\Phi(G')$?}
\end{proof}


\input{KKOV.tex}

\subsection{Algorithm and Analysis}
\label{sec:main_algo}

\paragraph{High-level description.}
The algorithm for \ref{lem:CA recursive} is described in \ref{alg:CA recursive}.
At a high level, \ref{alg:CA recursive} works as follows when $k>1$. We first apply \ref{prop:reduc constant degree} and assume that the given graph $G=(V,E)$ has constant degree. Then, we partition $V$ into $k$ parts equally, $V_1,\dots,V_k$. As suggested by \ref{prop:embed partition}, we will try to embed $k$ expanders simultaneously into these $k$ parts. To do this, we implement the cut-matching game from \ref{sec:KKOV} on each part. That is, we first initialize $W_i$ as an empty graph on vertex set $V_i$. For each round of the cut-matching game, we invoke $\vBCut$ to find a vertex-balanced sparse cut in each $W_i$ (independently), which defines the sets $A_i,B_i \subset V_i$. The goal now is to embed a matching $M_i$ between nodes from $A_i$ and $B_i$ simultaneously for all $i$. The $\ESMatch$ algorithm from \ref{thm:ES match} is exactly designed for this. If $\ESMatch$  returns a balance sparse cut, then we return such cut and terminate. Otherwise, it returns a collection $\P$ of  paths which corresponds $k$ matchings $M_1,\dots,M_k$ and $\cup_i M_i$ can be embedded into $G$ with small congestion. So, we set $W_i \gets W_i \cup M_i$. Therefore, after $O(\log m)$ rounds, we conclude using \ref{thm:KKOV} that each $W_i$ is an expander. Moreover, $\cup_i W_i$ can be embedded into $G$ with small congestion as desired. 

There is a small issue in the above argument because $\ESMatch$ does not guarantee that all nodes from $A_i$ and $B_i$ are matched in $M_i$ as required by  \ref{thm:KKOV}.
Fortunately, only a small fraction of nodes from $\cup_i (A_i \cup B_i)$ is not matched. So, we can fix this simply by augmenting $M_i$ with a set of edges $F_i$ in each round so that every node $A_i \cup B_i$ is matched. We then set $W_i \gets W_i \cup( M_i\cup F_{i})$ in each round, and so  $W_i$ is an expander after $O(\log m)$ rounds. We let $F^{in}$ denote all the ``fake'' matching edges augmented into all $M_i$ in all rounds. Although $\cup_i W_i$ might not be embeddable into $G$ because of $F^{in}$, we still have that $\cup_i W_i$ can be embedded into $G\cup F^{in}=(V, E\cup F^{in}$ with small congestion. 

Next, we let $G'$ be the graph after contracting each $V_{i}$. As $G'$ only has $k$ nodes and we are willing to spend $\poly(k)$ time, we can invoke any polynomial-time algorithm on $G'$. If there is a balanced sparse cut $S'$ in $G'$, then we return the corresponding cut $S$ in $G$ and terminate. Otherwise, we can find $F'$ where $G'\cup F'$ is an expander. We let $F^{out}$ be obtained from $F'$ after ``uncontraction'' (defined formally in \ref{enu:uncontract F} of \ref{alg:CA recursive}).
By \ref{prop:embed partition},
we can conclude that $G\cup F^{in} \cup F^{out}$ is an expander. So we return $F^{in} \cup F^{out}$ as an output for the $\CA$ problem.
See \ref{alg:CA recursive} for the formal description.


\begin{algorithm}
\underline{Input}: An $m$-edge graph $G=(V,E)$ and parameters $(\phi_{U},\phi_{L},\beta_{\cut},\beta_{\aug})$
satisfying the conditions in \ref{lem:CA recursive}.

\underline{Output}: As in \Cref{def:CA}, either
\begin{enumerate}[noitemsep,nolistsep]
\item a set $S\subset V$ such that $\beta_{\cut}\vol_{G}\le\vol_{G}(S)\le\vol_{G}/2$
and $\Phi_{G}(S)\le\phi_{U}$, or 
\item a set $F$ of edges where $|F|\le\beta_{\aug}\vol_{G}$ and $\Phi_{G\cup F}\ge\phi_{L}$.
\end{enumerate}
\underline{Algorithm}: 
\begin{enumerate}[noitemsep]
\item Invoke the algorithm in \ref{prop:reduc constant degree} so we can assume that $G$ is an $n$-node
graph with maximum degree 20 and $n\le2m$.\danupon{$n\leq 2m$ is not in \ref{prop:reduc constant degree}.}
\item Partition $V$ into $V_{1},\dots,V_{k}$ where $n/2k\le|V_{i}|\le n/k$.
\item Set $W_{i}$ as an empty graph on vertex set $V_{i}$ for each
$1\le i\le k$. Set $F^{in}\gets\emptyset$.
\item \label{enu:Cut recursive repeat loop}Repeat $R$ iterations:
\begin{enumerate}[noitemsep]
\item \label{enu:run vBalCut}For each $1\le i\le k:$
\begin{enumerate}[noitemsep]
\item $A_{i}\gets\vBCut(W_{i},R,1/4,\alpha)$. 
\item $B_{i}$ be a subset of $V_{i}-A_{i}$ where $|B_{i}|=|A_{i}|$.
\end{enumerate}
\item \label{enu:run Match}Run $\Match(G,\phi_{U},\cong,160\beta_{\cut},\{A_{1},B_{1},\dots,A_{k},B_{k}\})$
(using \ref{thm:ES match} when $k>1$ and \ref{thm:push match} when
$k=1$):
\item \label{enu:ret cut-match}If \Cref{enu:run Match} returns a cut $S$, then return $S$. (The algorithm then terminates.)\\
Else, do the following.
\begin{enumerate}[noitemsep]
\item Let $M_{1},\dots,M_{k}$ be the matchings returned from \Cref{enu:run Match}. 
\item For each $1\le i\le k$:
\begin{enumerate}
\item Let $F_{i}$ be an arbitrary set of edges such that $M_{i}\cup F_{i}$
is a matching between $A_{i}$ and $B_{i}$ of size $|A_{i}|$.
\item $W_{i}\gets W_{i}\cup(M_{i}\cup F_{i})$, $F^{in}\gets F^{in}\cup F_{i}$. 
\end{enumerate}
\end{enumerate}
\end{enumerate}
\item \label{enu:contract}$G'\gets G/V_{1}/V_{2}\dots/V_{k}$, i.e. $G'=(V', E')$ is the graph after contracting each $V_{i}$ into a vertex $v_{i}$.
\item \label{enu:run slowCA}Run $\SlowCA(G',\phi_{U},\beta_{\cut})$ (using
\ref{lem:slow CA}):\danupon{There should be 5 parameters}
%\begin{enumerate}[noitemsep]
\item \label{enu:ret cut-contract}If \Cref{enu:run slowCA} returns a cut $S'\subset V(H)$,
return $S\gets\cup_{v_{i}\in S'}V_{i}$. (The algorithm then terminates.)\\
Else (a set $F'\subseteq V'\times V'$ of edges (not necessarily in $G'$) is returned), do the following.
\begin{enumerate}[noitemsep]
\item \label{enu:uncontract F}Let $F^{out}$ be an arbitrary set of edges such that $\deg_{F^{out}}(v)=O(1)$
for each $v\in V$ and $\vol_{F^{out}}(V_{i})=\vol_{F'}(v_{i})$ for
each $v_{i}\in V(H)$.\danupon{How can $F^{out}$ exist if we don't restrict that $\deg_{F'}(v_i)=O(\log n)$?}
\item Return $F=F^{in}\cup F^{out}$.
%\end{enumerate}
\end{enumerate}
\end{enumerate}
\caption{\label{alg:CA recursive}Algorithm for $\protect\CA$ using $\vBCut$
(\ref{lem:CA recursive}; \ref{def:CA})}
\end{algorithm}

The algorithm description is the same when $k=1$. The only difference is that we invoke $\PushMatch$ from \ref{thm:push match}
instead of $\ESMatch$ for the  improved quality and running time.
Note that when $k=1$, the graph $G'$ from \ref{enu:contract}
of \ref{alg:CA recursive} is a singleton.

\paragraph{Analysis.}
%Before analyzing \ref{alg:CA recursive}, 
We first state the following algorithm for \ref{enu:run slowCA} of \ref{alg:CA recursive}.\danupon{Thatchaphol will move the lemma below to the front. Thatchaphol will distinguish fonts for algorithms and problems.}
\begin{lem}
\label{lem:slow CA}There is an algorithm called $\SlowCA$ for solving
the $\CA$ problem that, given $(G,\phi,\beta)$ where $G=(V,E)$
is an $n$-node $m$-edge (multi)-graph, $\phi\in[0,1]$ and $\beta\le1/3$,
in time $O(m+n^{5})$ returns either 
\begin{enumerate}
\item a set $S\subset V$ such that $\beta\vol_{G}\le\vol_{G}(S)\le\vol_{G}/2$
and $\Phi_{G}(S)\le\phi$, or 
\item a set $F\subseteq V\times V$ of edges (not necessarily in $E$) where $|F|\le\beta\vol_{G}$ and $\Phi_{G\cup F}\ge\phi/40\log m$.\danupon{How can we avoid the readers from confusing between edges in the graph and additional edges? Perhaps we can use a term like ``link''?}
\end{enumerate}
\end{lem}

This lemma is obtained iteratively applying a deterministic polynomial-time
approximate low-conductance cut algorithm (e.g. \cite{LeightonR99})
and removing the returned cuts from $G$ until we cannot. The proof
is straightforward and is deferred to the Appendix. We note that if
$G$ is a singleton, then $\SlowCA$ returns $F=\emptyset$.
In particular, when $k=1$, we have $F^{out}=\emptyset$ in \ref{alg:CA recursive}.

The running time of \ref{alg:CA recursive} is straightforward. Note
that $m\le n\le2m$. The total time \ref{enu:run vBalCut} takes is
$kR\cdot T_{\vBCut}(2m/k,R,1/4,\alpha)$. The total time \ref{enu:run Match}
takes is $R\cdot T_{\Match}(2m,k,\phi_{U},\cong,160\beta_{\cut})$.
Note that we have $\cong\ge\frac{c_{\match}\log^{2}2m}{\phi_{U}^{2}}$
when $k>1$ and $\cong\ge\frac{c_{\match}\log2m}{\phi_{U}}$ when
$k=1$. So the conditions for calling $\ESMatch$ from \ref{thm:ES match}
and the conditions for calling $\PushMatch$ from \ref{thm:push match} are indeed satisfied.
\ref{enu:run slowCA} takes $O(m+k^{5})$ time by \ref{lem:slow CA}.
Other steps clearly takes $O(m)$ time.

Now, we proof the correctness. First, by the guarantees of \ref{def:CM}
and \ref{lem:slow CA}, observe that the following:
\begin{lem}
If \ref{alg:CA recursive} returns a set $S$ from \ref{enu:ret cut-match}
or \ref{enu:ret cut-contract}, then $\beta_{\cut}\vol_{G}\le\vol_{G}(S)\le\vol_{G}/2$
and $\Phi_{G}(S)\le\phi_{U}$. 
\yp{$\phi_G(S)$?}
\end{lem}

We also have:
\begin{lem}
\label{lem:fake bound}$|F^{in}|\le320R\beta m$\danupon{Changed because of 80 vs 160} and $|F^{out}|\le\beta_{\cut}m$.
So $|F|\le\beta_{\aug}m$.
\end{lem}

\begin{proof}
In each iteration of \ref{enu:Cut recursive repeat loop} of \ref{alg:CA recursive},
we have that $|\cup_{i=1}^{k}F_{i}|\le160\beta_{\cut}n$ by \ref{def:CM}.
As there are $R$ iterations and $n\le2m$, we have $|F^{in}|\le320R\beta_{\cut}m$.\danupon{Changed because of 80 vs 160}
Also, $|F^{out}|\le\beta_{\cut}m$ by \ref{lem:slow CA}. So we have
$|F|\le330R\beta_{\cut}m\le\beta_{\aug}m$.\danupon{Now 170 becomes 330 everywhere.}
\end{proof}
Now, we need the notion of embedding from \ref{subsec:embedding}. Observe
the following:
\begin{lem}
\label{lem:embed W}$\cup_{i=1}^{k}W_{i}$ can be embedded into $G\cup F^{in}$
with congestion $R\cdot\cong$.
\end{lem}

\begin{proof}
For each iteration of the repeat loop at \ref{enu:Cut recursive repeat loop},
the matchings $M_{1},\dots,M_{k}$ returned are such that $\cup_{i=1}^{k}M_{i}$
can be embedding into $G$ with congestion $\cong$. This is true
by the definition of the matchings from \ref{def:CM}. The claim follows
because there are at most $R$ iterations.
\end{proof}
The remaining part is to prove the following:
\begin{lem}
\label{lem:G conduct}$\Phi_{G\cup F^{in}\cup F^{out}}\ge\phi_{L}$.
\yp{$\Phi(G\cup F^{in}\cup F^{out})$?}
\end{lem}

\begin{proof}
First, we claim that $\min_{i}\Phi_{W_{i}}\ge\alpha/9R$. Observe
that the way \ref{alg:CA recursive} inserts matchings into each $W_{i}$ is exactly
the same way as how \ref{alg:KKOV} works. As we find the set $A_{i}$
and $B_{i}$ by invoking $\vBCut(W_{i},R,1/4,\alpha)$, \ref{thm:KKOV}
implies that $\Phi_{W_{i}}\ge\alpha/9R$ for each $i$. 

Let $\Ghat$ be obtained from $G\cup F^{in}\cup F^{out}$ by contracting
$V_{1},\dots,V_{k}$. As $\cup_{i=1}^{k}W_{i}$ can be embedded into
$G\cup F^{in}$ with congestion $R\cdot\cong$ by \ref{lem:embed W}
and the maximum degree of both $G\cup F^{in}\cup F^{out}$ and $W_{i}$
is $O(R)$, by \ref{prop:embed partition}, we have 
\begin{align*}
\Phi_{G\cup F^{in}\cup F^{out}} & \ge\Omega(1)\cdot\frac{\Phi_{\Ghat}\cdot(\min_{i}\Phi_{W_{i}})}{R^{4}\cong}\\
 & \ge\Omega(1)\cdot\frac{\alpha\cdot\Phi_{\Ghat}}{R^{5}\cong}.
\end{align*}
\yp{$\Phi(G\cup F^{in}\cup F^{out})$? and $\Phi(\Ghat)$?}
There are two cases. If $k=1$, then $\Phi_{\Ghat}=1$ as $\Ghat$ is a singleton. In this case,
as we assume that $\phi_{L}\le c_{0}\alpha/(R^{5}\cong)$ where $c_{0}$
is small enough. So $\Phi_{G\cup F^{in}\cup F^{out}}\ge\phi_{L}$. 

Now, we consider the case when $k>1$. Observe that $G'\cup F'$ is
the graph $G\cup F^{out}$ after contracting $V_{1},\dots,V_{k}$. By \ref{lem:slow CA},
$\SlowBCut$ guarantees $\Phi_{G'\cup F'} \ge\phi_{U}/40R\log m$.
 \yp{$\Phi(G' \cup F')$?}
 As  each node is incident to at most $R$ edges from $F^{in}$,
 $\Phi_{\Ghat}\ge\Phi_{G'\cup F'}/R \ge \phi_{U}/40R\log m$.
\yp{$\Phi(\Ghat)$ and $\Phi(G'\cup F') / R$? In particular, the $/R$
	is division, not a set operation?}
 As $\phi_{L}\le c_{0}\alpha\phi_{U}/(R^{6}\cong\log m)$
where $c_{0}$ is small enough. We conclude  $\Phi_{G\cup F^{in}\cup F^{out}}\ge\phi_{L}$ as well in this case. 
\yp{$\Phi(G\cup F^{in}\cup F^{out})$?}
\end{proof}
We summarize the property of our algorithm when $k=1$ in the following remark. We will need this later in \ref{sec:BCut_nophi}.
\begin{rem}
\label{rem:embedding k one}When $k=1$, in the case the set $F$
is returned, we have that \ref{alg:CA recursive} computes the graph
$W_{1}$ where $\Phi_{W_{1}}\ge\alpha/9R$, \yp{$\Phi(W_1)$?} $E(W_{i})\supset F$,
and $W_{1}$ can be embedded into $G\cup F$ with congestion $R\cdot\cong$.
Moreover, $\max_{\emptyset\neq S\subset V}\{\frac{\vol_{W}(S)}{\vol_{G}(S)},\frac{\vol_{G}(S)}{\vol_{W}(S)}\}\le R=O(\log m)$
because the max degree of both $W_{1}$ and $G$ are at most $R$\@. 
\end{rem}

\begin{comment}
Next, we consider $\Ghat=G\cup(\cup_{i=1}^{k}W_{i})\cup F^{out}$
and show two claims about $\Ghat$ below:
\begin{claim}
\label{lem:Ghat embed}$\Ghat$ can be embedded into $G\cup F^{in}\cup F^{out}$
with congestion $R\cdot\cong$+1.
\end{claim}

\begin{proof}
For each iteration of the repeat loop at \ref{enu:Cut recursive repeat loop},
the matchings $M_{1},\dots,M_{k}$ returned are such that $\cup_{i=1}^{k}M_{i}$
can be embedding into $G$ with congestion $\cong$. This is true
by the definition of the matchings from \ref{def:CM}. Consequently,
after $R$ iterations of \ref{enu:Cut recursive repeat loop} in \ref{alg:CA recursive},
we have that $\cup_{i=1}^{k}W_{i}$ can be embedded into $G\cup F^{in}$
with congestion $R\cdot\cong$. In particular, $\Ghat=G\cup(\cup_{i=1}^{k}W_{i})\cup F^{out}$
can be embedded into $G\cup F^{in}\cup F^{out}$ with congestion $R\cdot\cong+1$.
\end{proof}
\begin{claim}
\label{lem:Ghat conduct}$\Phi_{\Ghat}=\Omega(\frac{\phi_{L}\gamma}{R}\cdot\frac{\phi_{U}}{\log m})$.
If $k=1$, then $\Phi_{\Ghat}=\Omega(\frac{\phi_{L}\gamma}{R})$.
\end{claim}

\begin{proof}
Let $\P=\{V_{1},\dots,V_{k}\}$ be a partition of $V$. Consider any
$S\subset V_{i}$, we have $\delta_{\Ghat[V_{i}]}(S)\ge\delta_{W_{i}}(S)$
and 
\[
\vol_{W_{i}}(S)\le\vol_{\Ghat[V_{i}]}(S)\le\vol_{W_{i}}(S)+\vol_{G\cup F^{out}}(S)\le\vol_{W_{i}}(S)+O(S)
\]
because both $G$ and $F^{out}$ has constant maximum degree. Therefore,
$\Phi_{\Ghat[V_{i}]}(S)=\Omega(\Phi_{W_{i}}(S))$ for each $S\subset V_{i}$
and each $i$. Hence, $\Phi_{\Ghat,\P}^{in}=\Omega(\min_{i}\Phi_{W_{i}})$. 

Next, consider any $S\subset V$ respecting $\P$. We have $\delta_{\Ghat}(S)=\delta_{G\cup F^{out}}(S)$
and also 
\[
\vol_{G\cup F^{out}}(S)\le\vol_{\Ghat}(S)\le\vol_{G\cup F^{out}}(S)+\vol_{(\cup_{i=1}^{k}W_{i})}(S)\le\vol_{G\cup F^{out}}(S)+O(R|S|)
\]
because each $W_{i}$ has maximum degree $R$. Therefore, $\Phi_{\Ghat}(S)=\Omega(\Phi_{G\cup F^{out}}(S)/R)$
for each $S$ respecting $\P$ implying that $\Phi_{\Ghat,\P}^{in}=\Omega(\Phi_{G'\cup F'}/R)$.

By \ref{thm:KKOV}, we have $\Phi_{W_{i}}\ge\phi_{L}\gamma/9R$ and,
by \ref{lem:slow CA}, we have $\Phi_{G'\cup F'}\ge\phi_{U}/40\log m$.
Therefore, by \ref{prop:conductance preserve}, we have $\Phi_{\Ghat}=\Omega(\Phi_{\Ghat,\P}^{in}\cdot\Phi_{\Ghat,\P}^{out})=\Omega(\frac{\phi_{L}\gamma}{R}\cdot\frac{\phi_{U}}{\log m})$.
Note that if $k=1$, then $\Phi_{\Ghat}=\Phi_{\Ghat,\P}^{in}=\Omega(\frac{\phi_{L}\gamma}{R}).$
\end{proof}

\paragraph{Proof of \ref{lem:G conduct}.}

With the above claims, we conclude the proof of \ref{lem:G conduct}:
\begin{align*}
\Phi_{G\cup F^{in}\cup F^{out}} & \ge\sigma_{G\cup F^{in}\cup F^{out}}/20 & (\ref{prop:sparsity vs conductance})\\
 & =\Omega(\sigma_{\Ghat}/(R\cdot\cong)) & (\ref{prop:embed sparsity}\text{ and }\ref{lem:Ghat embed})\\
 & =\Omega(\Phi_{\Ghat}/(R\cdot\cong)) & (\ref{prop:sparsity vs conductance})\\
 & =\Omega(\frac{\phi_{L}\gamma}{R}\cdot\frac{\phi_{U}}{\log m}\cdot\frac{1}{R\cdot\cong}) & (\ref{lem:Ghat conduct})\\
 & \ge\phi_{L} & (c_{0}\text{ is large enough and \ensuremath{\gamma\ge}\ensuremath{\ensuremath{c_{0}\cong\cdot\phi_{U}^{-1}R^{2}\log}m}}).
\end{align*}
In the case when $k=1$, we have
\begin{align*}
\Phi_{G\cup F^{in}\cup F^{out}} & =\Omega(\Phi_{\Ghat}/(R\cdot\cong))\\
 & =\Omega(\frac{\phi_{L}\gamma}{R}\cdot\frac{1}{R\cdot\cong}) & (\ref{lem:Ghat conduct})\\
 & \ge\phi_{L} & (c_{0}\text{ is large enough and \ensuremath{\gamma\ge}\ensuremath{\ensuremath{c_{0}\cong\cdot R^{2}}}}\text{ when \ensuremath{k=1}}).
\end{align*}
\end{comment}



==> weighted.tex <==
%%%%% BEGIN Jason's macros %%%%%
%\newcommand{\f}{\displaystyle\frac}
\newcommand{\f}{\frac}
\newcommand{\cd}{\cdot}
\newcommand{\bn}{\binom}
\newcommand{\sr}{\sqrt}
\newcommand{\cds}{\cdots}
\newcommand{\lds}{\ldots}
\newcommand{\vds}{\vdots}
\newcommand{\dds}{\ddots}
\newcommand{\pge}{\succeq}
\newcommand{\ple}{\preceq}
\newcommand{\sm}{\setminus}
\newcommand{\s}{\subseteq}
\newcommand{\su}{\supseteq}

\newcommand{\sumni}{\sum_{n=1}^\infty}
\newcommand{\sumin}{\sum_{i=1}^n}
\newcommand{\bigcupni}{\bigcup_{n=1}^\infty}
\newcommand{\bigcupin}{\bigcup_{i=1}^n}
\newcommand{\bigcapni}{\bigcap_{n=1}^\infty}
\newcommand{\bigcapin}{\bigcap_{i=1}^n}

\newcommand{\BE}{\begin{enumerate}}
\newcommand{\EE}{\end{enumerate}}
\newcommand{\im}{\item}
\newcommand{\BI}{\begin{itemize}}
\newcommand{\EI}{\end{itemize}}
\def\BAL#1\EAL{\begin{align*}#1\end{align*}}
\def\BALN#1\EALN{\begin{align}#1\end{align}}
\def\BG#1\EG{\begin{gather}#1\end{gather}}

\newcommand{\Sum}{\displaystyle\sum\limits}
\newcommand{\Prod}{\displaystyle\prod\limits}
\newcommand{\Int}{\displaystyle\int\limits}
\newcommand{\Lim}{\displaystyle\lim\limits}
\newcommand{\Max}{\displaystyle\max\limits}
\newcommand{\Min}{\displaystyle\min\limits}

\newcommand{\logn}{\log n}

\newcommand{\dx}{\frac d{dx}}
\newcommand{\dy}{\frac d{dy}}
\newcommand{\dz}{\frac d{dz}}
\newcommand{\dt}{\frac d{dt}}

\newcommand{\inv}{^{-1}}

\newcommand{\R}{\mathbb R}
\newcommand{\Z}{\mathbb Z}
\newcommand{\F}{\mathbb F}
\newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\Q}{\mathbb Q}

\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\el}{\ell}

\newcommand{\Ra}{\Rightarrow}

\newcommand{\lf}{\lfloor}
\newcommand{\rf}{\rfloor}
\newcommand{\lc}{\lceil}
\newcommand{\rc}{\rceil}

\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left[}
\newcommand{\rb}{\right]}
\newcommand{\lmt}{\left[\begin{matrix}}
\newcommand{\rmt}{\end{matrix}\right]}


\newcommand{\BT}{\begin{theorem}}
\newcommand{\ET}{\end{theorem}}
\newcommand{\BL}{\begin{lem}}
\newcommand{\EL}{\end{lem}}
\newcommand{\BD}{\begin{defn}}
\newcommand{\ED}{\end{defn}}

\newcommand{\BP}{\begin{proof}}
\newcommand{\EP}{\end{proof}}

\newcommand{\tO}{\tilde{O}}

\newcommand{\thml}[1]{\label{thm:#1}}
\newcommand{\thmm}[1]{\Cref{thm:#1}}
\newcommand{\leml}[1]{\label{lem:#1}}
\newcommand{\lemm}[1]{\Cref{lem:#1}}
\newcommand{\defnl}[1]{\label{def:#1}}
%\newcommand{\defn}[1]{\Cref{def:#1}}
%%%%% END Jason's macros %%%%%
\newcommand{\para}{\paragraph}
%\renewcommand{\emph}[1]{\textbf{\textup{#1}}}
\newcommand{\bd}{\mathbf d}
\newcommand{\WBCut}{\textsf{\textup{WeightedBalCutPrune}}}
\newcommand{\weighted}{\texttt{\textup{WeightedBalCut}}}
\newcommand{\rooted}{\texttt{\textup{RootedTreeBalCut}}}

\section{Weighted \BCut and  Expander Decomposition}


\BD[Weighted Sparsity]
Consider a weighted graph $G=(V,E)$ and a nonzero vector $\bd\in\R^V_{\ge0}$ of nonnegative entries on the vertices (the ``demands''). The \emph{$\bd$-sparsity} $\Psi^\bd_{G}(S)$ of a subset $S\s V$ with $0<\bd(S)<\bd(V)$ is
\[ \Psi_G^\bd(S)= \f{w(E(S,V\sm S))}{\min\{\bd(S),\bd(V\sm S)\}} .\]
The \emph{$\bd$-sparsity} $\Psi^\bd(G)$ of $G$ is $\min_{S:0<\bd(S)<\bd(V)}\Psi_G^\bd(S)$.
\ED

Our main theorem in this section is a weighted version of \BCut, both in terms of graph edge weights and the demands $\bd$, defined below.

\begin{defn}[$\WBCut$ problem]    
        The input to the $\alpha$-approximate $\WBCut$ problem is a graph $G=(V,E)$, a nonzero vector $\bd\in\R^V_{\ge0}$ of demands, a sparsity parameter $0<\psi\leq 1$, and an approximation factor $\alpha$. The goal is to compute a cut $(A,B)$ in $G$, 
        with $w_G(A,B)\leq \alpha \phi\cdot \bd(V)$, such that one of the following hold:
        either 
        %       Let $\Cut$ be an routine that, given $(G,\phi_{U},\phi_{L},\beta)$
        %       where $G=(V,E)$ is an $m$-edge graph, $\phi_{U},\phi_{L}\in[0,1]$
        %       where $\phi_{L}\le\phi_{U}$ and $\beta\le1/3$, returns either 
        \begin{enumerate}[noitemsep]
                \item \textbf{(Cut)} $\bd(A),\bd(B)\ge \bd(V)/3$; or
                \item \textbf{(Prune)} $\bd(A)\geq \bd(V)/2$, and $\Psi^\bd(G[A])\ge\psi$.
        \end{enumerate}
\end{defn}


\BT\thml{WBCut}
        There is a deterministic algorithm, that, given a graph $G=(V,E)$ with $m$ edges and edge weights in $[1,U]$, demands $\bd(v)\in\{0\}\cup [1,U]$ for all $v\in V$ that are not all zero,
        and parameters $0<\psi\leq 1$ and $r\geq 1$, solves the $(\log^{O(r^4)}m)$-approximate $\WBCut$ problem in time $m\cd(mU)^{O(1/r)}$.
\ET

From \thmm{WBCut}, we have the following immediately corollary, whose proof follows similarly from that of \Cref{cor:expander decomp}; the main difference is that there are $O(\log (mU))$ levels of recursion instead of $O(\log m)$.
\begin{cor}
There is an algorithm that, given a graph
$G=(V,E)$ with $m$ edges and edge weights in $[1,U]$, demands $\bd(v)\in\{0\}\cup[1,U]$ for all $v\in V$ that are not all zero,
        and a parameter $\epsilon\in(0,1]$, returns
a $\left(\epsilon,\epsilon/ \big( \log^{O(r^4)}m \log U \big) \right)$-expander decomposition
of $G$ in time $m\cd(mU)^{O(1/r)}$. 
%\jl{improved approx would be $\lp \eps,\eps/ \big( (\log m)^{O(r^4)} \log U \big) \rp$ I think.}
\end{cor}

%\BT[$(\psi,\bd)$-expander decomposition]\thml{exp}
%Given a graph $G=(V,E)$ and subset $R\s V$, there is a deterministic algorithm running in $m^{1+o(1)}$ time that partitions $V$ into subsets $V_1,\lds,V_\el$ such that
% \BE
% \im For each $i\in[\el]$, define the demands $\bd_i\in\R^{V_i}_{\ge0}$ as $\bd_i(v)=\bd(v)+w(E(\{v\},V\sm V_i))$ for all $v\in V_i$. Then, the graph $G[V_i]$ is a $(\psi,\bd_i)$-expander.
% \im The total weight $w(E(V_1,\lds,V_\el))$ of inter-cluster edges is $\psi n^{o(1)}\bd(V)$.
% \EE
%\ET

\subsection{Weighted Most-Balanced Sparse Cut}

\BD[$(\psi^*,c)$-most-balanced $(\psi,\bd)$-sparse cut]\label{def:most-balanced-s}
Given a graph $G=(V,E)$ and parameters $\psi,\psi^*,c$, a set $S\s V$ with $\bd(S)\le\bd(V)/2$ is a \emph{$(\psi^*,c)$-most-balanced $(\psi,\bd)$-sparse cut} if it satisfies:
 \BE
 \im $w(S,V\sm S)\le\psi\cd\min\{\bd(S),\bd(V\sm S)\}$.
 \im Let $S^*\s V$ be the set with maximum $\bd(S^*)$ out of all sets $S'$ satisfying $w(S',V\sm S')\le\psi\cd\min\{\bd(S'),\bd(V\sm S')\}$ and $\bd(S')\le\bd(V)/2$. Then, $\bd(S)\ge\bd(S^*)/c$.
 \EE
\ED
\thatchaphol{should we define most-balanced sparse cut in \Cref{sec:most-bal cut} and here more consistently?} \jl{this section seems to do better with this minimization version (instead of a decision version given a threshold $z$). we could state this is a minimization version of \Cref{sec:most-bal cut} definition}

Our algorithm for computing the weighted most-balanced sparse cut is a modification of the algorithm in Section~8~of~\cite{GaoLNPSY19}, and is based on decomposing the input graph into \emph{$j$-trees}~\cite{Madry10}. In particular, the algorithms $\weighted$ and $\rooted$ presented below are direct modifications of Algorithm~4 and Algorithm~5 in Section~8~of~\cite{GaoLNPSY19}, respectively.

Recall the definition of $j$-trees from \Cref{def:jtree}. In addition, for a $j$-tree $H$ and a vertex $v\in V_H$ on peripheral tree $T$, we define $c_H(v)$ as the unique vertex shared by $T$ and the core. %Throughout the algorithm, we make the convention that the input graph $G$ has $m$ edges, and the \emph{original} graph has $m_0$ edges.

% Comment out since j-tree already in Sec 6.5
\iffalse
\BD[$j$-tree]
A graph $G=(V,E)$ is a \emph{$j$-tree} if there exists a subset $K\s V$ of $j$ vertices, called the \emph{core}, such that $E\sm E(G[K])$ is a forest.
\ED

\begin{theorem}
        [\cite{Madry10} Paraphrased]
\thml{madry}
Let $G=(V,E)$ be a graph with $n$ vertices, $m$ edges, and capacity ratio $U$. For any parameter $t\ge1$, there is a deterministic algorithm running in $\tO(tm)$ time that outputs graphs $G_1,\lds,G_\el$ on vertices $V$ and subsets $K_1,\lds,K_t\s V$ such that:
\BE
\im For each $i\in[t]$, the graph $G_i$ is a $\tO(\f{m\log U}t)$-tree with core $K_i$, has capacity ratio at most $O(mU)$.
%\im For each $i\in[t]$, $|K_i|\le (\f{m\log U}t)$ and $G_i\sm G_i[K]$ is a forest. The set $K_i$ is called the \emph{core} of $G_i$.
\im There exists a universal function $\be(x)=O(\log^3x)$ such that for each subset $C\s V$,
 \BE
 \im $w(E_{G}(C,V-C))\le w( E_{G_{i}}(C,V-C))$ for all $i$, and
 \im $w(E_{G_{i}}(C,V-C))\le\beta(n)\cd w(E_{G}(C,V-C))$ for some $i$.
 \EE
\EE
\end{theorem}
We remark that Madry's original algorithm is randomized, but the only randomized component is calling a low-stretch spanning tree algorithm as a black-box,  but we replace that with a deterministic construction with slightly worse parameters~\cite{ElkinEST08}.
\fi
% End comment out
% 

%\subsection{The $\WBCut$ Algorithm}

\begin{algorithm}[H]
 $\weighted ( G,\bd, \psi, \psi^*, c )$ with $\psi \ge \psi^*$ and $c\ge1$:
\BE

\im Fix an integer $r\ge1$ and parameter $t = \left\lceil m_0^{1/r} (\log m)^{O(1)} \log^2 U \right\rceil$, where $m_0$ is the number of edges in the \emph{original} input graph to the recursive algorithm, $m\le m_0$ is the number of edges of the input graph $G$ to the current recursive call, and $U$ is the capacity ratio of  $G$.

\im Fix parameters  $\al =(\log m)^{O(r^2)}$ as the approximation factor from \Cref{cor:sparsifier}, and $\be =O(\log m(\log\log m)^{O(1)})$ as the congestion factor from \Cref{thm:madrythm}. 

\im Compute $O(m/t)$-trees $G_1,\lds,G_t$ using \Cref{thm:madrythm} with $G$ and $t$ as input. For each $i$, let $K_i$ denote the vertex set in the core of $G_i$

\im For each $i\in[t]$:
 \BE

\im $H_i \gets G_i[K_i]$ 

\im Construct demands $\bd_{H_i}$ on $K_i$ as $\bd_{H_i}(v)=\sum_{u\in V: c_{G_i}(u)=v}\bd(u)$ (so that $\bd_{H_i}(K_i)=\bd(V)$).

\im $H_i'\gets \al $-approximate spectral sparsifier of $H_i$

\im $S'_{H_i}\gets \weighted(H_i',\bd_{H_i},\, \psi/\al ,\, 3\al \be \psi^*,\, c/3)$ \label{line:a1}

\im $S_{H_i} \gets S'_{H_i}$ with each vertex $v$ replaced with $V(T_{G_i}(v))$ (see \Cref{def:jtree})\label{line:uncontract H}

\im Construct a tree $T_i=(V_{T_i},E_{T_i},w_{T_i})$ with demands $\bd_{T_i}$ as follows: Starting with $G_i$, contract $K_i$ into a single vertex $k_i$ with demand $\bd(K_i)$. All other vertices have demand $\bd(v)$ (so that $\bd_{T_i}(V_{T_i})=\bd(V)$).\label{line:a2}

\im Root $T_i$ at a vertex $r_i\in V_{T_i}$ such that every subtree rooted at a child of $r_i$ has total weight at most $\bd_{T_i}(V)/2=\bd(V)/2$. \label{line:a3}

\im $S'_{T_i}\gets \rooted(T_i,\bd_{T_i},r_i,\psi)$ 

\im $S_{T_i}\gets S'_{T_i}$ with the vertex $k_i$ replaced with $K_i$ if $k_i\in S'_{T_i}$\label{line:uncontract T}
\EE

\im Of all the cuts $S=S_{H_i}$ or $S=S_{T_i}$ computed satisfying $w(S,V\sm S)\le\psi\cd\min\{\bd(S),\bd(V\sm S)\}$, consider the set $S$ with maximum $\min\{\bd(S),\bd(V\sm S)\}$, and output $S$ if $\bd(S)\le\bd(V\sm S)$ and $V\sm S$ otherwise. If no cut $S$ satisfies $w(S,V\sm S)\le\psi\cd\min\{\bd(S),\bd(V\sm S)\}$, then return $\emptyset$.

%It is guaranteed that one of $S_H$ and $S_T$ has conductance $\le O(\psi)$. Of the (one or two) cuts satisfying this property, output the one with highest $\bd(\cd)$ value. \label{line:a5}

\EE
\end{algorithm}

\begin{algorithm}[H]
$\rooted(T=(V_T,E_T,w_T),\bd_T,r,\psi_T)$:

\BE
\im[0.] Assumption: $T$ is a weighted tree with demands $\bd_T$. The tree is rooted at a root $r$ such that every subtree $V_u$ rooted at a vertex $u\in V_T\sm\{r\}$ has total demand $\bd_T(V_u)\le \bd_T(V_T)/2$.
\\Output: a set $S\s V_T$ satisfying the conditions of \Cref{lem:tree-alg}.


\im Find all vertices $u\in V_T\sm\{r\}$ such that if $V_u$ is the vertices in the subtree rooted at $u$, then $w_T(E[V_u,V_T\sm V_u])/\bd_T(V_u)\le2\psi_T$. Let this set be $X$.
\im Let $X^\uparrow$ denote all vertices $u\in X$ without an ancestor in $X$ (that is, there is no $v\in X\sm\{u\}$ with $u\in T_v$).
\im Starting with $S=\emptyset$, iteratively add the vertices $V_u$ for $u\in X^\uparrow$. If $\bd_T(S)\ge \bd_T(V_T)/4$ at any point, then terminate immediately and output $S$. Otherwise, output $S$ at the end.\label{line:t3}

\EE
\end{algorithm}
We analyze our algorithm $\weighted$ by showing the following:


\BL\leml{analysis}
Fix parameters $c\ge6$,  $\psi^*>0$, and $\psi \ge 12\beta\cd\psi^*$ for $\beta$ as defined in $\weighted$.
$\weighted$ outputs a $(\psi^*,c)$-most-balanced $(\psi,\bd)$-sparse cut.%\thatchaphol{The bounds of number of vertices and edges are not proved. I wonder how the factor $\log U$ and $\log^2 U$ come from \Cref{thm:madrythm}.} \jl{moved size bound separately to \lemm{size-bound}}
\EL

We begin with a lemma which says that, for each $i\in[t]$, either the graph $H_i$ contains a good balanced cut with respect to the $j$-tree $G_i$, or the graph $T_i$ does:




\BL\label{lem:either}
Fix $i\in[t]$, and let $S^*\s V$ be any cut with $\bd(S^*)\le \bd(V)/2$. For simplicity, define $K=K_i$, $k=k_i$, $T=T_i$, $r=r_i$, and $H=H_i$. One of the following must hold:
\BE
\im There exists a cut $S^*_T\s V_T$ in $T$ satisfying $w_T(E_T(S^*_T,V_T\sm S^*_T))\le w(E_{G_i}(S^*,V\sm S^*))$ and $\bd(S^*)/2\le \bd_T( S^*_T)\le 2\bd(V)/3$, and $S^*_T$ is the disjoint union of subtrees of $T$ rooted at $r$.
\im There exists a cut $S^*_H\s K$ in $H$ satisfying $w_H(E_{H}(S^*_H,K\sm S^*_H))\le w(E_{G_i}(S^*,V\sm S^*))$ and \linebreak $\min \{ \bd_H(S^*_H) , \bd_H(K\sm S^*_H)\} \ge\bd(S^*)/3$.
\EE
\EL
\BP
Let $S^*\s V$ the set as described in \ref{def:most-balanced-s} ($w(S^*,V\sm S^*)\le\psi\cd\min\{\bd(S^*),\bd(V\sm S^*)\}$). Let $U$ be the vertices $u\in V$ whose (unique) path to $c_{G_i}(u)$ in $F$ contains at least one edge in $E[S^*,V\sm S^*]$ (see \ref{fig:j}). Note that $U\cap K=\emptyset$ and $E_{G_i}(U,V\sm U)\s E_{G_i}(S^*,V\sm S^*)$. Moreover, suppose we first root the tree $T$ at $k$ (not $r$); then, for each vertex $u\in U$, its entire subtree is contained in $U$. Therefore, $U$ is a union of subtrees of $T$ rooted at $k$.


\begin{figure}
\centering \includegraphics[scale=.7]{0.pdf} \qquad \includegraphics[scale=.7]{1.pdf}
\caption{
Left: Case~1 of \Cref{lem:either}. The set $S^*$ is the cyan vertices. Right: Cases~2a and 2b.
}
\label{fig:j}
\end{figure}

\para{Case 1: $r\in U$.}
%In this case, let $U'\s U$ be the vertices in the subtree containing $r$ (\ref{fig:j} left).\thatchaphol{I suggest the following definition of $U'$
        Let $F$ be the peripheral forest of $G_i$ (see \Cref{def:jtree}) and let $T'$ be the tree in $F$ that contains $r$. Define $U' = T' \cap U$ (\ref{fig:j} left). In words, $U'$ contains all vertices of $U$ in the tree of $F$ that contains $r$. 
    Let us re-root $T$ at vertex $r$, so that the vertices in $V_T\sm U'$ now form a subtree. 

\para{Case 1a: $r\in U$ and $\bd_T(U')\le3\bd(V)/4$.}Define $S^*_T\s V_T$ as $S^*_T:=V_T\sm U'$ . By our selection of $r$, $\bd_T(S^*_T) =\bd_T(V_T\sm U')\le \bd(V)/2$. Moreover, $\bd_T(S^*_T)=\bd_T(V_T\sm U')\ge \bd(V)/4\ge \bd(S^*)/2$ and $E_T(S^*_T,V\sm S^*_T)\s E_{G_i}(U,V\sm U)\s E_{G_i}(S^*,V\sm S^*)$, so the conditions $\bd(S^*)/2\le \bd_T(S^*_T)\le \bd(V)/2$ and $w(E_T(S^*_T,V\sm S^*_T))\le w( E_{G_i}(S^*,V\sm S^*))$ are satisfied, fulfilling condition~(1).

\para{Case 1b: $r\in U$ and $\bd_T(U')\ge3\bd(V)/4$.} Define $\ol U\s U'$ as all vertices $u\in U'$ whose (unique) path to $r$ in $T$ contains at least one vertex not in $S^*$ (possibly $u$ itself). Note that $\ol U\supseteq U'\sm S^*$, so $\bd_T(\ol U)\ge\bd_T(U'\sm S^*)=\bd_T(U')-\bd_T(U'\cap S^*)\ge\bd_T(U')-\bd(S^*)\ge3\bd(V)/4-\bd(V)/2=\bd(V)/4$. Moreover, $\ol U$ is a union of subtrees of $T$ rooted at $r$ and satisfies $E_{G_i}(\ol U,V\sm\ol U)\s E_{G_i}(S^*,V\sm S^*)$. By our choice of $r$, each subtree $T'$ of $U$ satisfies $\bd_T(V(T'))\le\bd(V)/2$. If there exists a subtree $T'\s\ol U$ with $\bd_T(V(T'))\ge\bd(V)/4$, then set $S^*_T:=V(T')$, which satisfies $\bd(S^*)/2\le\bd(V)/4\le\bd_T(S^*_T)\le\bd(V)/2$ and  $w(E_T(S^*_T,V\sm S^*_T))\le w( E_{G_i}(\ol U,V\sm \ol U))\le w( E_{G_i}(S^*,V\sm S^*))$, fulfilling condition~(1). Otherwise, since $\bd_T(\ol U)\ge\bd(V)/4$, we can greedily select a subset of subtrees of $\ol U$ with total $\bd(\cd)$ value in the range $[\bd(V)/4,\bd(V)/2]$, and set $S^*_T$ as those vertices. This selection of $S^*_T$ also satisfies $\bd(S^*)/2\le\bd(V)/4\le\bd_T(S^*_T)\le\bd(V)/2$ and $w(E_T(S^*_T,V\sm S^*_T))\le w( E_{G_i}(\ol U,V\sm \ol U))\le w( E_{G_i}(S^*,V\sm S^*))$, fulfilling condition~(1).

\para{Case 2a: $r\notin U$ and $\bd_T(U)\ge \bd(V)/6$.}
Since $r\notin U$, every subtree in $U$ has weight at most $\bd(V)/2$. Let $U'$ be a subset of these subtrees of total $\bd(\cd)$ value in the range $[\bd(V)/6,2\bd(V)/3]$.
Define $S^*_T:=U'$, which satisfies $\bd(V)/2\ge\bd_T(S^*_T)\ge \bd(V)/6\ge\bd(S^*)/3$ and $E_T(S^*_T,V\sm S^*_T)\s  E_{G_i}(U,V\sm U)\s E_{G_i}(S^*,V\sm S^*)$, fulfilling condition~(1).

\para{Case 2b: $r\notin U$ and $\bd_T(U)<\bd(V)/6$.}
In this case, let $S:=S^*\cup U$, which satisfies $\bd(S^*)\le\bd(S)\le\bd(S^*)+\bd_T(U)\le\bd(S^*)+\bd(V)/6\le2\bd(V)/3$ and $E_{G_i}(S,V\sm S)\s E_{G_i}(S^*,V\sm S^*)$. Next, partition $S$ into $S_H$ and $S_T^*$, where $S_H$ consists of the vertices of all connected components of $G_i[S]$ that intersect $K$, and $S_T^*:=S\sm S_H$ is the rest. Clearly, we have $E_{G_i}(S_H,V\sm S_H)\s E_{G_i}(S^*,V\sm S^*)$ and  $E_{G_i}(S_T^*,V\sm S_T^*)\s E_{G_i}(S^*,V\sm S^*)$. 
%Also, observe that for each tree $T'$ in the peripheral forest $F$ of $G_i$ (see \Cref{def:jtree}), either $V(T')\s S_T^*$ or $V(T')\cap S_T^*=\emptyset$.\thatchaphol{Why? Not true from figure. Define $F$. $T$ is used for the contracted graph already. Use $S_K$ or $S_H$ consistently.} \jl{defined $F$ as peripheral forest. Sticking with $S_H$}

We have that either $\bd_T(S_T^*)\ge\bd(S)/2$ or $\bd(S_H)\ge\bd(S)/2$. If the former is true, then the set $S^*_T$ satisfies condition~(1). Otherwise, assume the latter. 
Since $E_{G_i}(S_{H},V\sm S_{H})$ does not contain any edges in the peripheral forest $F$, there exists a set $S^*_H:=\{c_{G_i}(v):v\in S_H\}\s K$ such that $S_H$ is the vertices in the trees in $F$ intersecting $S^*_H$. This also means that $V\sm S_H$ is the vertices in the trees of $F$ intersecting $K\sm S^*_H$. We have $w_H(E_{H}(S^*_H,K\sm S^*_H))=w(E_{G_i}(S_H,V\sm S_H))\le w(E_{G_i}(S^*,V\sm S^*))$, and 
\[ \min \{ \bd_H(S^*_H) , \bd_H(K\sm S^*_H)\} = \min \{ \bd(S_H),\bd(V\sm S_H)\} .\]
It suffices to show that $\min\{\bd(S_H),\bd(V\sm S_H)\}\ge\bd(S^*)/3$. 
This is true because 
$\bd(S_H)\ge\bd(S)/2\ge \bd(S^*)/2$ and
$\bd(S_H)\le\bd(S)\le2\bd(V)/3$ which means that $\bd(V\sm S_H) \ge \bd(V)/3 \ge \bd(S^*)/3$.
 %$\bd(S_H)\le\bd(S^*)+\bd(V)/4\le3\bd(V)/4$
 %so $\min \{ \bd(S_H),\bd(V\sm S_H)\}\ge\bd(S^*)/3$, and this along with $\bd(S_H)\ge\bd(S^*)$ shows that $\min\{\bd(S_H),\bd(V\sm S_H)\}\ge\bd(S_H)/3\ge\bd(S^*)/3$.
\EP

If the graph $H$ contains a good balanced cut, then intuitively, the demands $\bd_H$ are set up so that the recursive call on $H'$ will find a good cut as well. The lemma below shows that if the tree $T$ contains a good balanced cut, then $\rooted$ will perform similarly well.

\BL\label{lem:tree-alg}
$\rooted(T=(V_T,E_T,w_T),\bd_T,r,\psi_T)$ can be implemented to run in $O(|V_T|)$ time.
The set $S$ output satisfies $\Phi_{T}^{\bd_T}(S)=w_T(E[S,V_T\sm S])/\min\{\bd_T(S),\bd_T(V_T\sm S)\}\le6\psi_T$.
Moreover, for any set $S^*$ with $w_T(E[S^*,V_T\sm S^*])/ \bd_T(S^*)\le \psi_T$ and  $ \bd_T(S^*)\le2 \bd_T(V_T)/3$, and which is composed of vertex-disjoint subtrees rooted at vertices in $T$, we have $\min\{ \bd_T(S), \bd_T(V_T\sm S)\}\ge  \bd_T(S^*)/3$.
\EL
\BP
Clearly, every line in the algorithm can be implemented in linear time, so the running time follows. We focus on the other properties.

Every set of vertices $V_u$ added to $S$ satisfies $w_T(E[V_u,V_T\sm V_u])/ \bd_T(V_u)\le2\psi_T$. Also, the added sets $V_u$ are vertex-disjoint, so $w_T(E[S,V_T\sm S]) = \sum_{V_u\s S}w_T(E[V_u,V_T\sm V_u])$. This means that $\rooted$ outputs $S$ satisfying $w_T(E[S,V_T\sm S])/ \bd_T(S)\le2\psi_T$. Since every set $V_u$ has total weight at most $ \bd_T(V_T)/2$, and since the algorithm terminates early if $ \bd_T(S)\ge  \bd_T(V_T)/4$, we have $ \bd_T(S)\le 3 \bd_T(V_T)/4$. This means that $\min\{ \bd_T(S), \bd_T(V_T\sm S)\}\ge \bd_T(S)/3$, so $w_T(E[S,V_T\sm S])/\min\{ \bd_T(S), \bd_T(V_T\sm S)\} \le 3w_T(E[S,V_T\sm S])/ \bd_T(S)\le6\psi_T$.

Suppose first that the algorithm terminates early. Then, as argued above, $\min\{ \bd_T(S), \bd_T(V_T\sm S)\}\ge  \bd_T(V_T)/4$, which is at least $(2 \bd_T(V_T)/3)/3\ge  \bd_T(S^*)/3$, so  $\min\{ \bd_T(S), \bd_T(V_T\sm S)\}\ge  \bd_T(S^*)/3$.

Now suppose that $S$ does not terminate early. Let $S^*_1,\lds,S^*_\el$ be the vertices in the (vertex-disjoint) subtrees that together compose $S^*$, that is, $\bigcup_iS^*_i=S^*$. Note that $E[S^*_i,V_T\sm S^*_i]$ is a single edge in $E$ for each $i$. Suppose we reorder the sets $S^*_i$ so that $S^*_1,\lds, S^*_q$ are the sets that satisfy $w_T(E[S^*_i,V_T\sm S^*_i])/ \bd_T(S^*_i)\le2\psi_T$. Since $w_T(E[S^*,V_T\sm S^*])/ \bd_T(S^*)\le \psi_T$, by a Markov's inequality-like argument, we must have $\sum_{i\in[q]} \bd_T(S^*_i) \ge (1/2)\sum_{i\in[\el]} \bd_T(S^*_i)= \bd_T(S^*)/2$. Observe that by construction of $X^\uparrow$, each of the subsets $S^*_1,\lds, S^*_q$ is inside $V_u$ for some $u\in X^\uparrow$. Therefore, the set $S$ that $\rooted$ outputs satisfies $ \bd_T(S)\ge\sum_{i\in[q]} \bd_T(S^*_i)\ge  \bd_T(S^*)/2$. The bound on $w_T(E[S,V_T\sm S])/\min\{ \bd_T(S), \bd_T(V_T\sm S)\}$ follows as before.
\EP

Finally, we prove \lemm{analysis}:

\BP[Proof (\lemm{analysis})]
Let $S^*\s V$ be the set for $G$ as described in \Cref{def:most-balanced-s}; that is, it is the set with maximum $\bd(S^*)$ out of all sets $S'$ satisfying  $\Psi_{G}^{\bd}(S')\le\psi ^*$ and $\bd(S')\le\bd(V)/2$. If $\bd(S^*)=0$, then  $\weighted$ always outputs a   $(\psi^*,c)$-most-balanced $(\psi,\bd)$-sparse cut, even if it outputs $\emptyset$. So for the rest of the proof, assume that $\bd(S^*)>0$, so that $\Psi_G^\bd(S^*)$ and $\Psi_{G_i}^\bd(S^*)$ are well-defined.

By \Cref{thm:madrythm}, there exists $i\in[t]$ such that $w(E_{G_i}(S^*,V-S^*))\le \be \cd w(E_G(S^*,V-S^*))$, which means that 
\[ \Psi_{G_i}^\bd(S^*)\le\be \cd \Psi_G^\bd(S^*) \le \be \cd\psi^* .\]
For the rest of the proof, we focus on this $i$, and define $K=K_i$, $H=H_i$, and $T=T_i$. We break into two cases, depending on which condition of \lemm{either} is true:
 \BE
 \im Suppose condition~(1) is true for the cut $S^*_T$. Then, since $w_T(E_T(S^*_T,V_T\sm S^*_T))\le w(E_{G_i}(S^*,V\sm S^*))$ and $\bd_T(S^*_T)\ge\bd(S^*)/2$, we have
\[ \f{w(E_{G_i}(S^*,V\sm S^*))}{\bd_T(S^*_T)} \le \f{w(E_{G_i}(S^*,V\sm S^*))}{\bd(S^*)/2}\le2\Psi_{G_i}^\bd(S^*)\le2\be \cd\psi^* .\]
Also, $\bd_T(S^*_T)\le2\bd(V)/3=2\bd_T(V_T)/3$. 
Let $S'_T$ be the cut in $T$ that $\rooted$ outputs and let $S_T$ the corresponding cut in $G_i$ after the uncontraction in Step~\Dref{line:uncontract T}.
Applying \lemm{tree-alg} with $\psi_T=2\be \cd\psi^*$, the cut $S'_T$ satisfies
$\Psi_T^{\bd_T} (S'_T)\le 6\psi_T = 12\be \cd\psi^*$ and $\min\{\bd_T(S'_T),\bd_T(V_T\sm S'_T)\}\ge\bd_T(S^*_T)/3$. By construction, $\bd(S_T)=\bd(S'_T)\ge\bd_T(S^*_T)/3\ge\bd(S^*)/6 \ge \bd(S^*)/c$ and $\Psi_{G_i}^\bd(S_T)=\Psi_T^{\bd_T}(S'_T)\le12\be \cd\psi^* \le \psi$.

\im Suppose condition~(2) is true for the cut $S^*_H$. Since $w_H(E_{H}(S^*_H,K\sm S^*_H))\le w(E_{G_i}(S^*,V\sm S^*))$ and $\min \{ \bd_H(S^*_H) , \bd_H(K\sm S^*_H)\} \ge\bd(S^*)/3 $, we have $\Psi_H^{\bd_H}(S^*_H)\le3\Psi_{G_i}^{\bd}(S^*)\le3\be \cd\psi^*$. Since $H'$ is an $\al$-approximate spectral sparsifier of $H$, we have $\Psi_{H'}^{\bd_H}(S^*_H) \le \al \cd3\Psi_H^{\bd_H}(S^*_H)\le3\al \be \cd\psi^*$. By induction on the smaller recursive instance $\weighted(H',\bd_H, \psi/\al , 3\al \be \psi^*,c/3)$, the cut $S'_H$ computed is a $(3\al \be \psi^*,c/3)$-most-balanced $(\psi/\al ,\bd_H)$-sparse cut. Since $H'$ is an $\al$-approximate spectral sparsifier of $H$, we have $\Psi_H^{\bd_H}(S'_H) \le \al \cd\Psi_{H'}^{\bd_H}(S'_H)\le\al \cd \psi/\al =\psi$. 
Let $S_H$ be the cut in $G_i$ corresponding to $S'_H$ after the uncontraction in Step~\Dref{line:uncontract H}.
By construction, $\Psi_{G_i}^\bd(S_H)=\Psi_H^{\bd_H}(S'_H) \le \psi$ and
$\bd(S_H)=\bd_H(S'_H)$. Since $S^*_H$ is a cut with $\Psi_{H'}^{\bd_H}(S^*_H)\le3\al \be \psi^*$, we have
\[ \bd(S_H)=\bd_H(S'_H)\ge\f{\min\{\bd_H(S^*_H),\bd_H(K\sm S^*_H)\}}{c/3} \ge \f{\bd(S^*)/3}{c/3}=\f{\bd(S^*)}c .\]
 \EE
In both cases, the computed cut is a  $(\psi^*,c)$-most-balanced $(\psi,\bd)$-sparse cut.
\EP

The lemma below will be useful in bounding the running time of the recursive algorithm.
\BL\leml{size-bound}
For any integer $t\ge1$ (as defined by the algorithm), the algorithm makes $t$ recursive calls $\weighted(H',\bd_H,\psi/\al ,\, 3\al \be \psi^*,\, c/3)$ on graphs $H'$ with $\tO(\f{m\log U}t)$ vertices and $\tO(\f{m \log^2U}t)$ edges, and runs in $\tO(tm)$ time outside these recursive calls.
\EL
\BP
By \thmm{madrythm}, computing the graphs $G_1,\lds,G_t$ takes $\tO(tm)$ time. By \lemm{tree-alg}, $\rooted$ runs in $O(m)$ time for each $G_t$, for a total of $O(tm)$ time. Since each graph $G_i$ is a $\tO(\f{m\log U}t)$-tree, by construction, each graph $H_{i}$ has at most $\tO(\f{m\log U}t)$ vertices. By \Cref{cor:sparsifier}, the sparsified graphs $H'_{i}$ have at most $\tO(\f{m\log U}t)\log m\log U\le\tO(\f{m\log^2U}t)$ edges.
\EP

Finally, we plug in our value $t = \left\lceil m^{1/r} (\log m)^{O(1)} \log^2 U \right\rceil$ that balances out the running time $\tO(tm)$ outside the recursive calls and the number $r$ of recursion levels.

\BT\thml{weighted-bal}
Fix parameters $\psi^*>0$ and $\psi=12\be\cd(3\al^2\be)^r\cd\psi^* = (\log m)^{O(r^3)}\cd\psi^*$.
There is a constant $c_0$ and deterministic algorithm that, given a weighted graph $G$ with $m$ edges and capacity ratio $U$, and demands $\bd$, and parameters $\psi^*\in (0,1]$ and $1\leq r\leq O(\log m)$, computes a $(\psi^*,6\cd3^r)$-most-balanced $((\log(mU))^{c_0 r^3} \cd \psi^*,\bd)$-sparse cut in time $m^{1+1/r}\lp\log(mU)\rp^{O(1)}$.
\ET
\BP
Let $G$ be the original graph with $m=m_0$ edges.
Let $G'$ be the current input graph in a recursive call of $\weighted$, with $m'$ edges and capacity ratio $U'$. Set the parameters $t = \left\lceil m^{1/r} (\log m')^{O(1)} \log^2 U' \right\rceil$ from the algorithm and $\al =(\log m')^{O(r^2)}$ from \Cref{cor:sparsifier} and $\be =O(\log m'(\log\log m')^{O(1)})\le(\log m')^{O(1)}$ from \Cref{thm:madrythm}. By \lemm{size-bound}, the algorithm makes $t=m^{1/r} (\log m')^{O(1)}\log^2U'$ many recursive calls to graphs with at most  $\tO(\f{m'\log^2U'}t)\le m'/m^{1/r}$ edges, where $U'$ is the capacity ratio of the current graph, so there are $r$ levels of recursion. By \Cref{thm:madrythm}, the capacity ratio of the graph increases by an $O(m)$ factor in each recursive call, so we have $U'\le O(m)^r U$ for all recursive graphs, which means $t \le m^{1/r}(r\log m+\log U)^{O(1)}$. By \lemm{size-bound}, the running time $\tO(tm')$ outside the recursive calls for this graph is $m'm^{1/r}(r\log m+\log U)^{O(1)}$. For recursion level $1\le i\le r$, there are $m^{i/r}\lp r\log m+\log U\rp^{O(i)}$ many graphs at this recursion level, each with $m'\le m^{1-i/r}$, so the total time spent on graphs at this level, outside their own recursive calls, is at most
\[ m^{i/r}\lp r\log m+\log U\rp^{O(i)} \cd m^{1-i/r}m^{1/r}(r\log m+\log U)^{O(1)} = m^{1+1/r}(r\log m+\log U)^{O(i)} .\]
Summed over all $1\le i\le r$ and using $r\le O(\log m)$, the overall total running time becomes $m^{1+1/r}(\log(mU))^{O(r)}$.

We also need to verify that the conditions $\psi\ge12\be\cd\psi^*$ and $c\ge6$ of \lemm{analysis} are always satisfied throughout the recursive calls. Since each recursive call decreases the parameter $c$ by a factor of $3$, and $c=6\cd3^r$ initially, the value of $c$ is always at least $6$. Also, in  each recursive call, the ratio $\psi/\psi^*$ decreases by a factor $3\al^2\be$, so for the initial value $\psi=12\be\cd(3\al^2\be)^r\cd\psi^* $ in the theorem statement, we always have $\psi/\psi^*\ge12\be$.
\EP

\subsection{Completing the Proof of \thmm{WBCut}}

In order to prove \thmm{WBCut}, we first present the lemma below, which is essentially a weighted version of \Cref{lem: single stage}.

\begin{lem}\leml{z}
Let $G=(V,E)$ be a weighted graph with edge weights in $[1,U]$, and demands $\bd(v)\in\{0\}\cup[1,U]$ for all $v\in V$ that are not all zero.
        There is a universal constant $c_1$ and a deterministic algorithm, that, given a vertex subset $V'\subseteq V$ with $\bd(V')\ge\bd(V)/2$, 
        and parameters $0<\psi<1$, $0<z'<z$, such that for every partition $(A,B)$ of $V'$ with $w(E_{G}(A,B))\leq \psi\cdot  \min\set{\bd(A),\bd(B)}$, $\min\set{\bd(A),\bd(B)}\leq z$ holds,
        computes a partition $(X,Y)$ of $V'$, where  $\bd(X)\leq \bd(Y)$ (where possibly $X=\emptyset$),  $w(E_{\hG}(X,Y))\leq \psi \cdot\bd(X)$, and one of the following holds:
        
        \begin{itemize}
                \item either $\bd(X),\bd(Y)\geq \bd(V')/3$ (note that this can only happen if $z\geq \bd(V')/3$); or
                \item for every partition $(A',B')$ of the set $Y$ of vertices with \[ w(E_{\hG}(A',B'))\leq \frac{\psi}{(\log(mU))^{c_1 r^3}}\cdot \min\set{\bd(A'),\bd(B')},\] $\min\set{\bd(A'),\bd(B')}\leq z'$ must hold (if $z'<1$, then graph $G[Y]$ is guaranteed to be a $\psi / (\log(mU))^{c_1 r^3}$-expander).
        \end{itemize}

The running time of the algorithm is $O\left (\frac{z}{z'}\cdot m^{1+1/r}\lp\log(mU)\rp^{O(1)} \right )$.
\end{lem}
\BP
The algorithm and analysis proceed similarly to that of \Cref{lem: single stage}, except that here, the graph $ G$ is the same as $G$. Also, \lemm{analysis} takes the role of both \Cref{thm: sparse edge cut of large profit or witness} and \Cref{thm: sparse edge cut or expander} in the proof of \Cref{lem: single stage}.

We set parameter $z^*=z'/(6\cd3^r)$. Unlike in the proof of \Cref{lem: single stage}, we do not make the distinction whether $z^*\ge1$.% Assume first that $z^*\geq 1$; we will discuss the other case later.

Our algorithm is iterative. At the beginning of iteration $i$, we are given a subgraph $G_i\subseteq  G$, such that $\bd(V(G_i))\geq 2\bd(V')/3$; at the beginning of the first iteration, we set $G_1= G[V']$. 
At the end of iteration $i$, we either terminate the algorithm with the desired solution, or we compute a subset $S_i\subseteq V(G_i)$ of vertices, such that $\bd(S_i)\leq \bd(V(G_i))/2$, and $w(E_{G_i}(S_i, V(G_i)\setminus S_i))\leq \psi\cdot \bd(S_i)/2$. We then delete the vertices of $S_i$ from $G_i$, in order to obtain the graph $G_{i+1}$, that serves as the input to the next iteration. The algorithm terminates once the current graph $G_i$ satisfies $\bd(V(G_i)) < 2\bd(V')/3$ (unless it terminates with the desired output beforehand).

We now describe the execution of the $i$th iteration. We assume that the sets $S_1,\ldots,S_{i-1}$ of vertices are already computed, and that $\sum_{i'=1}^{i-1}\bd(S_{i'})\leq \bd(V')/3$. Recall that $G_i$ is the sub-graph of $ G[V']$ that is obtained by deleting the vertices of $S_1,\ldots,S_{i-1}$ from it. Recall also that we are guaranteed that $\bd(V(G_i))\geq 2\bd(V')/3\geq \bd(V)/3$. We apply \thmm{weighted-bal} to graph $G_i$ with parameters $\psi^*=(\psi/2) / (\log(mU))^{c_1 r^3}$ and $r$, and let $X$ be the returned set, which is  a  $(\psi^*,6\cd3^r)$-most-balanced $((\log(mU))^{c_1 r^3} \cd \psi^*,\bd)$-sparse cut satisfying $\bd(X)\le\bd(V)/2$. 

If $\bd(X)\le z^*=z'/(6\cd3^r)$, then we terminate the algorithm, and return the partition $(X,Y)$ of $V'$ where $X=\bigcup_{i'=1}^iS_{i'}$, and $Y=V'\setminus X$. This satisfies the second condition of \lemm{z}, since by the most-balanced sparse cut definition, every partition $(A',B')$ of the set $Y$ of vertices with $w(E_{\hG}(A',B'))\leq \frac{\psi}{(\log(mU))^{c_1 r^3}}\cdot \min\set{\bd(A'),\bd(B')}$ must satisfy $\min\{\bd(A'),\bd(B')\}\le6\cd3^r\cd\bd(X) < 6\cd3^r\cd z^*=z'$.

Otherwise, $\bd(X)> z^*$. In this case, we set $S_i=X$ and continue the algorithm. If $\sum_{i'=1}^i\bd(S_{i'})\leq \bd(V')/3$ continues to hold, then we let $G_{i+1}=G_i\setminus S_i$, and continue to the next iteration. Otherwise, we terminate the algorithm, and return the partition $(X,Y)$ of $V'$ where $X=\bigcup_{i'=1}^iS_{i'}$, and $Y=V'\setminus X$. Recall that we are guaranteed that $\bd(X)\geq \bd(V')/3$. 

To show that  $w(E_{\hG}(X,Y))\leq \psi \cdot\bd(X)$, note that every cut $S_i$ satisfies $w(E_{G_{i}}(S_i,V(G_i)\sm S_i))\le(\psi/2)\bd(S_i)$, so $w(E_G(X,Y)) \le \sum_{i'=1}^iw(E_{G_i}(S_i,V(G_i)\sm S_i)) \le (\psi/2)\sum_{i'=1}^i\bd(S_i)=(\psi/2)\bd(X)$, which is at most $\psi\min\{\bd(X),\bd(V\sm X)\}$ since  $\bd(X)\le2\bd(V)/3$. to \Cref{lem: single stage}.

The bound on the running time of the algorithm proceeds similarly. Observe that we are guaranteed that for all $i$, $\bd(S_i)\geq z^*$. Notice however that throughout the algorithm, if we set $A=\bigcup_{i'=1}^iS_{i'}$ and $B=V'\setminus A$, then 
$\bd(A)<\bd(B)$ holds, and $w(E_{ G}(A,B))\leq \psi\cdot  \bd(A)$. Therefore, from the condition of the lemma, $\bd(A)\leq z$ must hold. Overall, the number of iterations in the algorithm is bounded by $z/z^*=6\cd3^r\cdot z/z'$, and, since every iteration takes time $m^{1+1/r}\lp\log(mU)\rp^{O(1)} $, total running time of the algorithm is bounded by $\frac z {z'}\cdot m^{1+1/r}\cdot (\log (mU))^{O(1)}$. 
\EP

We are now ready to complete the proof of \thmm{WBCut}, which follows almost identically from that of \ref{thm:main restatement} with slightly different parameters. First, we set $z_1=\bd(V)/2$, and for $1<i\leq r$, we set $z_i=z_{i-1}/(\bd(V)/2)^{1/r}$; in particular, $z_r=1$ holds. We also define parameters $\psi_1,\ldots,\psi_{r}$, by letting $\psi_r=\psi$, and, for all $1\leq i<r$, setting $\psi_{i}=8 \cd (\log(mU))^{c_1 r^3}\cdot \psi_{i+1}$, where $c_1$ is the constant from \lemm{z}. Notice that $\psi_1\leq \psi \cd  (\log m)^{O(r^4)}$. The algorithm and analysis follow identically, except that here, $\hat G=G$ (i.e., all sets are canonical), cardinalities $|X|$ of vertex sets $X$ are replaced by $\bd(X)$, and sizes of cuts $|E_G(X,Y)|$ are replaced by their weighted counterpart $w_G(X,Y)$. In particular, the running time is now $O\left (\frac{z_i}{z_{i+1}}\cdot m^{1+1/r}\cdot (\log (mU))^{O(1)}\right ) = O \lp (\bd(V)/2)^{1/r} \cd m^{1+1/r} \cd (\log(mU))^{O(1)} \rp = m\cd(mU)^{O(1/r)}$, as required.


 

